Disparate Impact Diminishes Consumer Trust Even for Advantaged Users

Systems aiming to aid consumers in their decision-making (e.g., by implementing persuasive techniques) are more likely to be effective when consumers trust them. However, recent research has demonstrated that the machine learning algorithms that often underlie such technology can act unfairly towards specific groups (e.g., by making more favorable predictions for men than for women). An undesired disparate impact resulting from this kind of algorithmic unfairness could diminish consumer trust and thereby undermine the purpose of the system. We studied this effect by conducting a between-subjects user study investigating how (gender-related) disparate impact affected consumer trust in an app designed to improve consumers' financial decision-making. Our results show that disparate impact decreased consumers' trust in the system and made them less likely to use it. Moreover, we find that trust was affected to the same degree across consumer groups (i.e., advantaged and disadvantaged users) despite both of these consumer groups recognizing their respective levels of personal benefit. Our findings highlight the importance of fairness in consumer-oriented artificial intelligence systems.

==> library <==
Automatically generated by Mendeley Desktop 1.19.4
Any changes to this file will be lost if it is regenerated by Mendeley.

BibTeX export options can be customized via Preferences -> BibTeX in Mendeley Desktop

@article{Yang2018a,
abstract = {HCI has become particularly interested in using machine learning (ML) to improve user experience (UX). However, some design researchers claim that there is a lack of design innovation in envisioning how ML might improve UX. We investigate this claim by analyzing 2,494 related HCI research publications. Our review confirmed a lack of research integrating UX and ML. To help span this gap, we mined our corpus to generate a topic landscape, mapping out 7 clusters of ML technical capabilities within HCI. Among them, we identified 3 under-explored clusters that design researchers can dig in and create sensitizing concepts for. To help operationalize these technical design materials, our analysis then identified value channels through which the technical capabilities can provide value for users: self, context, optimal, and utility-capability. The clusters and the value channels collectively mark starting places for envisioning new ways for ML technology to improve people's lives.},
author = {Yang, Qian and Banovic, Nikola and Zimmerman, John},
doi = {10.1145/3173574.3173704},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Yang, Banovic, Zimmerman - 2018 - Mapping machine learning advances from HCI research to reveal starting places for design innovation.pdf:pdf},
isbn = {9781450356206},
journal = {Conf. Hum. Factors Comput. Syst. - Proc.},
keywords = {Bibliometric,Data mining,Machine learning,Research transfer,Sensitizing concept,User experience},
pages = {1--11},
title = {{Mapping machine learning advances from HCI research to reveal starting places for design innovation}},
volume = {2018-April},
year = {2018}
}
@article{Singh2018a,
abstract = {Rankings are ubiquitous in the online world today. As we have transitioned from finding books in libraries to ranking products, jobs, job applicants, opinions and potential romantic partners, there is a substantial precedent that ranking systems have a responsibility not only to their users but also to the items being ranked. To address these often conflicting responsibilities, we propose a conceptual and computational framework that allows the formulation of fairness constraints on rankings in terms of exposure allocation. As part of this framework, we develop efficient algorithms for finding rankings that maximize the utility for the user while provably satisfying a specifiable notion of fairness. Since fairness goals can be application specific, we show how a broad range of fairness constraints can be implemented using our framework, including forms of demographic parity, disparate treatment, and disparate impact constraints. We illustrate the effect of these constraints by providing empirical results on two ranking problems.},
annote = {introducing conceptual and computational framework that allows for fairness constraints on rankings in terms of exposure (algorithm makes a utility-fairness tradeoff)

see summary 3.5 for description of framework

different applications have different fairness constraints (e.g., demographic parity, disparate impact, disparate treatment, ...); the authors aimed to make a framework that can incorporate all of these 

basically with this framework you can add fairness constraints to any ranking that would otherwise be entirely relevance based},
archivePrefix = {arXiv},
arxivId = {1802.07281},
author = {Singh, Ashudeep and Joachims, Thorsten},
doi = {10.1145/3219819.3220088},
eprint = {1802.07281},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Singh, Joachims - 2018 - Fairness of exposure in rankings.pdf:pdf},
isbn = {9781450355520},
journal = {Proc. ACM SIGKDD Int. Conf. Knowl. Discov. Data Min.},
keywords = {Algorithmic bias,Equal opportunity,Fairness,Fairness in rankings,Position bias},
pages = {2219--2228},
title = {{Fairness of exposure in rankings}},
year = {2018}
}
@article{Thonet2017,
abstract = {{\textcopyright} 2017 ACM. Social media platforms such as weblogs and social networking sites provide Internet users with an unprecedented means to express their opinions and debate on a wide range of issues. Concurrently with their growing importance in public communication, social media platforms may foster echo chambers and filter bubbles: homophily and content personalization lead users to be increasingly exposed to conforming opinions.There is therefore a need for unbiased systems able to identify and provide access to varied viewpoints. To address this task, we propose in this paper a novel unsupervised topic model, the Social Network Viewpoint Discovery Model (SNVDM). Given a specific issue (e.g., U.S. policy) as well as the text and social interactions from the users discussing this issue on a social networking site, SNVDM jointly identifies the issue's topics, the users' viewpoints, and the discourse pertaining to the different topics and viewpoints. In order to overcome the potential sparsity of the social network (i.e., some users interact with only a few other users), we propose an extension to SNVDM based on the Generalized p{\'{o}}lya Urn sampling scheme (SNVDM-GPU) to leverage "acquaintances of acquaintances" relationships. We benchmark the different proposed models against three baselines, namely TAM, SN-LDA, and VODUM, on a viewpoint clustering task using two real-world datasets. We thereby provide evidence that our model SNVDM and its extension SNVDM-GPU significantly outperform state-of-the-art baselines, and we show that utilizing social interactions greatly improves viewpoint clustering performance.},
author = {Thonet, Thibaut and Cabanac, Guillaume and Boughanem, Mohand and Pinel-Sauvagnat, Karen},
doi = {10.1145/3132847.3132897},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Thonet et al. - 2017 - Users Are Known by the Company They Keep.pdf:pdf},
isbn = {9781450349185},
keywords = {social networks,topic modeling,viewpoint discovery},
pages = {87--96},
title = {{Users Are Known by the Company They Keep}},
year = {2017}
}
@article{Whittlestone,
annote = {PhD thesis about confirmation bias and open-mindedness

cool insights with regard to a lack of evidence for the pervasiveness of confirmation bias; 

nice suggestions for future research at the end},
author = {Whittlestone, Jess},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Whittlestone - Unknown - The importance of making assumptions why confirmation is not necessarily a bias by.pdf:pdf},
title = {{The importance of making assumptions : why confirmation is not necessarily a bias by}}
}
@article{Araujo2020,
abstract = {Fueled by ever-growing amounts of (digital) data and advances in artificial intelligence, decision-making in contemporary societies is increasingly delegated to automated processes. Drawing from social science theories and from the emerging body of research about algorithmic appreciation and algorithmic perceptions, the current study explores the extent to which personal characteristics can be linked to perceptions of automated decision-making by AI, and the boundary conditions of these perceptions, namely the extent to which such perceptions differ across media, (public) health, and judicial contexts. Data from a scenario-based survey experiment with a national sample (N = 958) show that people are by and large concerned about risks and have mixed opinions about fairness and usefulness of automated decision-making at a societal level, with general attitudes influenced by individual characteristics. Interestingly, decisions taken automatically by AI were often evaluated on par or even better than human experts for specific decisions. Theoretical and societal implications about these findings are discussed.},
author = {Araujo, Theo and Helberger, Natali and Kruikemeier, Sanne and de Vreese, Claes H.},
doi = {10.1007/s00146-019-00931-w},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Araujo et al. - 2020 - In AI we trust Perceptions about automated decision-making by artificial intelligence.pdf:pdf},
isbn = {0123456789},
issn = {14355655},
journal = {AI Soc.},
keywords = {Algorithmic appreciation,Algorithmic fairness,Artificial intelligence,Automated decision-making,User perceptions},
number = {3},
pages = {611--623},
publisher = {Springer London},
title = {{In AI we trust? Perceptions about automated decision-making by artificial intelligence}},
url = {https://doi.org/10.1007/s00146-019-00931-w},
volume = {35},
year = {2020}
}
@article{Loyd2013,
abstract = {Apurported downside of social category diversity is decreased relationship focus (i.e., one's focus on establishing a positive social bond with a coworker). However, we argue that this lack of relationship focus serves as a central mechanism that improves information processing even prior to interaction and, ultimately, decision-making performance in diverse settings. We introduce the construct of premeeting elaboration (i.e., the extent to which individuals consider their own and others' perspectives in the anticipation of an interaction) and explore its link with social category diversity and relationship focus. Experiments 1 and 2 demonstrate that when disagreement occurs, social category diversity increases premeeting elaboration, with relationship focus as a central causal mechanism. Experiment 3 shows that premeeting elaboration has important implications for performance: disagreeing dyads with social category diversity elaborate more prior to meeting and, as a result, perform better on a decision-making task than those with social category homogeneity. We discuss the value of studying early-stage interaction and propose a reconsideration of the "downside" of social category diversity. {\textcopyright} 2013 INFORMS.},
author = {Loyd, Denise Lewin and Wang, Cynthia S. and Phillips, Katherine W. and Lount, Robert B.},
doi = {10.1287/orsc.1120.0761},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Loyd et al. - 2013 - Social category diversity promotes premeeting elaboration The role of relationship focus.pdf:pdf},
issn = {10477039},
journal = {Organ. Sci.},
keywords = {Decision-making performance,Disagreement,Premeeting elaboration,Relationship focus,Social category diversity},
number = {3},
pages = {757--772},
title = {{Social category diversity promotes premeeting elaboration: The role of relationship focus}},
volume = {24},
year = {2013}
}
@article{Sakai2011,
abstract = {Search queries are often ambiguous and/or underspecified. To accomodate different user needs, search result diversification has received attention in the past few years. Accordingly, several new metrics for evaluating diversification have been proposed, but their properties are little understood. We compare the properties of existing metrics given the premises that (1) queries may have multiple intents; (2) the likelihood of each intent given a query is available; and (3) graded relevance assessments are available for each intent. We compare a wide range of traditional and diversified IR metrics after adding graded relevance assessments to the TREC 2009 Web track diversity task test collection which originally had binary relevance assessments. Our primary criterion is discriminative power, which represents the reliability of a metric in an experiment. Our results show that diversified IR experiments with a given number of topics can be as reliable as traditional IR experiments with the same number of topics, provided that the right metrics are used. Moreover, we compare the intuitiveness of diversified IR metrics by closely examining the actual ranked lists from TREC. We show that a family of metrics called D{\#}-measures have several advantages over other metrics such as $\alpha$-nDCG and Intent-Aware metrics.},
annote = {the diversity metrics discussed here are about diversity as a means of dealing with underspecified or ambiguous queries; by increasing diversity lowering the risk of user dissatisfaction

in this paper the authors just list a couple of diversity metrics and evaluate them; they conclude that D{\#} measures (their own) are the best},
author = {Sakai, Tetsuya and Song, Ruihua},
doi = {10.1145/2009916.2010055},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sakai, Song - 2011 - Evaluating diversified search results using per-intent graded relevance.pdf:pdf},
isbn = {9781450309349},
journal = {SIGIR'11 - Proc. 34th Int. ACM SIGIR Conf. Res. Dev. Inf. Retr.},
keywords = {Ambiguity,Diversity,Evaluation,Graded relevance,Test collection},
pages = {1043--1052},
title = {{Evaluating diversified search results using per-intent graded relevance}},
year = {2011}
}
@article{Swanson2015,
abstract = {Online forums are now one of the primary venues for public dialogue on current social and political issues. The related corpora are often huge, covering any topic imaginable. Our aim is to use these dialogue corpora to automatically discover the semantic aspects of arguments that conversants are making across multiple dialogues on a topic. We frame this goal as consisting of two tasks: argument extraction and argument facet similarity. We focus here on the argument extraction task, and show that we can train regressors to predict the quality of extracted arguments with RRSE values as low as .73 for some topics. A secondary goal is to develop regressors that are topic independent: we report results of cross-domain training and domain-adaptation with RRSE values for several topics as low as .72, when trained on topic independent features.},
author = {Swanson, Reid and Ecker, Brian and Walker, Marilyn},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Swanson, Ecker, Walker - 2015 - Argument mining Extracting arguments from online dialogue.pdf:pdf},
isbn = {9781941643754},
journal = {SIGDIAL 2015 - 16th Annu. Meet. Spec. Interes. Gr. Discourse Dialogue, Proc. Conf.},
number = {September},
pages = {217--226},
title = {{Argument mining: Extracting arguments from online dialogue}},
year = {2015}
}
@article{Bansal2016,
abstract = {Research and business practice have already established the central role of trust in business, particularly in online interactions. Many online business exchanges require the disclosure of sensitive personal information on a regular basis. Simultaneously, customers are reluctant to disclose private information online due to concerns about privacy. Thus, trust plays a critical role in such disclosures. However, a number of factors could influence the extent of customers' trust and their willingness to disclose their private information. In this study, we explore the critical roles of two sets of factors: the sensitivity of the context within which the private information is disclosed and the customer's personality. Our theory building is based on the contextualization of the theory of reasoned action (TRA-Privacy) and its synthesis with Prospect theory. Our theory argues that context sensitivity as a moderator and individuals' salient attributes in terms of personality types and privacy concern are critical factors impacting trust and the willingness to disclose personal information. Our results indicate that context moderates the parameters and path structure of the trust model and that the influence of personality on privacy concern and trust depends on the nature of the context. Applying these "who" and "where" aspects of theory building, the study opens a new avenue of context-related research that can further increase the specificity and richness of trust and privacy research. The study also provides a new perspective in trust scholarship, therein requiring the examination of three inter-related components: trustee, trustor and the context of trust.},
annote = {this study is on the influence of personality and context on disclosing personal information online; so not exactly the more closed group recommender scenario but similar enough; they relate privacy to trust here, whereas we relate it to transparency

basically they establish that both personality and context influence the privacy decisions of people

interesting in there is the notion of context sensitivity; that is some situations are more sensitive than others and people are more / less willing to share information... we could simply look at the influence of different contextual factors on context sensitivity

drawbacks:
- unclear whether the Big 5 test they used is valid},
author = {Bansal, Gaurav and Zahedi, Fatemeh Mariam and Gefen, David},
doi = {10.1016/j.im.2015.08.001},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Bansal, Zahedi, Gefen - 2016 - Do context and personality matter Trust and privacy concerns in disclosing private information online.pdf:pdf},
issn = {03787206},
journal = {Inf. Manag.},
keywords = {Context sensitivity,Personality,Privacy,Prospect theory,TRA-Privacy,Theory of reasoned action,Trust},
number = {1},
pages = {1--21},
publisher = {Elsevier B.V.},
title = {{Do context and personality matter? Trust and privacy concerns in disclosing private information online}},
url = {http://dx.doi.org/10.1016/j.im.2015.08.001},
volume = {53},
year = {2016}
}
@article{Kanoulas2009,
abstract = {The nDCG measure has proven to be a popular measure of retrieval effectiveness utilizing graded relevance judgments. However, a number of different instantiations of nDCG exist, depending on the arbitrary definition of the gain and discount functions used (1) to dictate the relative value of documents of different relevance grades and (2) to weight the importance of gain values at different ranks, respectively. In this work we discuss how to empirically derive a gain and discount function that optimizes the efficiency or stability of nDCG. First, we describe a variance decomposition analysis framework and an optimization procedure utilized to find the efficiency- or stability-optimal gain and discount functions. Then we use TREC data sets to compare the optimal gain and discount functions to the ones that have appeared in the IR literature with respect to (a) the efficiency of the evaluation, (b) the induced ranking of systems, and (c) the discriminative power of the resulting nDCG measure. Copyright 2009 ACM.},
author = {Kanoulas, Evangelos and Aslam, Javed A.},
doi = {10.1145/1645953.1646032},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Kanoulas, Aslam - 2009 - Empirical justification of the gain and discount function for nDCG.pdf:pdf},
isbn = {9781605585123},
journal = {Int. Conf. Inf. Knowl. Manag. Proc.},
keywords = {Evaluation,Generalizability theory,nDCG},
pages = {611--620},
title = {{Empirical justification of the gain and discount function for nDCG}},
year = {2009}
}
@article{Gevelber2016,
author = {Gevelber, Lisa},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Gevelber - 2016 - How Mobile Has Changed How People Get Things Done New Consumer Behavior Data.pdf:pdf},
journal = {Think with Google},
pages = {1--6},
title = {{How Mobile Has Changed How People Get Things Done : New Consumer Behavior Data}},
url = {https://think.storage.googleapis.com/docs/mobile-search-consumer-behavior-data.pdf},
year = {2016}
}
@article{Sarafoglou2018,
abstract = {Current developments in the statistics community suggest that modern statistics education should be structured holistically, i.e., by allowing students to work with real data and answer concrete statistical questions, but also by educating them about alternative statistical frameworks, such as Bayesian statistics. In this article, we describe how we incorporated such a holistic structure in a Bayesian thesis project on ordered binomial probabilities. The project was targeted at undergraduate students in psychology with basic knowledge in Bayesian statistics and programming, but no formal mathematical training. The thesis project aimed to (1) convey the basic mathematical concepts of Bayesian inference, (2) let students experience the entire empirical cycle including the collection, analysis, and interpretation of data, and (3) teach students open science practices.},
archivePrefix = {arXiv},
arxivId = {1810.07496},
author = {Sarafoglou, Alexandra and van der Heijden, Anna and Draws, Tim and Cornelisse, Joran and Wagenmakers, Eric-Jan and Marsman, Maarten},
eprint = {1810.07496},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sarafoglou et al. - 2018 - Combine Statistical Thinking With Scientific Practice A Protocol of a Bayesian Thesis Project For Undergradua.pdf:pdf},
title = {{Combine Statistical Thinking With Scientific Practice: A Protocol of a Bayesian Thesis Project For Undergraduate Students}},
url = {https://arxiv.org/abs/1810.07496{\%}0Ahttp://arxiv.org/abs/1810.07496},
year = {2018}
}
@article{Kunaver2017,
abstract = {Diversification has become one of the leading topics of recommender system research not only as a way to solve the over-fitting problem but also an approach to increasing the quality of the user's experience with the recommender system. This article aims to provide an overview of research done on this topic from one of the first mentions of diversity in 2001 until now. The articles, and research, have been divided into three sub-topics for a better overview of the work done in the field of recommendation diversification: the definition and evaluation of diversity; the impact of diversification on the quality of recommendation results and the development of diversification algorithms themselves. In this way, the article aims both to offer a good overview to a researcher looking for the state-of-the-art on this topic and to help a new developer get familiar with the topic.},
author = {Kunaver, Matev{\v{z}} and Po{\v{z}}rl, Toma{\v{z}}},
doi = {10.1016/j.knosys.2017.02.009},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Kunaver, Po{\v{z}}rl - 2017 - Diversity in recommender systems – A survey.pdf:pdf},
issn = {09507051},
journal = {Knowledge-Based Syst.},
keywords = {Diversity,Personalization,Recommender system,Survey},
pages = {154--162},
title = {{Diversity in recommender systems – A survey}},
volume = {123},
year = {2017}
}
@article{Markus2010,
abstract = {Americans live in a political, social, and historical context that values personal freedom and choice above all else, an emphasis that has been amplified by con- temporary psychology. However, this article reviews research that shows that in non-Western cultures and among working-class Westerners, freedom and choice do not have the meaning or importance they do for the university-educated people who have been the subjects of almost all research on this topic.Wecannot assume that choice, as understood by educated, affluent Westerners, is a universal as- piration. The meaning and significance of choice are cultural constructions. More- over, even when choice can foster freedom, empowerment, and independence, it is not an unalloyed good. Too much choice can produce a paralyzing uncertainty, depression, and selfishness. In the United States, the path to well-being may re- quire that we strike a balance between the positive and negative consequences of proliferating choice in every domain of life.},
annote = {this is a nice review on the topic of choice in relation to human well-being; only read the abstract so far, but this will be useful for background on info overload

it explains how educated westerners are now obsessed with increasing their potential choices as much as possible, while for less educated people and non-Westerners, having many choices is mostly not a desired state -- however, most of the research subjects in this area are educated Westerners

it also explains how information overload can introduce a paralyzing uncertainty, where people are eventually less happy with their choices},
author = {Markus, Hazel Rose and Schwartz, Barry},
doi = {10.1086/651242},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Markus, Schwartz - 2010 - Does Choice Mean Freedom and Well-Being.pdf:pdf},
issn = {0093-5301},
journal = {J. Consum. Res.},
number = {2},
pages = {344--355},
title = {{Does Choice Mean Freedom and Well-Being?}},
volume = {37},
year = {2010}
}
@article{Agrawal2009,
abstract = {We study the problem of answering ambiguous web queries in a setting where there exists a taxonomy of information, and that both queries and documents may belong to more than one category according to this taxonomy. We present a systematic approach to diversifying results that aims to minimize the risk of dissatisfaction of the average user. We propose an algorithm that well approximates this objective in general, and is provably optimal for a natural special case. Furthermore, we generalize several classical IR metrics, including NDCG, MRR, and MAP, to explicitly account for the value of diversification. We demonstrate empirically that our algorithm scores higher in these generalized metrics compared to results produced by commercial search engines.},
annote = {the aim of this group of measures is to deal with ambiguous keywords in IR; increasing diversity will decrease the risk of a failure to satisfy the user

$\backslash$citeA{\{}Agrawal2009{\}} introduce a group of $\backslash$emph{\{}intent-aware{\}} metrics. The authors define the diversification problem as follows: given a search query {\$}q{\$}, a set of documents {\$}D{\$}, a probability distribution of categories for the query {\$}P(c|q){\$}, the quality values of the documents {\$}V(d|q,c){\$}, the aim is to find a set of documents {\$}S \backslashsubseteq D{\$} that maximizes

$\backslash$begin{\{}equation{\}}
P(S|q) = $\backslash$sum{\_}c P(c|q)(1 - $\backslash$prod(1 - V(d|q,c))).
$\backslash$end{\{}equation{\}}

$\backslash$noindent Here, the document categories correspond to the different intents a user might have when entering a query. {\$}(1 - V(d|q,c){\$} is the probability that {\$}d{\$} does not satisfy the user. Subtracting the product of all of these values from 1 gives the probability that at least one of the documents will satisfy category {\$}c{\$} for query {\$}q{\$}. The authors obtain this probability by inserting a classical IR evaluation metric such as NDCG, MRR, or MAP. For instance, the formula for intent-aware NDCG given a search result set of documents {\$}Q{\$} and a rank threshold {\$}k{\$} is

$\backslash$begin{\{}equation{\}}
NDCG-IA(Q,k) = $\backslash$sum{\_}c P(c|q)NDCG(Q,k|c).
$\backslash$end{\{}equation{\}}

$\backslash$noindent The NDCG is computed for each category that corresponds to the query, multiplied by the probability distribution of categories, and subsequently summed up. This way, a trade-off between relevance and category diversity is forced. A drawback with this approach seems to be that since queries can have different numbers of categories, results are not comparable across queries. Furthermore, in order to calculate this metric the category and user evaluation of every document in the list of results have to be known.$\backslash$footnote{\{}Thought: I could adapt this metric to replace {\$}P(c|q){\$} -- the probability distribution of categories -- with the distribution of viewpoints that the articles correspond to.{\}}},
author = {Agrawal, Rakesh and Gollapudi, Sreenivas and Halverson, Alan and Ieong, Samuel},
doi = {10.1145/1498759.1498766},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Agrawal et al. - 2009 - Diversifying search results.pdf:pdf},
isbn = {9781605583907},
journal = {Proc. 2nd ACM Int. Conf. Web Search Data Mining, WSDM'09},
keywords = {Marginal utility,Relevance,Result diversification},
pages = {5--14},
title = {{Diversifying search results}},
year = {2009}
}
@article{Halevy2016,
abstract = {Enterprises increasingly rely on structured datasets to run their businesses. These datasets take a variety of forms, such as structured files, databases, spreadsheets, or even services that provide access to the data. The datasets often reside in different storage systems, may vary in their formats, may change every day. In this paper, we present Goods, a project to rethink how we organize structured datasets at scale, in a setting where teams use diverse and often idiosyncratic ways to produce the datasets and where there is no centralized system for storing and querying them. Goods extracts metadata ranging from salient information about each dataset (owners, timestamps, schema) to relationships among datasets, such as similarity and provenance. It then exposes this metadata through services that allow engineers to find datasets within the company, to monitor datasets, to annotate them in order to enable others to use their datasets, and to analyze relationships between them. We discuss the technical challenges that we had to overcome in order to crawl and infer the metadata for billions of datasets, to maintain the consistency of our metadata catalog at scale, and to expose the metadata to users. We believe that many of the lessons that we learned are applicable to building large-scale enterprise-level data-management systems in general.},
author = {Halevy, Alon and Korn, Flip and Noy, Natalya F. and Olston, Christopher and Polyzotis, Neoklis and Roy, Sudip and Whang, Steven Euijong},
doi = {10.1145/2882903.2903730},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Halevy et al. - 2016 - Goods Organizing Google's datasets.pdf:pdf},
isbn = {9781450335317},
issn = {07308078},
journal = {Proc. ACM SIGMOD Int. Conf. Manag. Data},
pages = {795--806},
title = {{Goods: Organizing Google's datasets}},
volume = {26-June-20},
year = {2016}
}
@article{hodson2014ai,
author = {Hodson, Hal},
journal = {New Sci.},
title = {{The AI boss that deploys Hong Kong's subway engineers}},
url = {https://www.newscientist.com/article/mg22329764-000-the-ai-boss-that-deploys-hong-kongs-subway-engineers/},
year = {2014}
}
@article{Onkal2009,
abstract = {Decision makers and forecasters often receive advice from different sources including human experts and statistical methods. This research examines, in the context of stock price forecasting, how the apparent source of the advice affects the attention that is paid to it when the mode of delivery of the advice is identical for both sources. In Study 1, two groups of participants were given the same advised point and interval forecasts. One group was told that these were the advice of a human expert and the other that they were generated by a statistical forecasting method. The participants were then asked to adjust forecasts they had previously made in light of this advice. While in both cases the advice led to improved point forecast accuracy and better calibration of the prediction intervals, the advice which apparently emanated from a statistical method was discounted much more severely. In Study 2, participants were provided with advice from two sources. When the participants were told that both sources were either human experts or both were statistical methods, the apparent statistical-based advice had the same influence on the adjusted estimates as the advice that appeared to come from a human expert. However when the apparent sources of advice were different, much greater attention was paid to the advice that apparently came from a human expert. Theories of advice utilization are used to identify why the advice of a human expert is likely to be preferred to advice from a statistical method. {\textcopyright} 2009 John Wiley {\&} Sons, Ltd.},
author = {{\"{O}}nkal, Dilek and Goodwin, Paul and Thomson, Mary and G{\"{o}}n{\"{u}}l, Sinan and Pollock, Andrew},
doi = {10.1002/bdm.637},
issn = {10990771},
journal = {J. Behav. Decis. Mak.},
keywords = {Advice,Advice utilization,Forecast adjustment,Forecasting,Role of experts,Source framing},
number = {4},
pages = {390--409},
publisher = {John Wiley and Sons Ltd},
title = {{The relative influence of advice from human experts and statistical methods on forecast adjustments}},
volume = {22},
year = {2009}
}
@article{Toreini2020,
abstract = {To design and develop AI-based systems that users and the larger public can justifiably trust, one needs to understand how machine learning technologies impact trust. To guide the design and implementation of trusted AI-based systems, this paper provides a systematic approach to relate considerations about trust from the social sciences to trustworthiness technologies proposed for AI-based services and products. We start from the ABI+ (Ability, Benevolence, Integrity, Predictability) framework augmented with a recently proposed mapping of ABI+ on qualities of technologies that support trust. We consider four categories of trustworthiness technologies for machine learning, namely these for Fairness, Explainability, Auditability and Safety (FEAS) and discuss if and how these support the required qualities. Moreover, trust can be impacted throughout the life cycle of AI-based systems, and we therefore introduce the concept of Chain of Trust to discuss trustworthiness technologies in all stages of the life cycle. In so doing we establish the ways in which machine learning technologies support trusted AI-based systems. Finally, FEAS has obvious relations with known frameworks and therefore we relate FEAS to a variety of international 'principled AI' policy and technology frameworks that have emerged in recent years.},
archivePrefix = {arXiv},
arxivId = {1912.00782},
author = {Toreini, Ehsan and Aitken, Mhairi and Coopamootoo, Kovila and Elliott, Karen and Zelaya, Carlos Gonzalez and van Moorsel, Aad},
doi = {10.1145/3351095.3372834},
eprint = {1912.00782},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Toreini et al. - 2020 - The relationship between trust in AI and trustworthy machine learning technologies.pdf:pdf},
isbn = {9781450369367},
journal = {FAT* 2020 - Proc. 2020 Conf. Fairness, Accountability, Transpar.},
keywords = {Artificial intelligence,Machine learning,Trust,Trustworthiness},
pages = {272--283},
title = {{The relationship between trust in AI and trustworthy machine learning technologies}},
year = {2020}
}
@inproceedings{Pogacar2017,
abstract = {{\textcopyright} 2017 Copyright held by the owner/author(s). People regularly use web search engines to investigate the efficacy of medical treatments. Search results can contain documents that present incorrect information that contradicts current established medical understanding on whether a treatment is helpful or not for a health issue. If people are influenced by the incorrect information found in search results, they can make harmful decisions about the appropriate treatment. To determine the extent to which people can be influenced by search engine results, we conducted a controlled laboratory study that biased search results towards correct or incorrect information for 10 different medical treatments. We found that search engine results can significantly influence people both positively and negatively. Importantly, study participants made more incorrect decisions when they interacted with search results biased towards incorrect information than when they had no interaction with search results at all. For search domains such as health information, search engine designers and researchers must recognize that not all non-relevant information is the same. Some non-relevant information is incorrect and potentially harmful when people use it to make decisions that may negatively impact their lives.},
address = {New York, NY, USA},
annote = {(no minimum amount of time exploring the SERP)},
author = {Pogacar, Frances A. and Ghenai, Amira and Smucker, Mark D. and Clarke, Charles L.A.},
booktitle = {Proc. ACM SIGIR Int. Conf. Theory Inf. Retr.},
doi = {10.1145/3121050.3121074},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Pogacar et al. - 2017 - The Positive and Negative Influence of Search Results on People's Decisions about the Efficacy of Medical Trea.pdf:pdf},
isbn = {9781450344906},
keywords = {Harmful Effects,Health Search,Misinformation,User Study},
pages = {209--216},
publisher = {Association for Computing Machinery},
series = {ICTIR '17},
title = {{The Positive and Negative Influence of Search Results on People's Decisions about the Efficacy of Medical Treatments}},
year = {2017}
}
@article{Kang2018,
abstract = {With the rapid growth of social media, text mining is extensively utilized in practical fields, and opinion mining, also known as sentiment analysis, plays an important role in analyzing opinion and sentiment in texts. Methods in opinion mining generally depend on a sentiment lexicon, which is a set of predefined key words that express sentiment. Opinion mining requires proper sentiment words to be extracted in advance and has difficulty classifying sentences that imply an opinion without using any sentiment key words. This paper presents a new sentiment analysis method, based on text-based hidden Markov models (TextHMMs), for text classification that uses a sequence of words in training texts instead of a predefined sentiment lexicon. We sought to learn text patterns representing sentiment through ensemble TextHMMs. Our method defines hidden variables in TextHMMs by semantic cluster information in consideration of the co-occurrence of words, and thus calculates the sentiment orientation of sentences by fitted TextHMMs. To reflect diverse patterns, we applied an ensemble of TextHMM-based classifiers. In the experiments with a benchmark data set, we show that this method is superior to some existing methods and particularly has potential to classify implicit opinions. We also demonstrate the practicality of the proposed method in a real-life data set of online market reviews.},
author = {Kang, Mangi and Ahn, Jaelim and Lee, Kichun},
doi = {10.1016/j.eswa.2017.07.019},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Kang, Ahn, Lee - 2018 - Opinion mining using ensemble text hidden Markov models for text classification.pdf:pdf},
issn = {09574174},
journal = {Expert Syst. Appl.},
keywords = {Boosting,Clustering,Ensemble,Hidden Markov models,Opinion mining,Sentiment analysis},
pages = {218--227},
publisher = {Elsevier Ltd},
title = {{Opinion mining using ensemble text hidden Markov models for text classification}},
volume = {94},
year = {2018}
}
@article{Das2019,
abstract = {While search efficacy has been evaluated traditionally on the basis of result relevance, fairness of search has attracted recent attention. In this work, we define a notion of distributional fairness and provide a conceptual framework for evaluating search results based on it. As part of this, we formulate a set of axioms which an ideal evaluation framework should satisfy for distributional fairness. We show how existing TREC test collections can be repurposed to study fairness, and we measure potential data bias to inform test collection design for fair search. A set of analyses show metric divergence between relevance and fairness, and we describe a simple but flexible interpolation strategy for integrating relevance and fairness into a single metric for optimization and evaluation.},
annote = {this is a theoretical framework on how to evaluate fairness in search; specifically distributional fairness (which is what I want to do)

they argue one should define a target distribution (e.g. uniform) and compare that to the results distribution

very nice examples show that we can basically start with the fairness metrics on already existing TREC data sets!},
archivePrefix = {arXiv},
arxivId = {1907.09328},
author = {Das, Anubrata and Lease, Matthew},
eprint = {1907.09328},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Das, Lease - 2019 - A Conceptual Framework for Evaluating Fairness in Search.pdf:pdf},
journal = {arXiv Prepr. arXiv1907.09328},
keywords = {14,19,5,and,and racial,application areas such as,evaluation,fairness,inequality,information retrieval,ir systems face existing,resume-search,societal bias,such as gender},
title = {{A Conceptual Framework for Evaluating Fairness in Search}},
year = {2019}
}
@article{Alheneidi2019,
abstract = {We are living in an information age, where the overabundance of information can result in stressful conditions for information users, such as information overload. This might lead to internet addiction or problematic internet use, because the internet is the most used information source and can be addictive or misused due to its evolving and endless content and activities. An individual can face difficulties in understanding an issue or making a decision because of the presence of too much information, like the flow of instant messages, text messages, phone calls, emails, social network notifications, advertisements, as well as non-cyber based information sources. This flood of information we are being exposed to can result in negative consequences for individual wellbeing. This mixed methods study investigated the impact of information overload and internet addiction on adults' psychological wellbeing, work performance and academic attainment. Five empirical studies were used to measure the influence of information overload and internet addiction on wellbeing through a holistic approach. These studies also controlled possible factors that could influence or interfere with the wellbeing process. The results revealed interesting findings: The influence of information overload and internet addiction on university students' predicted negative wellbeing, and the cultural differences between Kuwait and UK sample were not significant. However, the influence of information overload and internet addiction was significantly different between students and workers. The impact of different internet uses on workers were also significantly different than students. The diary study revealed significant differences between problematic internet users and non-problematic internet users' wellbeing scores, although hours spent on the internet and internet activities were similar. The thesis provides a comprehensive approach to understanding the influence of information overload and internet addiction on adults' wellbeing, which can provide intervention plans and solutions in universities and workplaces.},
author = {Alheneidi, Hasah H.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Alheneidi - 2019 - The influence of information overload and problematic Internet use on adults wellbeing.pdf:pdf},
title = {{The influence of information overload and problematic Internet use on adults wellbeing}},
year = {2019}
}
@article{Wagenmakers2018,
abstract = {Bayesian parameter estimation and Bayesian hypothesis testing present attractive alternatives to classical inference using confidence intervals and p values. In part I of this series we outline ten prominent advantages of the Bayesian approach. Many of these advantages translate to concrete opportunities for pragmatic researchers. For instance, Bayesian hypothesis testing allows researchers to quantify evidence and monitor its progression as data come in, without needing to know the intention with which the data were collected. We end by countering several objections to Bayesian hypothesis testing. Part II of this series discusses JASP, a free and open source software program that makes it easy to conduct Bayesian estimation and testing for a range of popular statistical scenarios (Wagenmakers et al. this issue).},
author = {Wagenmakers, Eric Jan and Marsman, Maarten and Jamil, Tahira and Ly, Alexander and Verhagen, Josine and Love, Jonathon and Selker, Ravi and Gronau, Quentin F. and {\v{S}}m{\'{i}}ra, Martin and Epskamp, Sacha and Matzke, Dora and Rouder, Jeffrey N. and Morey, Richard D.},
doi = {10.3758/s13423-017-1343-3},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Wagenmakers et al. - 2018 - Bayesian inference for psychology. Part I Theoretical advantages and practical ramifications.pdf:pdf},
issn = {15315320},
journal = {Psychon. Bull. Rev.},
keywords = {Bayes factor,Hypothesis test,Posterior distribution,Statistical evidence},
number = {1},
pages = {35--57},
pmid = {28779455},
title = {{Bayesian inference for psychology. Part I: Theoretical advantages and practical ramifications}},
volume = {25},
year = {2018}
}
@article{carey2016companies,
author = {{Carey, Dennis and Smith}, Matt},
journal = {Harv. Bus. Rev.},
title = {{How companies are using simulations, competitions, and analytics to hire}},
url = {https://hbr.org/2016/04/how-companies-are-using-simulations-competitions-and-analytics-to-hire},
year = {2016}
}
@article{Gordon2013,
abstract = {Much work in knowledge extraction from text tacitly assumes that the frequency with which people write about actions, outcomes, or properties is a reflection of real-world frequencies or the degree to which a property is characteristic of a class of individuals. In this paper, we question this idea, examining the phenomenon of reporting bias and the challenge it poses for knowledge extraction. We conclude with discussion of approaches to learning commonsense knowledge from text despite this distortion.},
author = {Gordon, Jonathan and {Van Durme}, Benjamin},
doi = {10.1145/2509558.2509563},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Gordon, Van Durme - 2013 - Reporting bias and knowledge acquisition.pdf:pdf},
isbn = {9781450324113},
journal = {AKBC 2013 - Proc. 2013 Work. Autom. Knowl. Base Constr. Co-located with CIKM 2013},
keywords = {knowledge extraction,reporting bias,text frequency},
number = {circa},
pages = {25--29},
title = {{Reporting bias and knowledge acquisition}},
year = {2013}
}
@article{Stevens2012,
abstract = {We apply two new automated semantic eval- uations to three distinct latent topic models. Both metrics have been shown to align with human evaluations and provide a balance be- tween internal measures of information gain and comparisons to human ratings of coher- ent topics. We improve upon the measures by introducing new aggregate measures that allows for comparing complete topic models. We further compare the automated measures to other metrics for topic models, compar- ison to manually crafted semantic tests and document classification. Our experiments re- veal that LDA and LSA each have different strengths; LDA best learns descriptive topics while LSA is best at creating a compact se- mantic representation of documents and words in a corpus.},
author = {Stevens, Keith and Kegelmeyer, Philip and Andrzejewski, David and Buttler, David},
doi = {10.5694/j.1326-5377.1993.tb137878.x},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Stevens et al. - 2012 - Exploring Topic Coherence over many models and many topics.pdf:pdf},
issn = {0025729X},
journal = {Proc. 2012 Jt. Conf. Empir. Methods Nat. Lang. Process. Comput. Nat. Lang. Learn.},
pages = {952--961},
title = {{Exploring Topic Coherence over many models and many topics}},
year = {2012}
}
@article{Haran2013,
abstract = {Errors in estimating and forecasting often result from the failure to collect and consider enough relevant information. We examine whether attributes associated with persistence in information acquisition can predict performance in an estimation task. We focus on actively open-minded thinking (AOT), need for cognition, grit, and the tendency to maximize or satisfice when making decisions. In three studies, participants made estimates and predictions of uncertain quantities, with varying levels of control over the amount of information they could collect before estimating. Only AOT predicted performance. This relationship was mediated by information acquisition: AOT predicted the tendency to collect information, and information acquisition predicted performance. To the extent that available information is predictive of future outcomes, actively open-minded thinkers are more likely than others to make accurate forecasts. {\textcopyright} 2013. The authors license this article under the terms of the Creative Commons Attribution 3.0 License.},
author = {Haran, Uriel and Ritov, Ilana and Mellers, Barbara A.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Haran, Ritov, Mellers - 2013 - The role of actively open-minded thinking in information acquisition, accuracy, and calibration.pdf:pdf},
issn = {19302975},
journal = {Judgm. Decis. Mak.},
keywords = {Actively open-minded thinking,Calibration,Forecasting,Individual differences,Overconfidence,Prediction},
number = {3},
pages = {188--201},
title = {{The role of actively open-minded thinking in information acquisition, accuracy, and calibration}},
volume = {8},
year = {2013}
}
@article{Abid2015,
abstract = {The quantity of information placed on the web has been greater than before and is increasing rapidly day by day. Searching through the huge amount of data and finding the most relevant and useful result set involves searching, ranking, and presenting the results. Most of the users probe into the top few results and neglect the rest. In order to increase user's satisfaction, the presented result set should not only be relevant to the search topic, but should also present a variety of perspectives, that is, the results should be different from one another. The effectiveness of web search and the satisfaction of users can be enhanced through providing various results of a search query in a certain order of relevance and concern. The technique used to avoid presenting similar, though relevant, results to the user is known as a diversification of search results. This article presents a survey of the approaches used for search result diversification. To this end, this article not only provides a technical survey of existing diversification techniques, but also presents a taxonomy of diversification algorithms with respect to the types of search queries.},
author = {Abid, Adnan and Hussain, Naveed and Abid, Kamran and Ahmad, Farooq and Farooq, Muhammad Shoaib and Farooq, Uzma and Khan, Sher Afzal and Khan, Yaser Daanial and Naeem, Muhammad Azhar and Sabir, Nabeel},
doi = {10.1007/s00521-015-1945-5},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Abid et al. - 2015 - A survey on search results diversification techniques.pdf:pdf},
isbn = {0052101519455},
issn = {09410643},
journal = {Neural Comput. Appl.},
keywords = {Diversification of search results,Diversification techniques,Web search},
number = {5},
pages = {1207--1229},
publisher = {Springer London},
title = {{A survey on search results diversification techniques}},
volume = {27},
year = {2015}
}
@article{Zhang2016,
abstract = {There are multiple sides to every story, and while statistical topic models have been highly successful at topically summarizing the stories in corpora of text documents, they do not explicitly address the issue of learning the different sides, the viewpoints, expressed in the documents. In this paper, we show how these viewpoints can be learned completely unsupervised and represented in a human interpretable form. We use a novel approach of applying CorrLDA2 for this purpose, which learns topic-viewpoint relations that can be used to form groups of topics, where each group represents a viewpoint. A corpus of documents about the Israeli-Palestinian conflict is then used to demonstrate how a Palestinian and an Israeli viewpoint can be learned. By leveraging the magnitudes and signs of the feature weights of a linear SVM, we introduce a principled method to evaluate associations between topics and viewpoints. With this, we demonstrate, both quantitatively and qualitatively, that the learned topic groups are contextually coherent, and form consistently correct topic-viewpoint associations.},
annote = {in this paper, they try to figure out on which side of a controversial topic an author of a text document stands; using the example of a data set containing articles about the israeli - palestine conflict

limitations of this paper:

- they conflate stance and viewpoint, and they actually only measure stance
- they regard controversial topics as bimodal (essentially looking at all topics in terms of agree / disagree); which is not useful if we want to model a variety of viewpoints

basically they only cover the first layer of the hierarchy; they don't touch the reasons behind the sentiment, or assume them to be the same across documents within the same opinion group},
archivePrefix = {arXiv},
arxivId = {1608.04089},
author = {Zhang, Kerry and Karlgren, Jussi and Zhang, Cheng and Lagergren, Jens},
eprint = {1608.04089},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Zhang et al. - 2016 - Viewpoint and Topic Modeling of Current Events.pdf:pdf},
pages = {1--16},
title = {{Viewpoint and Topic Modeling of Current Events}},
url = {http://arxiv.org/abs/1608.04089},
year = {2016}
}
@article{VanDoorn2019,
abstract = {Despite the increasing popularity of Bayesian inference in empirical research, few practical guidelines provide detailed refile:///Users/tim/Documents/Academia/Papers with my name on them/BayesianGuidelinesFinal(2).pdfcommendations for how to apply Bayesian procedures and interpret the results. Here we offer specific guidelines for four different stages of Bayesian statistical reasoning in a research setting: planning the analysis, executing the analysis, interpreting the results, and reporting the results. The guidelines for each stage are illustrated with a running example. Although the guidelines are geared toward analyses performed with the open-source statistical software JASP, most guidelines extend to Bayesian inference in general.},
archivePrefix = {arXiv},
arxivId = {10.31234/osf.io/yqxfr},
author = {van Doorn, Johnny and van den Bergh, Don and Bohm, Udo and Dablander, Fabian and Derks, Koen and Draws, Tim and Evans, Nathan J and Gronau, Quentin Frederik and Hinne, Max and Kucharsk{\'{y}}, {\v{S}}imon and Ly, Alexander and Marsman, Maarten and Matzke, Dora and Raj, Akash and Sarafoglou, Alexandra and Stefan, Angelika and Voelkel, Jan G and Wagenmakers, Eric-Jan},
doi = {10.31234/osf.io/yqxfr},
eprint = {osf.io/yqxfr},
file = {:Users/tim/Surfdrive/Research/Library/Literature/van Doorn et al. - 2019 - The JASP Guidelines for Conducting and Reporting a Bayesian Analysis.pdf:pdf},
journal = {PsyArxiv Prepr.},
number = {February},
pages = {0--31},
primaryClass = {10.31234},
title = {{The JASP Guidelines for Conducting and Reporting a Bayesian Analysis}},
url = {https://osf.io/yqxfr},
year = {2019}
}
@article{Baden2014,
abstract = {Does news users' commentary contribute to widening the diversity of viewpoints represented in the news? This article comparatively analyses the interpretations of the current financial crisis in the online coverage of five German newspapers and the subsequent commentary of news users. Using an innovative strategy to identify the interpretative repertoires constructed by news and user frames, it assesses how user commentary deviates from those viewpoints represented in the news. Findings show that user accounts mostly remain within the wider interpretative repertoires offered by the media. However, they utilize media frame fragments rather freely to construct their own views, shifting focus and elaborating upon new aspects. While no consistent alternative repertoires were constructed, users thus valuably complemented the diversity of concerns discussed on news websites.},
author = {Baden, Christian and Springer, Nina},
doi = {10.1177/0267323114538724},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Baden, Springer - 2014 - Com(ple)menting the news on the financial crisis The contribution of news users' commentary to the diversity.pdf:pdf},
issn = {14603705},
journal = {Eur. J. Commun.},
keywords = {Audience research,content analysis,journalism,news/information,political communication,semiology/language/discourse},
number = {5},
pages = {529--548},
title = {{Com(ple)menting the news on the financial crisis: The contribution of news users' commentary to the diversity of viewpoints in the public debate}},
volume = {29},
year = {2014}
}
@article{VanDenBergh2020,
abstract = {Analysis of variance (ANOVA) is the standard procedure for statistical inference in factorial designs. Typically, ANOVAs are executed using frequentist statistics, where p-values determine statistical significance in an all-or-none fashion. In recent years, the Bayesian approach to statistics is increasingly viewed as a legitimate alternative to the p-value. However, the broad adoption of Bayesian statistics-and Bayesian ANOVA in particular-is frustrated by the fact that Bayesian concepts are rarely taught in applied statistics courses. Consequently, practitioners may be unsure how to conduct a Bayesian ANOVA and interpret the results. Here we provide a guide for executing and interpreting a Bayesian ANOVA with JASP, an open-source statistical software program with a graphical user interface. We explain the key concepts of the Bayesian ANOVA using two empirical examples.},
author = {{Van Den Bergh}, Don and {Van Doorn}, Johnny and Marsman, Maarten and Draws, Tim and {Van Kesteren}, Erik Jan and Derks, Koen and Dablander, Fabian and Gronau, Quentin F. and Kucharsk{\'{y}}, {\v{S}}imon and Gupta, Akash R.Komarlu Narendra and Sarafoglou, Alexandra and Voelkel, Jan G. and Stefan, Angelika and Ly, Alexander and Hinne, Max and Matzke, Dora and Wagenmakers, Eric Jan},
doi = {10.3917/anpsy1.201.0073},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Van Den Bergh et al. - 2020 - A tutorial on conducting and interpreting a bayesian ANOVA in JASP.pdf:pdf},
isbn = {9782130822936},
issn = {00035033},
journal = {Annee Psychol.},
keywords = {Analysis of Variance,Bayes Factor,Hypothesis Test,JASP,Posterior distribution,Tutorial},
number = {1},
pages = {73--96},
title = {{A tutorial on conducting and interpreting a bayesian ANOVA in JASP}},
volume = {120},
year = {2020}
}
@article{Blei2003,
archivePrefix = {arXiv},
arxivId = {1111.6189v1},
author = {Blei, David M and Ng, Andrew Y and Jordan, Michael I},
doi = {10.1162/jmlr.2003.3.4-5.993},
eprint = {1111.6189v1},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Blei, Ng, Jordan - 2003 - Latent Dirichlet Allocation.pdf:pdf},
isbn = {9781577352815},
issn = {0003-6951},
pages = {993--1022},
pmid = {21362469},
title = {{Latent Dirichlet Allocation}},
volume = {3},
year = {2003}
}
@article{Wagenmakers2011,
abstract = {Does psi exist? D. J. Bem (2011) conducted 9 studies with over 1,000 participants in an attempt to demonstrate that future events retroactively affect people's responses. Here we discuss several limitations of Bem's experiments on psi; in particular, we show that the data analysis was partly exploratory and that one-sided p values may overstate the statistical evidence against the null hypothesis. We reanalyze Bem's data with a default Bayesian t test and show that the evidence for psi is weak to nonexistent. We argue that in order to convince a skeptical audience of a controversial claim, one needs to conduct strictly confirmatory studies and analyze the results with statistical tests that are conservative rather than liberal. We conclude that Bem's p values do not indicate evidence in favor of precognition; instead, they indicate that experimental psychologists need to change the way they conduct their experiments and analyze their data. {\textcopyright} 2011 American Psychological Association.},
author = {Wagenmakers, Eric Jan and Wetzels, Ruud and Borsboom, Denny and van der Maas, Han L.J.},
doi = {10.1037/a0022790},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Wagenmakers et al. - 2011 - Why Psychologists Must Change the Way They Analyze Their Data The Case of Psi Comment on Bem (2011).pdf:pdf},
issn = {00223514},
journal = {J. Pers. Soc. Psychol.},
keywords = {Bayesian hypothesis test,Confirmatory experiments,ESP},
number = {3},
pages = {426--432},
title = {{Why Psychologists Must Change the Way They Analyze Their Data: The Case of Psi: Comment on Bem (2011)}},
volume = {100},
year = {2011}
}
@article{Niculae2017,
abstract = {We propose a novel factor graph model for argument mining, designed for settings in which the argumentative relations in a document do not necessarily form a tree structure. (This is the case in over 20{\%} of the web comments dataset we release.) Our model jointly learns elementary unit type classification and argumentative relation prediction. Moreover, our model supports SVM and RNN parametrizations, can enforce structure constraints (e.g., transitivity), and can express dependencies between adjacent relations and propositions. Our approaches outperform unstructured baselines in both web comments and argumentative essay datasets.},
archivePrefix = {arXiv},
arxivId = {arXiv:1704.06869v1},
author = {Niculae, Vlad and Park, Joonsuk and Cardie, Claire},
doi = {10.18653/v1/P17-1091},
eprint = {arXiv:1704.06869v1},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Niculae, Park, Cardie - 2017 - Argument mining with structured SVMs and RNNs.pdf:pdf},
isbn = {9781945626753},
journal = {ACL 2017 - 55th Annu. Meet. Assoc. Comput. Linguist. Proc. Conf. (Long Pap.},
pages = {985--995},
title = {{Argument mining with structured SVMs and RNNs}},
volume = {1},
year = {2017}
}
@article{Novin2017,
abstract = {Currently, there is widespread media coverage about the problems with 'fake news' that appears in social media, but the effects of biased information that appears in search engine results is also increasing. The authors argue that the search engine results page (SERP) exposes three important types of bias: source bias, algorithmic bias, and cognitive bias. To explore the relationship between these three types of bias, we conducted a mixed methods study with sixty participants (plus fourteen in a pilot to make a total of seventy-four participants). Within a library setting, participants were provided with mock search engine pages that presented order-controlled sources on a science controversy. Participants were then asked to rank the sources' usefulness and then summarize the controversy. We found that participants ranked the usefulness of sources depending on its presentation within a SERP. In turn, this also influenced how the participants summarized the topic. We attribute the differences in the participants' writings to the cognitive biases that affect a user's judgment when selecting sources on a SERP. We identify four main cognitive biases that a SERP can evoke in students: Priming, Anchoring, Framing, and the Availability Heuristic. While policing information quality is a quixotic task, changes can be made to both SERPs and a user's decision-making when selecting sources. As bias emerges both on the system side and the user side of search, we suggest a two-fold solution is required to address these challenges. Copyright is held by the owner/author(s). Publication rights licensed to ACM.},
annote = {this is about user interaction},
author = {Novin, Alamir and Meyers, Eric},
doi = {10.1145/3020165.3020185},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Novin, Meyers - 2017 - Making sense of conflicting science information Exploring bias in the search engine result page.pdf:pdf},
isbn = {9781450346771},
journal = {CHIIR 2017 - Proc. 2017 Conf. Hum. Inf. Interact. Retr.},
pages = {175--184},
title = {{Making sense of conflicting science information: Exploring bias in the search engine result page}},
year = {2017}
}
@inproceedings{fokkens2017,
author = {Fokkens, Antske and Vossen, Piek and Rospocher, Marco and Hoekstra, Rinke and van Hage, Willem R.},
booktitle = {J. R. Inst. Chem.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Fokkens et al. - 2017 - GRaSP Grounded Representation and Source Perspective.pdf:pdf},
isbn = {9789544520403},
issn = {03683958},
pages = {19--25},
title = {{GRaSP: Grounded Representation and Source Perspective}},
year = {2017}
}
@article{Reis2000,
abstract = {Emotional well-being is most typically studied in trait or trait-like terms, yet a growing literature indicates that daily (within-person) fluctuations in emotional well-being may be equally important. The present research explored the hypothesis that daily variations may be understood in terms of the degree to which three basic needs—autonomy, competence, and related-ness—are satisfied in daily activity. Hierarchical linear models were used to examine this hypothesis across 2 weeks of daily activ-ity and well-being reports controlling for trait-level individual differences. Results strongly supported the hypothesis. The authors also examined the social activities that contribute to sat-isfaction of relatedness needs. The best predictors were meaning-ful talk and feeling understood and appreciated by interaction partners. Finally, the authors found systematic day-of-the-week variations in emotional well-being and need satisfaction. These results are discussed in terms of the importance of daily activities and the need to consider both trait and day-level determinants of well-being.},
author = {Reis, Harry T and Sheldon, Kennon M and Gable, Shelly L and Roscoe, Joseph and Ryan, Richard M},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Reis et al. - 2000 - Daily Well-Being The Role of Autonomy, Competence, and Relatedness.pdf:pdf},
journal = {Pers. Soc. Psychol. Bull.},
number = {4},
pages = {419--435},
title = {{Daily Well-Being: The Role of Autonomy, Competence, and Relatedness}},
volume = {26},
year = {2000}
}
@article{Wehnert2018,
abstract = {Due to the ever-increasing amount of legal regulations, it became an interest of scholars to find ways of capturing domain-relevant knowledge and facilitate the navigation in legal text corpora. Furthermore, the contextual nature of legislation requires enhanced semantic capabilities to identify relevant regulations for specific user needs. This work aims for collecting concept hierarchies from German literature in the legal domain which are then integrated into a knowledge base with multiple clusters, allowing for different perspectives and efficient lookups. Having references to regulations in the leaves of the concept tree and higher levels with an increasingly abstract context, the resulting hierarchies provide the basis for creating legal domain knowledge in German law. Starting with rule-based annotation, we cluster extracted references, given their context features derived from tables of contents and reasons for citing from various textbook formats. We study the expressiveness of the obtained reference context features. Since different authors have their own notion of hierarchy given by the table of contents, we propose a heterogeneous lightweight ontology allowing for the coexistence of similar, yet diverse concept hierarchies to dynamically determine the best fit for a user in a semi-supervised setting. This approach is novel, since state-of-the-art ontologies are conventionally modeled under full integration and in a top-down manner, often not accounting for perspectives in knowledge representation.},
author = {Wehnert, Sabine and Broneske, David and Langer, Stefan and Saake, Gunter},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Wehnert et al. - 2018 - Concept Hierarchy Extraction from Legal Literature.pdf:pdf},
journal = {CEUR Work. Proc. (to Appear.},
keywords = {Legal literatur,Rule-based information extraction,all or part of,concept learn-,ing,legal literature,lightweight ontology,or,or hard copies of,permission to make digital,rule-based information extraction,this work for personal,web knowledge},
number = {October},
title = {{Concept Hierarchy Extraction from Legal Literature}},
year = {2018}
}
@article{Mehrabi2019,
abstract = {With the widespread use of AI systems and applications in our everyday lives, it is important to take fairness issues into consideration while designing and engineering these types of systems. Such systems can be used in many sensitive environments to make important and life-changing decisions; thus, it is crucial to ensure that the decisions do not reflect discriminatory behavior toward certain groups or populations. We have recently seen work in machine learning, natural language processing, and deep learning that addresses such challenges in different subdomains. With the commercialization of these systems, researchers are becoming aware of the biases that these applications can contain and have attempted to address them. In this survey we investigated different real-world applications that have shown biases in various ways, and we listed different sources of biases that can affect AI applications. We then created a taxonomy for fairness definitions that machine learning researchers have defined in order to avoid the existing bias in AI systems. In addition to that, we examined different domains and subdomains in AI showing what researchers have observed with regard to unfair outcomes in the state-of-the-art methods and how they have tried to address them. There are still many future directions and solutions that can be taken to mitigate the problem of bias in AI systems. We are hoping that this survey will motivate researchers to tackle these issues in the near future by observing existing work in their respective fields.},
annote = {lists different types of biases and discusses real world examples},
archivePrefix = {arXiv},
arxivId = {1908.09635},
author = {Mehrabi, Ninareh and Morstatter, Fred and Saxena, Nripsuta and Lerman, Kristina and Galstyan, Aram},
eprint = {1908.09635},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Mehrabi et al. - 2019 - A Survey on Bias and Fairness in Machine Learning.pdf:pdf},
journal = {arXiv Prepr. arXiv1908.09635},
title = {{A Survey on Bias and Fairness in Machine Learning}},
url = {http://arxiv.org/abs/1908.09635},
year = {2019}
}
@article{Bakshi2016,
abstract = {An important part of our information-gathering behavior has always been to find out what other people think. With the growing availability and popularity of opinion-rich resources such as online review sites and personal blogs, new opportunities and challenges arise as people now can, and do, actively use information technologies to seek out and understand the opinions of others. The sudden eruption of activity in the area of opinion mining and sentiment analysis, which deals with the computational treatment of opinion, sentiment, and subjectivity in text, has thus occurred at least in part as a direct response to the surge of interest in new systems that deal directly with opinions as a first-class object. This survey covers techniques and approaches that promise to directly enable opinion-oriented information-seeking systems. Our focus is on methods that seek to address the new challenges raised by sentiment-aware applications, as compared to those that are already present in more traditional fact-based analysis. We include material on summarization of evaluative text and on broader issues regarding privacy, manipulation, and economic impact that the development of opinion-oriented information-access services gives rise to. To facilitate future work, a discussion of available resources, benchmark datasets, and evaluation campaigns is also provided.},
author = {Bakshi, Rushlene Kaur and Kaur, Navneet and Kaur, Ravneet and Kaur, Gurpreet},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Bakshi et al. - 2016 - Opinion mining and sentiment analysis.pdf:pdf},
isbn = {9789380544199},
journal = {Proc. 10th INDIACom; 2016 3rd Int. Conf. Comput. Sustain. Glob. Dev. INDIACom 2016},
keywords = {Micro Blogging,Natural Language Processing,Opinion Mining,Sentiment Analysis,Twitter},
number = {1},
pages = {452--455},
title = {{Opinion mining and sentiment analysis}},
volume = {2},
year = {2016}
}
@article{Mullainathan2012,
abstract = {PURPOSE To investigate the response characteristics of the corneal afferents that detect ocular conditions critical to the activation of the "afferent limb" of the lacrimation reflex. METHODS In isoflurane-anesthetized male rats, trigeminal ganglia were explored extracellularly in vivo to identify the corneal neurons that can be activated by ocular stimuli important to lacrimation. After verifying their receptive field loci to be restricted to the cornea, neural response properties were characterized with a variety of stimuli, such as drying and wetting of the cornea, by applying and removing artificial tears, temperature changes (35 degrees C-15 degrees C and 39 degrees C-51 degrees C), menthol (10-100 microM), and hyperosmolar solutions (NaCl, sucrose; 297-3014 mOsm), applied to the ocular surface. RESULTS A specific type of corneal afferent was identified that responded to drying of the ocular surface. These neurons were classified as innocuous "cold" thermoreceptors by their responses to steady state and dynamic temperature changes applied to the cornea. In addition to drying and slight cooling ({\textless}1 degree C) of the corneal surface, these neurons were excited by evaporation of tears from the ocular surface and hyperosmolar tears. Moreover, these neurons were activated by noxious thermal stimulation and menthol applied to the corneal surface. CONCLUSIONS These results demonstrate that innocuous "cold" cornea thermoreceptors are activated by drying of the ocular surface and hyperosmotic solutions, conditions that are consistent with a role in tear production. The authors hypothesize that the dysfunction of these corneal afferents and the lacrimation reflex pathway they activate lead to some forms of dry eye disease.},
annote = {professional financial advisors are often biased in unfavourable ways; this paper shows that they more frequently advise women to invest more carefully compared to men},
author = {Mullainathan, Sendhil and Noeth, Markus and Schoar, Antoinette},
doi = {10.2139/ssrn.1572334},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Mullainathan, Noeth, Schoar - 2012 - The Market for Financial Advice An Audit Study.pdf:pdf},
journal = {SSRN Electron. J.},
title = {{The Market for Financial Advice: An Audit Study}},
year = {2012}
}
@article{Masini2018,
abstract = {News media can be considered to fulfil their democratic role as a “marketplace of ideas” only if they present a diverse content that gives space to a wider range of ideas and viewpoints. But how can content diversity be assessed? And what determines actor and viewpoint diversity in the first place? By employing measurements of actor and viewpoint diversity at the article and newspaper level, this study provides a complete overview on the content diversity of immigration news, and it investigates factors that have an impact on content diversity of immigration newspaper articles in Belgium, Germany, Italy and the United Kingdom (2013-2014). The results of a multilevel analysis indicate that both the articles' size and the elite character of a newspaper play a key role in enhancing news' multiperspectivalness. Also, the findings show that these two measurements of content diversity are different yet related to each other. [ABSTRACT FROM AUTHOR], Copyright of Journalism Studies is the pro)},
annote = {these authors have had contributors annotate a large number of articles according to their actor and viewpoint diversity; these numbers are then compared on article- and newspaper level

only articles about immigration, but from several countries

but its more of a descriptive study; it doesn't introduce a novel way of measuring diversity... although it lists a few determinants of viewpoint diversity within articles and news outlets that could be handy, for example article length and level of newspaper (high- vs lowbrow)

if we could get their data, we might be able to extract more relevant predictors of viewpoint diversity},
author = {Masini, Andrea and {Van Aelst}, Peter and Zerback, Thomas and Reinemann, Carsten and Mancini, Paolo and Mazzoni, Marco and Damiani, Marco and Coen, Sharon},
doi = {10.1080/1461670x.2017.1343650},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Masini et al. - 2018 - Measuring and Explaining the Diversity of Voices and Viewpoints in the News.pdf:pdf},
issn = {1461-670X},
journal = {Journal. Stud.},
number = {15},
pages = {2324--2343},
publisher = {Taylor {\&} Francis},
title = {{Measuring and Explaining the Diversity of Voices and Viewpoints in the News}},
volume = {19},
year = {2018}
}
@article{Nargesian2020,
abstract = {We consider the problem of creating an effective navigation structure over a data lake. We define an organization as a navigation graph that contains nodes representing sets of attributes within a data lake and edges indicating subset relationships among nodes. We propose the data lake organization problem as the problem of finding an organization that allows a user to most effectively navigate a data lake. We present a new probabilistic model of how users interact with an organization and propose an approximate algorithm for the data lake organization problem. We show the effectiveness of the algorithm on both a real data lake containing data from open data portals and on a benchmark that contains rich metadata emulating the observed characteristics of real data lakes. Through a formal user study, we show that navigation can help users find relevant tables that cannot be found by keyword search.},
author = {Nargesian, Fatemeh and Pu, Ken Q. and Zhu, Erkang and {Ghadiri Bashardoost}, Bahar and Miller, Ren{\'{e}}e J.},
doi = {10.1145/3318464.3380605},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Nargesian et al. - 2020 - Organizing Data Lakes for Navigation.pdf:pdf},
isbn = {9781450367356},
issn = {07308078},
journal = {Proc. ACM SIGMOD Int. Conf. Manag. Data},
keywords = {data lakes,dataset discovery and search,structure learning},
pages = {1939--1950},
title = {{Organizing Data Lakes for Navigation}},
year = {2020}
}
@article{Ahmad2016,
abstract = {The rapid growth of information technology and communication has make the development of persuasive technology become aggressive. Trust has become one of the crucial elements in persuasive technology apart of credibility. This paper investigated trust in terms of cognitive and affective perception in relationship of human-computer interaction with persuasive technologies particularly in fitness application and educational games on environmental sustainability. A study was conducted with 25 participants for 6 weeks which requires them to use both categories of persuasive technologies. The result shows that the lack of trust problem in using persuasive technology found to be strongly significant. Cognitive trust perception is the main perception that leads users in making trust decision compared to affective trust.},
author = {Ahmad, Wan Nooraishya Wan and Ali, Nazlena Mohamad},
doi = {10.1109/ICCOINS.2016.7783187},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Ahmad, Ali - 2016 - Trust perceptions in using persuasive technologies.pdf:pdf},
isbn = {9781509051342},
journal = {2016 3rd Int. Conf. Comput. Inf. Sci. ICCOINS 2016 - Proc.},
keywords = {Affective,Cognitive,Persuasive technology,Trust},
number = {July 2017},
pages = {49--53},
title = {{Trust perceptions in using persuasive technologies}},
year = {2016}
}
@article{Verbeek2006,
abstract = {How to deal with ethical issues surrounding persuasive technologies? Despite the obvious goodintentions behind technologies like the FoodPhone (helping to fight obesity), the HygieneGuard (motivating people to wash their hands after using the toilet), and the EconoMeter (helping people to drive their cars more economically), ethical questions abound. Persuasive technologies can have undesirable consequences, employ problematic methods of persuasion, or persuade users to do things which cannot be morally justified. Moreover, the very practice of technological persuasion can raise moral questions in itself, because it might be seen as a threat to human autonomy, a source of moral laziness or an anti-democratic force in society which lets designers rather than representatives of the people steer our behaviour. This paper will address the ethical aspects of persuasive technologies and their designs in three steps. First it will locaclise the most important points of application for moral reflection during the design of persuasive technologies. By integrating the concept of ‘persuasive technology' with the concept of ‘technological mediation', as developed in theoretical frameworks from the field of persuasive technology and from the philosophy of technology, it will be possible to identify three such points of application. Second, this paper will deal with the process of moral reflection itself. A method will be elaborated to facilitate moral decision-making during the design of persuasive technologies, using the points of application identified in section 2. Third, the paper will discuss a number of ethical issues which are a bit more external to the practice of designing persuasive technologies, and which mainly concern the moral acceptability of specific persuasive technologies and of the phenomenon of persuasive technology as such. 2.},
author = {Verbeek, Peter-Paul},
journal = {Persuasive},
pages = {1--15},
title = {{Persuasive Technology and Moral Responsibility Toward an ethical framework for persuasive technologies}},
volume = {6},
year = {2006}
}
@article{Eskandanian2017,
abstract = {Much of the focus of recommender systems research has been on the accurate prediction of users' ratings for unseen items. Recent work has suggested that objectives such as diversity and novelty in recommendations are also important factors in the effectiveness of a recommender system. However, methods that attempt to increase diversity of recommendation lists for all users without considering each user's preference or tolerance for diversity may lead to monotony for some users and to poor recommendations for others. Our goal in this research is to evaluate the hypothesis that users' propensity towards diversity varies greatly and that the diversity of recommendation lists should be consistent with the level of user interest in diverse recommendations. We propose a pre-filtering clustering approach to group users with similar levels of tolerance for diversity. Our contributions are twofold. First, we propose a method for personalizing diversity by performing collaborative filtering independently on different segments of users based on the degree of diversity in their profiles. Secondly, we investigate the accuracy-diversity tradeoffs using the proposed method across different user segments. As part of this evaluation we propose new metrics, adapted from information retrieval, that help us measure the effectiveness of our approach in personalizing diversity. Our experimental evaluation is based on two different datasets: MovieLens movie ratings, and Yelp restaurant reviews.},
author = {Eskandanian, Farzad and Mobasher, Bamshad and Burke, Robin},
doi = {10.1145/3079628.3079699},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Eskandanian, Mobasher, Burke - 2017 - A clustering approach for personalizing diversity in collaborative recommender systems.pdf:pdf},
isbn = {9781450346351},
journal = {UMAP 2017 - Proc. 25th Conf. User Model. Adapt. Pers.},
keywords = {Collaborative filtering,Diversity,Personalization,Recommender systems},
pages = {280--284},
title = {{A clustering approach for personalizing diversity in collaborative recommender systems}},
year = {2017}
}
@article{Chen2019,
abstract = {One key consequence of the information revolution is a significant increase and a contamination of our information supply. The practice of fact checking won't suffice to eliminate the biases in text data we observe, as the degree of factuality alone does not determine whether biases exist in the spectrum of opinions visible to us. To better understand controversial issues, one needs to view them from a diverse yet comprehensive set of perspectives. For example, there are many ways to respond to a claim such as "animals should have lawful rights", and these responses form a spectrum of perspectives, each with a stance relative to this claim and, ideally, with evidence supporting it. Inherently, this is a natural language understanding task, and we propose to address it as such. Specifically, we propose the task of substantiated perspective discovery where, given a claim, a system is expected to discover a diverse set of well-corroborated perspectives that take a stance with respect to the claim. Each perspective should be substantiated by evidence paragraphs which summarize pertinent results and facts. We construct PERSPECTRUM, a dataset of claims, perspectives and evidence, making use of online debate websites to create the initial data collection, and augmenting it using search engines in order to expand and diversify our dataset. We use crowd-sourcing to filter out noise and ensure high-quality data. Our dataset contains 1k claims, accompanied with pools of 10k and 8k perspective sentences and evidence paragraphs, respectively. We provide a thorough analysis of the dataset to highlight key underlying language understanding challenges, and show that human baselines across multiple subtasks far outperform ma-chine baselines built upon state-of-the-art NLP techniques. This poses a challenge and opportunity for the NLP community to address.},
archivePrefix = {arXiv},
arxivId = {arXiv:1906.03538v1},
author = {Chen, Sihao and Khashabi, Daniel and Yin, Wenpeng and Callison-Burch, Chris and Roth, Dan},
doi = {10.18653/v1/n19-1053},
eprint = {arXiv:1906.03538v1},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Chen et al. - 2019 - Seeing Things from a Different AngleDiscovering Diverse Perspectives about Claims.pdf:pdf},
pages = {542--557},
title = {{Seeing Things from a Different Angle:Discovering Diverse Perspectives about Claims}},
year = {2019}
}
@article{Masini2017,
abstract = {News content diversity is generally considered to be an essential precondition for the promotion of social pluralism. However, how diversity of news content should be conceptualized and measured is less clear. We use a content analysis of newspaper articles about immigration (2013−14) in Belgium (Flanders) to measure the diversity of actors and viewpoints in the news, and to study the link between those two subdimensions of content diversity. We find that the representation of a plurality of active actors in a news article seems to go hand in hand with a more diverse range of viewpoints. The findings show that there are no significant differences in the level of actor and viewpoint diversity between quality and popular newspapers. However, the length of the article has a positive effect on providing more diversity. Moreover, our results indicate that allowing for individual immigrants to talk in the reporting is fundamental to promoting a more positive representation of immigration in the news.},
author = {Masini, Andrea and {Van Aelst}, Peter},
doi = {10.1515/commun-2017-0017},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Masini, Van Aelst - 2017 - Actor diversity and viewpoint diversity Two of a kind.pdf:pdf},
issn = {16134087},
journal = {Communications},
keywords = {content analysis,content diversity,immigration,journalism,news,public},
number = {2},
pages = {107--126},
title = {{Actor diversity and viewpoint diversity: Two of a kind?}},
volume = {42},
year = {2017}
}
@article{Rennhoff2014,
abstract = {Existing market-based measures of viewpoint diversity in the media have been criticized for lacking a theoretical foundation. This paper proposes a theoretical framework to develop market-based measures of viewpoint diversity. It then uses this framework to develop four viewpoint diversity measures using a panel dataset of local television ratings. Finally, an econometric model relates these viewpoint diversity measures to media ownership variables. It does not appear that market-based measures of viewpoint diversity are strongly related to media ownership structures. {\textcopyright} 2013 Elsevier B.V.},
annote = {Not really relevant for online content and viewpoint diversity in online news.

This is about marked share of TV channels; first determining viewers preferences and then relating market shares to viewpoint diversity. Many different channels with many shares = high diversity.

Assumption: a station's market shares are determined by the viewpoints they espouse (if they share the viewpoint of most people, they will get a lot of viewers)},
author = {Rennhoff, Adam D. and Wilbur, Kenneth C.},
doi = {10.1016/j.infoecopol.2013.10.002},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Rennhoff, Wilbur - 2014 - Market-based measures of viewpoint diversity.pdf:pdf},
issn = {01676245},
journal = {Inf. Econ. Policy},
keywords = {Media ownership,News,Viewpoint diversity},
number = {1},
pages = {1--11},
publisher = {Elsevier B.V.},
title = {{Market-based measures of viewpoint diversity}},
url = {http://dx.doi.org/10.1016/j.infoecopol.2013.10.002},
volume = {26},
year = {2014}
}
@inproceedings{Sakai2019,
abstract = {This study evaluates 30 IR evaluation measures or their instances, of which nine are for adhoc IR and 21 are for diversified IR, primarily from the viewpoint of whether their preferences of one SERP (search engine result page) over another actually align with users' preferences. The gold preferences were contructed by hiring 15 assessors, who independently examined 1,127 SERP pairs and made preference assessments. Two sets of preference assessments were obtained: one based on a relevance question “Which SERP is more relevant?” and the other based on a diversity question “Which SERP is likely to satisfy a higher number of users?” To our knowledge, our study is the first to have collected diversity preference assessments in this way and evaluated diversity measures successfully. Our main results are that (a) Popular adhoc IR measures such as nDCG actually align quite well with the gold relevance preferences; and that (b) While the D♯-measures align well with the gold diversity preferences, intent-aware measures perform relatively poorly. Moreover, as by-products of our analysis of existing evaluation measures, we define new adhoc measures called iRBU (intentwise Rank-Biased Utility) and EBR (Expected Blended Ratio); we demonstrate that an instance of iRBU performs as well as nDCG when compared to the gold relevance preferences. On the other hand, the original RBU, a recently-proposed diversity measure, underperforms the best D♯-measures when compared to the gold diversity preferences.},
annote = {IR = information retrieval
SERP = search engine result page
gold relevance = what users actually think
RBU = rank-biased utility

Wikipedia: Evaluation measures for an information retrieval (IR) system are used to assess how well the search results satisfied the user's query intent. Such metrics are often split into kinds: online metrics look at users' interactions with the search system, while offline metrics measure relevance, in other words how likely each result, or search engine results page (SERP) page as a whole, is to meet the information needs of the user.

This paper aims to compare two kinds of IR evaluation metrics with user's actual preferences: adhoc measures (used for relevance) and diversity measures. They do this by exposing 15 participants to a total of 1127 SERP pairs and asking them:

(1) Which SERP is more relevant?
(2) Which SERP is likely to satisfy a higher number of users?

The authors then compared people's decisions with the decisions made according to 9 adhoc measures (comparing to question 1) and 21 diversity measures (comparing to question 2). They analyzed the differences in choices using Kendalls Tau...?

This makes little sense for several reasons. First, it is not a good measure to ask people outright, since they do not know what is relevant for them (SOURCE, Facebook knows you better than you know yourself). Moreover, why would you ask a single person whether many people will prefer a given SERP? An algorithm will surely know that better. Second, why is everyone talking about different interpretations of diversity without explaining themselves? It seems to me that viewpoint diversity is the only relevant category, but it's always about some other diversity (topic, source, diverse user relevance...). Third, this is a multilevel structure. The analysis is questionable.

However, the adhoc and diversity measures are interesting and should be studied.},
author = {Sakai, Tetsuya and Zeng, Zhaohao},
booktitle = {SIGIR'19},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sakai, Zeng - 2019 - Which Diversity Evaluation Measures Are “ Good ”.pdf:pdf},
isbn = {9781450361729},
keywords = {2019,acm reference format,evaluation measures,search result diversification,tetsuya sakai and zhaohao,user preferences,which diversity evaluation mea-,zeng},
pages = {595--604},
title = {{Which Diversity Evaluation Measures Are “ Good ”?}},
year = {2019}
}
@article{Geiger2020,
annote = {structured content analysis to see whether human labelled training data is garbage or not (it's about reporting data sets)

we should report all the key infos from our data sets},
author = {Geiger, R Stuart and Yu, Kevin and Yang, Yanlai and Dai, Mindy and Qiu, Jie and Tang, Rebekah and Huang, Jenny},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Geiger et al. - 2020 - Garbage In , Garbage Out Do Machine Learning Application Papers in Social Computing Report Where Human-Labeled T.pdf:pdf},
isbn = {9781450369367},
keywords = {acm reference format,content analy-,data labeling,human annotation,machine learning,machine learning, data labeling, human annotation,,meta-research,research integrity,sis,training data},
pages = {325--336},
title = {{Garbage In , Garbage Out ? Do Machine Learning Application Papers in Social Computing Report Where Human-Labeled Training Data Comes From ?}},
year = {2020}
}
@inproceedings{Verma2018,
abstract = {Algorithm fairness has started to attract the attention of researchers in AI, Software Engineering and Law communities, with more than twenty different notions of fairness proposed in the last few years. Yet, there is no clear agreement on which definition to apply in each situation. Moreover, the detailed differences between multiple definitions are difficult to grasp. To address this issue, this paper collects the most prominent definitions of fairness for the algorithmic classification problem, explains the rationale behind these definitions, and demonstrates each of them on a single unifying case-study. Our analysis intuitively explains why the same case can be considered fair according to some definitions and unfair according to others.},
address = {New York, NY, USA},
annote = {great paper summarizing all definitions and metrics of algorithmic fairness},
author = {Verma, Sahil and Rubin, Julia},
booktitle = {Proc. Int. Work. Softw. Fairness},
doi = {10.1145/3194770.3194776},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Verma, Rubin - 2018 - Fairness definitions explained.pdf:pdf},
isbn = {9781450357463},
issn = {02705257},
pages = {1--7},
publisher = {Association for Computing Machinery},
series = {FairWare '18},
title = {{Fairness definitions explained}},
year = {2018}
}
@incollection{Kuang2015,
abstract = {Nonnegative matrix factorization (NMF) approximates a nonnegative matrix by the product of two low-rank nonnegative matrices. Since it gives semantically meaningful result that is easily interpretable in clustering applications, NMF has been widely used as a clustering method especially for document data, and as a topic modeling method. We describe several fundamental facts of NMF and introduce its optimization framework called block coordinate descent. In the context of clustering, our framework provides a flexible way to extend NMF such as the sparse NMF and the weakly-supervised NMF. The former provides succinct representations for better interpretations while the latter flexibly incorporate extra information and user feedback in NMF, which effectively works as the basis for the visual analytic topic modeling system that we present. Using real-world text data sets, we present quantitative experimental results showing the superiority of our framework from the following aspects: fast conver- gence, high clustering accuracy, sparse representation, consistent output, and user interactivity. In addition, we present a visual analytic system called UTOPIAN (User-driven Topic modeling based on Interactive NMF) and show several usage scenarios. Overall, our book chapter cover the broad spectrum of NMF in the context of clustering and topic modeling, from fundamental algorithmic behaviors to practical visual analytics systems.},
author = {Kuang, Da and Choo, Jaegul and Park, Haesun},
chapter = {7},
editor = {Celebri., Emre},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Kuang, Choo, Park - 2015 - Nonnegative Matrix Factorization for Interactive Topic Modeling and Document Clustering.pdf:pdf},
isbn = {9783319092584},
pages = {215--243},
publisher = {Springer},
title = {{Nonnegative Matrix Factorization for Interactive Topic Modeling and Document Clustering}},
year = {2015}
}
@article{Wang2019,
author = {Wang, Rui and Zhou, Deyu and Jiang, Mingmin and Si, Jiasheng and Yang, Yang},
doi = {10.1109/ACCESS.2019.2906754},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Wang et al. - 2019 - A survey on opinion mining From stance to product aspect.pdf:pdf},
issn = {21693536},
journal = {IEEE Access},
keywords = {Opinion mining,deep neural network,product aspect mining,stance detection,topic model},
pages = {41101--41124},
publisher = {IEEE},
title = {{A survey on opinion mining: From stance to product aspect}},
volume = {7},
year = {2019}
}
@article{Tversky1973,
abstract = {This paper explores a judgmental heuristic in which a person evaluates the frequency of classes or the probability of events by availability, i.e., by the ease with which relevant instances come to mind. In general, avail- ability is correlated with ecological frequency, but it is also affected by other factors. Consequently, the reliance on the availability heuristic leads to systematic biases. Such biases are demonstrated in the judged frequency of classes of words, of combinatorial outcomes, and of repeated events. The phenomenon of illusory correlation is explained as an availability bias. The effects of the availability of incidents and scenarios on subjective prob- ability are discussed.},
author = {Tversky, Amos and Kahnemann, Daniel},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Tversky, Kahnemann - 1973 - Availability A Heuristic for Judging Frequency and Probability.pdf:pdf},
journal = {Cogn. Psychol.},
pages = {207--232},
title = {{Availability: A Heuristic for Judging Frequency and Probability}},
volume = {5},
year = {1973}
}
@article{Nickerson1998,
abstract = {Confirmation bias, as the term is typically used in the psychological literature, connotes the seeking or interpreting of evidence in ways that are partial to existing beliefs, expectations, or a hypothesis in hand. The author reviews evidence of such a bias in a variety of guises and gives examples of its operation in several practical contexts. Possible explanations are considered, and the question of its utility or disutility is discussed.},
author = {Nickerson, Raymond S.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Nickerson - 1998 - Confirmation Bias A Ubiquitous Phenomenon in Many Guises.pdf:pdf},
journal = {Rev. Gen. Psychol.},
number = {2},
pages = {175--220},
title = {{Confirmation Bias: A Ubiquitous Phenomenon in Many Guises}},
volume = {2},
year = {1998}
}
@article{Epstein2015,
abstract = {Internet search rankings have a significant impact on consumer choices, mainly because users trust and choose higher-ranked results more than lower-ranked results. Given the apparent power of search rankings, we asked whether they could be manipulated to alter the preferences of undecided voters in democratic elections. Here we report the results of five relevant double-blind, randomized controlled experiments, using a total of 4,556 undecided voters representing diverse demographic characteristics of the voting populations of the United States and India. The fifth experiment is especially notable in that it was conducted with eligible voters throughout India in the midst of India's 2014 Lok Sabha elections just before the final votes were cast. The results of these experiments demonstrate that (i) biased search rankings can shift the voting preferences of undecided voters by 20{\%} or more, (ii) the shift can be much higher in some demographic groups, and (iii) search ranking bias can be masked so that people show no awareness of the manipulation. We call this type of influence, which might be applicable to a variety of attitudes and beliefs, the search engine manipulation effect. Given that many elections are won by small margins, our results suggest that a search engine company has the power to influence the results of a substantial number of elections with impunity. The impact of such manipulations would be especially large in countries dominated by a single search engine company.},
author = {Epstein, Robert and Robertson, Ronald E.},
doi = {10.1073/pnas.1419828112},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Epstein, Robertson - 2015 - The search engine manipulation effect (SEME) and its possible impact on the outcomes of elections.pdf:pdf},
issn = {10916490},
journal = {Proc. Natl. Acad. Sci. U. S. A.},
keywords = {Digital bandwagon effect,Internet influence,Search engine manipulation effect,Search rankings,Voter manipulation},
number = {33},
pages = {E4512--E4521},
title = {{The search engine manipulation effect (SEME) and its possible impact on the outcomes of elections}},
volume = {112},
year = {2015}
}
@article{Stanovich1997,
abstract = {A sample of 349 college students completed an argument evaluation test (AET) in which they evaluated arguments concerning real-life situations. A separate regression analysis was conducted for each student predicting his or her evaluations of argument quality from an objective indicator of argument quality and the strength of his or her prior beliefs about the target propositions. The beta weight for objective argument quality was interpreted in this analysis as an indicator of the ability to evaluate objective argument quality independent of prior belief. Individual differences in this index were reliably linked to individual differences in cognitive ability and actively open-minded thinking dispositions. Further, actively open-minded thinking predicted variance in AET performance even after individual differences in cognitive ability had been partialled out.},
author = {Stanovich, Keith E. and West, Richard F.},
doi = {10.1037/0022-0663.89.2.342},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Stanovich, West - 1997 - Reasoning Independently of Prior Belief and Individual Differences in Actively Open-Minded Thinking.pdf:pdf},
issn = {00220663},
journal = {J. Educ. Psychol.},
number = {2},
pages = {342--357},
title = {{Reasoning Independently of Prior Belief and Individual Differences in Actively Open-Minded Thinking}},
volume = {89},
year = {1997}
}
@inproceedings{Tintarev,
abstract = {Recommender systems for news articles on social media select and filter content through automatic personalization. As a result, users are often unaware of opposing points of view, leading to informational blindspots and potentially polarized opinions. They may be aware of a topic, but only be exposed to one viewpoint on this topic. However, recommender systems have just as much potential to help users find a plurality of viewpoints. In this spirit, this paper introduces an approach to automatically identifying content that represents a wider range of opinions on a given topic. Our offline results show positive results for our distance measure with regard to diversification on topic and channel. However, our user study results confirm that user acceptance of this diversification also needs to be addressed in tandem to enable a complete solution.},
annote = {- recommender systems select most relevant content, but they might as well optimise for diversity so that people become aware of different viewpoints

Tintarev et al. came up with a method to diversify articles within a topic based on linguistic features and metadata

- use case: system where user can select a topic to obtain several recent and relevant articles; articles are chosen based on diversity and relevance using a distance function applied to a Maximal Marginal Relevance (MMR) re-ranking algorithim

(MMR quantifies the extent of dissimilarity between an item being considered vs items that are already selected)

- how: similarity of articles is measured using linguistic features and metadata; combined in a linear weighted sum

thought: is it a problem that different viewpoints are displayed differently (e.g., short form vs long form content), causing people to not want to engage certain viewpoints for that reason?

thought 2: it would be interesting to evaluate this method with annotators; do we actually get a list of diverse viewpoints when we optimize according to this metric?},
author = {Tintarev, Nava and Sullivan, Emily and Guldin, Dror and Qiu, Sihang and Odijk, Daan},
booktitle = {UMAP '18 Adjun.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Tintarev et al. - 2018 - Same, Same, but Different.pdf:pdf},
keywords = {News recommendation,diversity based ranking,framing},
title = {{Same, Same, but Different}},
year = {2018}
}
@article{Yamamoto2016,
abstract = {During web search and browsing, people often accept misinformation due to their inattention to information credibility and biases. To obtain correct web information and support effective decision making, it is important to enhance searcher credibility assessment and develop algorithms to detect suspicious information. In this paper, we investigate how credibility alarms for web search results affect searcher behavior and decision making in information access systems. This study focuses on disputed topic suggestion as a credibility alarm approach. We conducted an online user study in which 92 participants performed a search task for health information. Through log analysis and user surveys, we confirmed the following. (1) Disputed topic suggestion in a search results list makes participants spend more time browsing pages than ordinary search conditions, thereby promoting careful information seeking. (2) Disputed topic suggestion during web browsing does not change participant behaviors but works as complementary information. This study contributes to system designs to enhance user engagement in critical and careful information seeking.},
author = {Yamamoto, Yusuke and Shimada, Satoshi},
doi = {10.1145/2914586.2914592},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Yamamoto, Shimada - 2016 - Can disputed topic suggestion enhance user consideration of information credibility in web search.pdf:pdf},
isbn = {9781450342476},
journal = {HT 2016 - Proc. 27th ACM Conf. Hypertext Soc. Media},
keywords = {Behavior analysis,Careful information seeking,Credibility,Decision making,Web search},
pages = {169--177},
title = {{Can disputed topic suggestion enhance user consideration of information credibility in web search?}},
year = {2016}
}
@article{vigdor2019apple,
author = {Vigdor, Neil},
journal = {New York Times},
title = {{Apple card investigated after gender discrimination complaints}},
year = {2019}
}
@article{Dietvorst2015,
abstract = {Research shows that evidence-based algorithms more accurately predict the future than do human forecasters. Yet when forecasters are deciding whether to use a human forecaster or a statistical algorithm, they often choose the human forecaster. This phenomenon, which we call algorithm aversion, is costly, and it is important to understand its causes. We show that people are especially averse to algorithmic forecasters after seeing them perform, even when they see them outperform a human forecaster. This is because people more quickly lose confidence in algorithmic than human forecasters after seeing them make the same mistake. In 5 studies, participants either saw an algorithm make forecasts, a human make forecasts, both, or neither. They then decided whether to tie their incentives to the future predictions of the algorithm or the human. Participants who saw the algorithm perform were less confident in it, and less likely to choose it over an inferior human forecaster. This was true even among those who saw the algorithm outperform the human.},
author = {Dietvorst, Berkeley J. and Simmons, Joseph P. and Massey, Cade},
doi = {10.1037/xge0000033},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Dietvorst, Simmons, Massey - 2015 - Algorithm aversion People erroneously avoid algorithms after seeing them err.pdf:pdf},
issn = {00963445},
journal = {J. Exp. Psychol. Gen.},
keywords = {Confidence,Decision aids,Decision making,Forecasting,Heuristics and biases},
number = {1},
pages = {114--126},
pmid = {25401381},
title = {{Algorithm aversion: People erroneously avoid algorithms after seeing them err}},
volume = {144},
year = {2015}
}
@article{Agarwal2019,
abstract = {Presentation bias is one of the key challenges when learning from implicit feedback in search engines, as it confounds the relevance signal. While it was recently shown how counterfactual learning-to-rank (LTR) approaches [18] can provably overcome presentation bias when observation propensities are known, it remains to show how to effectively estimate these propensities. In this paper, we propose the first method for producing consistent propensity estimates without manual relevance judgments, disruptive interventions, or restrictive relevance modeling assumptions. First, we show how to harvest a specific type of intervention data from historic feedback logs of multiple different ranking functions, and show that this data is sufficient for consistent propensity estimation in the position-based model. Second, we propose a new extremum estimator that makes effective use of this data. In an empirical evaluation, we find that the new estimator provides superior propensity estimates in two real-world systems - Arxiv Full-text Search and Google Drive Search. Beyond these two points, we find that the method is robust to a wide range of settings in simulation studies.},
annote = {this paper proposes a novel method (Intervention Harvesting) to gather interventional data under mild assumptions; with the end goal of estimating position bias

position bias has to be estimated, otherwise the behavior of users (clicks, dwell time etc.) cannot be modelled correctly in order to estimate relevance of documents

normally, the estimation of position bias is costly (either manual relevance judgements, disruptive interventions, or restrictive relevance-modeling assumptions) -- but the authors show that their method can be used for much less cost and achieve a performance similar to a gold standard},
archivePrefix = {arXiv},
arxivId = {1812.05161},
author = {Agarwal, Aman and Wang, Xuanhui and Li, Cheng and Najork, Marc and Zaitsev, Ivan and Joachims, Thorsten},
doi = {10.1145/3289600.3291017},
eprint = {1812.05161},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Agarwal et al. - 2019 - Estimating position bias without intrusive interventions.pdf:pdf},
isbn = {9781450359405},
journal = {WSDM 2019 - Proc. 12th ACM Int. Conf. Web Search Data Min.},
keywords = {Counterfactual inference,Propensity estimation,Unbiased learning-to-rank},
pages = {474--482},
title = {{Estimating position bias without intrusive interventions}},
year = {2019}
}
@article{Gollapudi2010,
abstract = {Click through rates (CTR) offer useful user feedback that can be used to infer the relevance of search results for queries. However it is not very meaningful to look at the raw click through rate of a search result because the likelihood of a result being clicked depends not only on its relevance but also the position in which it is displayed. One model of the browsing behavior, the {\{}$\backslash$em Examination Hypothesis{\}} $\backslash$cite{\{}RDR07,Craswell08,DP08{\}}, states that each position has a certain probability of being examined and is then clicked based on the relevance of the search snippets. This is based on eye tracking studies $\backslash$cite{\{}Claypool01, GJG04{\}} which suggest that users are less likely to view results in lower positions. Such a position dependent variation in the probability of examining a document is referred to as {\{}$\backslash$em position bias{\}}. Our main observation in this study is that the position bias tends to differ with the kind of information the user is looking for. This makes the position bias {\{}$\backslash$em query specific{\}}. In this study, we present a model for analyzing a query specific position bias from the click data and use these biases to derive position independent relevance values of search results. Our model is based on the assumption that for a given query, the positional click through rate of a document is proportional to the product of its relevance and a {\{}$\backslash$em query specific{\}} position bias. We compare our model with the vanilla examination hypothesis model (EH) on a set of queries obtained from search logs of a commercial search engine. We also compare it with the User Browsing Model (UBM) $\backslash$cite{\{}DP08{\}} which extends the cascade model of Craswell et al$\backslash$cite{\{}Craswell08{\}} by incorporating multiple clicks in a query session. We show that the our model, although much simpler to implement, consistently outperforms both EH and UBM on well-used measures such as relative error and cross entropy.},
annote = {this paper is about a new click model that the authors developed to predict which search result users will click on; the model builds on the examination hypothesis and computes a position bias based on the probability of examining and the relevance of documents

takeaways:
- examination hypothesis (see refs in text) states that a user has a certain probability of examining a result; if that result happens to be relevant (0,1) they will click on it
- position bias is query specific -- for example, it depends on whether the search is informational, navigational, or transactional},
archivePrefix = {arXiv},
arxivId = {1003.2458},
author = {Gollapudi, Sreenivas and Panigrahy, Rina},
eprint = {1003.2458},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Gollapudi, Panigrahy - 2010 - Revisiting the Examination Hypothesis with Query Specific Position Bias.pdf:pdf},
journal = {arXiv Prepr. arXiv1003.2458},
title = {{Revisiting the Examination Hypothesis with Query Specific Position Bias}},
url = {http://arxiv.org/abs/1003.2458},
year = {2010}
}
@article{Ghose2014,
abstract = {In this paper, we study the effects of three different kinds of search engine rankings on consumer behavior and search engine revenues: direct ranking effect, interaction effect between ranking and product ratings, and personalized ranking effect. We combine a hierarchical Bayesian model estimated on approximately one million online sessions from Travelocity, together with randomized experiments using a real-world hotel search engine application. Our archival data analysis and randomized experiments are consistent in demonstrating the following: (1) A consumer-utility-based ranking mechanism can lead to a significant increase in overall search engine revenue. (2) Significant interplay occurs between search engine ranking and product ratings. An inferior position on the search engine affects “higher-class” hotels more adversely. On the other hand, hotels with a lower customer rating are more likely to benefit from being placed on the top of the screen. These findings illustrate that product search engines could benefit from directly incorporating signals from social media into their ranking algorithms. (3) Our randomized experiments also reveal that an “active” personalized ranking system (wherein users can interact with and customize the ranking algorithm) leads to higher clicks but lower purchase propensities and lower search engine revenue compared with a “passive” personalized ranking system (wherein users cannot interact with the ranking algorithm). This result suggests that providing more information during the decision-making process may lead to fewer consumer purchases because of information overload. Therefore, product search engines should not adopt personalized ranking systems by default. Overall, our study unravels the economic impact of ranking and its interaction with social media on product search engines.},
author = {Ghose, Anindya and Ipeirotis, Panagiotis G. and Li, Beibei},
doi = {10.1287/mnsc.2013.1828},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Ghose, Ipeirotis, Li - 2014 - Examining the impact of ranking on consumer behavior and search engine revenue.pdf:pdf},
issn = {15265501},
journal = {Manage. Sci.},
keywords = {Electronic commerce,Hierarchical Bayesian methods,IT policy and management,Information systems,Randomized experiments,Travel search engine},
number = {7},
pages = {1632--1654},
title = {{Examining the impact of ranking on consumer behavior and search engine revenue}},
volume = {60},
year = {2014}
}
@article{Epstein2017,
abstract = {A recent series of experiments demonstrated that introducing ranking bias to election-related search engine results can have a strong and undetectable influence on the preferences of undecided voters. This phenomenon, called the Search Engine Manipulation Effect (SEME), exerts influence largely through order effects that are enhanced in a digital context. We present data from three new experiments involving 3,600 subjects in 39 countries in which we replicate SEME and test design interventions for suppressing the effect. In the replication, voting preferences shifted by 39.0{\%}, a number almost identical to the shift found in a previously published experiment (37.1{\%}). Alerting users to the ranking bias reduced the shift to 22.1{\%}, and more detailed alerts reduced it to 13.8{\%}. Users' browsing behaviors were also significantly altered by the alerts, with more clicks and time going to lower-ranked search results. Although bias alerts were effective in suppressing SEME, we found that SEME could be completely eliminated only by alternating search results – in effect, with an equal-time rule. We propose a browser extension capable of deploying bias alerts in real-time and speculate that SEME might be impacting a wide range of decision-making, not just voting, in which case search engines might need to be strictly regulated.},
author = {Epstein, Robert and Robertson, Ronald E. and Lazer, David and Wilson, Christo},
doi = {10.1145/3134677},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Epstein et al. - 2017 - Suppressing the Search Engine Manipulation Effect (SEME).pdf:pdf},
journal = {Proc. ACM Human-Computer Interact.},
keywords = {algorithmic influence,persuasive technology,search engine bias,search engine manipulation effect (SEME),voter manipulation},
number = {CSCW},
pages = {1--22},
title = {{Suppressing the Search Engine Manipulation Effect (SEME)}},
volume = {1},
year = {2017}
}
@article{Lin1991,
abstract = {A new class of information-theoretic divergence measures based on the Shannon entropy is introduced. Unlike the well-known Kullback divergences, the new measures do not require the condition of absolute continuity to be satisfied by the probability distributions involved. More importantly, their close relationship with the variational distance and the probability of misclassification error are established in terms of bounds. These bounds are crucial in many applications of divergence measures. The new measures are also well characterized by the properties of nonnegativity, finiteness, semiboundedness, and boundedness. {\textcopyright} 1991 IEEE},
author = {Lin, Jianhua},
doi = {10.1109/18.61115},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Lin - 1991 - Divergence Measures Based on the Shannon Entropy.pdf:pdf},
issn = {15579654},
journal = {IEEE Trans. Inf. Theory},
keywords = {Divergence,discrimination in,dissimilarity measure,entropy,formation,probability of error bounds},
number = {1},
pages = {145--151},
title = {{Divergence Measures Based on the Shannon Entropy}},
volume = {37},
year = {1991}
}
@inproceedings{Sapiezynski2019,
abstract = {In this work, we introduce a novel metric for auditing group fairness in ranked lists. Our approach offers two benefits compared to the state of the art. First, we offer a blueprint for modeling of user attention. Rather than assuming a logarithmic loss in importance as a function of the rank, we can account for varying user behaviors through parametrization. For example, we expect a user to see more items during a viewing of a social media feed than when they inspect the results list of a single web search query. Second, we allow non-binary protected attributes to enable investigating inherently continuous attributes (e.g., political alignment on the liberal to conservative spectrum) as well as to facilitate measurements across aggregated sets of search results, rather than separately for each result list. By combining these two elements into our metric, we are able to better address the human factors inherent in this problem. We measure the whole sociotechnical system, consisting of a ranking algorithm and individuals using it, instead of exclusively focusing on the ranking algorithm. Finally, we use our metric to perform three simulated fairness audits. We show that determining fairness of a ranked output necessitates knowledge (or a model) of the end-users of the particular service. Depending on their attention distribution function, a fixed ranking of results can appear biased both in favor and against a protected group1},
address = {New York, NY, USA},
annote = {these authors introduce another metric for categorical ranking bias (they claim that they can do continuous; but really they are just transforming continuous into categorical variables and then measuring)

their metric gives the auditor a lot of freedom: you can decide on the discounting, the estimation of the origin distribution, etc.

they then evaluate this on some data sets but it gets a bit confusing},
author = {Sapiezynski, Piotr and Zeng, Wesley and Robertson, Ronald E. and Mislove, Alan and Wilson, Christo},
booktitle = {Companion Proc. 2019 World Wide Web Conf.},
doi = {10.1145/3308560.3317595},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sapiezynski et al. - 2019 - Quantifying the Impact of User Attentionon Fair Group Representation in Ranked Lists.pdf:pdf},
isbn = {9781450366755},
keywords = {Group fairness,Information retrieval,Ranked lists},
pages = {553--562},
publisher = {Association for Computing Machinery},
series = {WWW '19},
title = {{Quantifying the Impact of User Attentionon Fair Group Representation in Ranked Lists}},
year = {2019}
}
@book{Clarke2009,
abstract = {Personalisation can have a significant impact on the way information is disseminated on the web today. Information Filtering$\backslash$n can be a significant ingredient towards a personalised web. Collaborative Filtering is already being applied successfully$\backslash$n for generating personalised recommendations of music tracks, books, movies and more. The same is not true for Content-Based$\backslash$n Filtering. In this paper, we identify some possible reasons for the notable absence of a broad range of personalised information$\backslash$n delivery and dissemination services on the web today. We advocate that a more holistic approach to user profiling is required$\backslash$n and we discuss the series of still open, challenging research issues raised.},
author = {Clarke, Charles L.A. and Kolla, Maheedhar and Vechtomova, Olga},
booktitle = {Adv. Inf. Retr. Theory},
doi = {10.1007/978-3-642-04417-5},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Clarke, Kolla, Vechtomova - 2009 - An Effectiveness Measure for Ambiguous and Underspecified Queries.pdf:pdf},
isbn = {978-3-642-04416-8},
pages = {188--199},
title = {{An Effectiveness Measure for Ambiguous and Underspecified Queries}},
url = {http://www.springerlink.com/index/10.1007/978-3-642-04417-5},
volume = {5766},
year = {2009}
}
@article{Tormala2018,
abstract = {Psychological certainty has been the subject of a great deal of research across a number of different literatures. This review focuses on prior and ongoing research on attitude certainty—the subjective sense of confidence of conviction a person has about an attitude—to provide a general overview of the role of certainty in attitudes and persuasion. First, we describe the antecedents, or origins, of attitude certainty, with particular attention to the metacognitive appraisals that drive people's feelings of certainty or uncertainty about their own attitudes. Second, we review the known consequences of attitude certainty, emphasizing the role of certainty in shaping information processing, attitude strength, and attitudinal advocacy. Third, we discuss recent developments that point to an upside for uncertainty in persuasion, whereby uncertainty experienced during message processing can increase message engagement and, thus, enhance message impact. Finally, we highlight several promising directions for future research. Our hope is that this review helps organize classic and contemporary research on attitude certainty and, in so doing, sparks new interest and continuing progress in the years to come.},
author = {Tormala, Zakary L. and Rucker, Derek D.},
doi = {10.1002/arcp.1004},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Tormala, Rucker - 2018 - Attitude certainty Antecedents, consequences, and new directions.pdf:pdf},
journal = {Consum. Psychol. Rev.},
number = {1},
pages = {72--89},
title = {{Attitude certainty: Antecedents, consequences, and new directions}},
volume = {1},
year = {2018}
}
@book{Lee2013,
abstract = {Bayesian inference has become a standard method of analysis in many fields of science. Students and researchers in experimental psychology and cognitive science, however, have failed to take full advantage of the new and exciting possibilities that the Bayesian approach affords. Ideal for teaching and self study, this book demonstrates how to do Bayesian modeling. Short, to-the-point chapters offer examples, exercises, and computer code (using WinBUGS or JAGS, and supported by Matlab and R), with additional support available online. No advance knowledge of statistics is required and, from the very start, readers are encouraged to apply and adjust Bayesian analyses by themselves. The book contains a series of chapters on parameter estimation and model selection, followed by detailed case studies from cognitive science. After working through this book, readers should be able to build their own Bayesian models, apply the models to their own data, and draw their own conclusions.},
author = {Lee, Michael D. and Wagenmakers, Eric Jan},
booktitle = {Bayesian Cogn. Model. A Pract. Course},
doi = {10.1017/CBO9781139087759},
isbn = {9781139087759},
publisher = {Cambridge University Press},
title = {{Bayesian cognitive modeling: A practical course}},
year = {2014}
}
@article{Bakshy2015,
abstract = {Exposure to news, opinion, and civic information increasingly occurs through social media. How do these online networks influence exposure to perspectives that cut across ideological lines? Using deidentified data,we examined how 10.1million U.S. Facebook users interact with socially shared news.We directlymeasured ideological homophily in friend networks and examined the extent to which heterogeneous friends could potentially expose individuals to cross-cutting content.We then quantified the extent to which individuals encounter comparativelymore or less diverse content while interacting via Facebook's algorithmically rankedNews Feed and further studied users'choices to click through to ideologically discordant content. Compared with algorithmic ranking, individuals' choices played a stronger role in limiting exposure to cross-cutting content. Supplementary mateirals included},
author = {Bakshy, Eytan and Messing, Solomon and Adamic, Lada A.},
doi = {10.1126/science.aaa1160},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Bakshy, Messing, Adamic - 2015 - Exposure to ideologically diverse news and opinion on Facebook.pdf:pdf},
issn = {10959203},
journal = {Science (80-. ).},
number = {6239},
pages = {1130--1132},
title = {{Exposure to ideologically diverse news and opinion on Facebook}},
volume = {348},
year = {2015}
}
@article{Lucic2019,
abstract = {At Ahold Delhaize, there is an interest in using more complex machine learning techniques for sales forecasting. It is difficult to convince analysts, along with their superiors, to adopt these techniques since the models are considered to be 'black boxes,' even if they perform better than current models in use. We aim to explore the impact of contrastive explanations about large errors on users' attitudes towards a 'black-box' model. In this work, we make two contributions. The first is an algorithm, Monte Carlo Bounds for Reasonable Predictions (MC-BRP). Given a large error, MC-BRP determines (1) feature values that would result in a reasonable prediction, and (2) general trends between each feature and the target, based on Monte Carlo simulations. The second contribution is the evaluation of MC-BRP along with its outcomes, which has both objective and subjective components. We evaluate on a real dataset with real users from Ahold Delhaize by conducting a user study to determine if explanations generated by MC-BRP help users understand why a prediction results in a large error, and if this promotes trust in an automatically-learned model. The study shows that users are able to answer objective questions about the model's predictions with overall 81.7{\%} accuracy when provided with these contrastive explanations. We also show that users who saw MC-BRP explanations understand why the model makes large errors in predictions significantly more than users in the control group.},
annote = {discussed during Rho Dec 2019

the goal of this paper was to increase people's trust in algorithms that help forecast sales by giving good explanations for large errors that the algorithm makes

they want to explain model failure by showing people what the prediction for "usual data" would have been; basically saying: look, this was just an outlier

they generate explanations and evaluate them in a user study; unfortunately they compare only to a control group (no explanation) and apparently the assignment to conditions was not random},
archivePrefix = {arXiv},
arxivId = {1908.00085},
author = {Lucic, Ana and Haned, Hinda and de Rijke, Maarten},
doi = {10.1145/3351095.3372824},
eprint = {1908.00085},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Lucic, Haned, de Rijke - 2019 - Contrastive Explanations for Large Errors in Retail Forecasting Predictions through Monte Carlo Simulati.pdf:pdf},
isbn = {9781450369367},
keywords = {2020,acm reference format,ana lucic,and maarten de rijke,erroneous predictions,explainability,hinda haned,interpretability,why does my model},
title = {{Contrastive Explanations for Large Errors in Retail Forecasting Predictions through Monte Carlo Simulations}},
url = {http://arxiv.org/abs/1908.00085},
year = {2019}
}
@article{Ross1977,
author = {{Ross, Lee and Greene, David and House}, Pamela},
doi = {10.1145/2984751.2985729},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Ross, Lee and Greene, David and House - 1977 - The “false consensus effect” An egocentric bias in social perception and attribution.pdf:pdf},
isbn = {9781450345316},
journal = {J. Exp. Soc. Psychol.},
number = {3},
pages = {279----301},
title = {{The “false consensus effect”: An egocentric bias in social perception and attribution processes}},
volume = {13},
year = {1977}
}
@inproceedings{Wauthier2011,
abstract = {Biased labelers are a systemic problem in crowdsourcing, and a comprehensive toolbox for handling their responses is still being developed. A typical crowdsourcing application can be divided into three steps: data collection, data curation, and learning. At present these steps are often treated separately. We present Bayesian Bias Mitigation for Crowdsourcing (BBMC), a Bayesian model to unify all three. Most data curation methods account for the effects of labeler bias by modeling all labels as coming from a single latent truth. Our model captures the sources of bias by describing labelers as influenced by shared random effects. This approach can account for more complex bias patterns that arise in ambiguous or hard labeling tasks and allows us to merge data curation and learning into a single computation. Active learning integrates data collection with learning, but is commonly considered infeasible with Gibbs sampling inference. We propose a general approximation strategy for Markov chains to efficiently quantify the effect of a perturbation on the stationary distribution and specialize this approach to active learning. Experiments show BBMC to outperform many common heuristics.},
author = {Wauthier, Fabian L. and Jordan, Michael I.},
booktitle = {Adv. Neural Inf. Process. Syst. 24 25th Annu. Conf. Neural Inf. Process. Syst. 2011, NIPS 2011},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Wauthier, Jordan - 2011 - Bayesian bias mitigation for crowdsourcing.pdf:pdf},
isbn = {9781618395993},
pages = {1--9},
title = {{Bayesian bias mitigation for crowdsourcing}},
year = {2011}
}
@article{White2014a,
abstract = {Search engines help people answer consequential questions. Biases in retrieved and indexed content (e.g., skew toward erroneous outcomes that represent deviations from reality), coupled with searchers' biases in how they examine and interpret search results, can lead people to incorrect answers. In this article, we seek to better understand biases in search and retrieval, and in particular those affecting the accuracy of content in search results, including the search engine index, features used for ranking, and the formulation of search queries. Focusing on the important domain of online health search, this research broadens previous work on biases in search to examine the role of search systems in contributing to biases. To assess bias, we focus on questions about medical interventions and employ reliable ground truth data from authoritative medical sources. In the course of our study, we utilize large-scale log analysis using data from a popular Web search engine, deep probes of result lists on that search engine, and crowdsourced human judgments of search result captions and landing pages. Our findings reveal bias in results, amplifying searchers' existing biases that appear evident in their search activity. We also highlight significant bias in indexed content and show that specific ranking signals and specific query terms support bias. Both of these can degrade result accuracy and increase skewness in search results. Our analysis has implications for bias mitigation strategies in online search systems, and we offer recommendations for search providers based on our findings.},
author = {White, Ryen W. and Hassan, Ahmed},
doi = {10.1145/2663355},
file = {:Users/tim/Surfdrive/Research/Library/Literature/White, Hassan - 2014 - Content bias in online health search.pdf:pdf},
issn = {1559114X},
journal = {ACM Trans. Web},
keywords = {Content biases,Health search},
number = {4},
pages = {1--33},
title = {{Content bias in online health search}},
volume = {8},
year = {2014}
}
@article{Orji2018,
abstract = {The evolving field of persuasive and behavior change technology is increasingly targeted at influencing behavior in the area of health and wellness. This paper provides an empirical review of 16 years (85 papers) of literature on persuasive technology for health and wellness to: (1.) answer important questions regarding the effectiveness of persuasive technology for health and wellness, (2.) summarize and highlight trends in the technology design, research methods, motivational strategies, theories, and health behaviors targeted by research to date, (3.) uncover pitfalls of existing persuasive technological interventions for health and wellness, and (4.) suggest directions for future research.},
author = {Orji, Rita and Moffatt, Karyn},
doi = {10.1177/1460458216650979},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Orji, Moffatt - 2018 - Persuasive technology for health and wellness State-of-the-art and emerging trends(2).pdf:pdf},
issn = {17412811},
journal = {Health Informatics J.},
keywords = {behavior change systems,behavior theories,gamification,health and wellness,health interventions,health technology,healthy behavior,motivational strategies,persuasive strategies,persuasive technology},
number = {1},
pages = {66--91},
pmid = {27245673},
title = {{Persuasive technology for health and wellness: State-of-the-art and emerging trends}},
volume = {24},
year = {2018}
}
@article{Flynn2016,
author = {Flynn, O and Tedesco, Salvatore and Urru, Andrea and Peckitt, James and Flynn, Brendan O},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Flynn et al. - 2016 - UCC Library and UCC researchers have made this item openly available . Please let us know how this has helped you.pdf:pdf},
isbn = {9781612085111},
title = {{UCC Library and UCC researchers have made this item openly available . Please let us know how this has helped you . Thanks ! Wearable Inertial Sensors as a Tool for Quantitative Assessment of Progress during Rehabilitation}},
year = {2016}
}
@article{Clarke2008,
abstract = {Evaluation measures act as objective functions to be optimized by information retrieval systems. Such objective functions must accurately reflect user requirements, particularly when tuning IR systems and learning ranking functions. Ambiguity in queries and redundancy in retrieved documents are poorly reflected by current evaluation measures. In this paper, we present a framework for evaluation that systematically rewards novelty and diversity. We develop this framework into a specific evaluation measure, based on cumulative gain. We demonstrate the feasibility of our approach using a test collection based on the TREC question answering track. Copyright 2008 ACM.},
author = {Clarke, Charles L.A. and Kolla, Maheedhar and Cormack, Gordon V. and Vechtomova, Olga and Ashkan, Azin and B{\"{u}}ttcher, Stefan and MacKinnon, Ian},
doi = {10.1145/1390334.1390446},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Clarke et al. - 2008 - Novelty and diversity in information retrieval evaluation.pdf:pdf},
isbn = {9781605581644},
journal = {ACM SIGIR 2008 - 31st Annu. Int. ACM SIGIR Conf. Res. Dev. Inf. Retrieval, Proc.},
keywords = {Experimentation,Human factors,Measurement},
pages = {659--666},
title = {{Novelty and diversity in information retrieval evaluation}},
year = {2008}
}
@book{carR,
abstract = {Title Companion to Applied Regression Depends R ({\textgreater}= 3.2.0), carData ({\textgreater}= 3.0-0) Description Functions to Accompany J. Fox and S. Weisberg, An R Companion to Applied Regression, Third Edition, Sage, in press. License GPL ({\textgreater}= 2) URL https://r-forge.r-project.org/projects/car/, https://CRAN.R-project.org/package=car,},
address = {Thousand Oaks CA},
author = {Fox, John and Weisberg, Sanford},
booktitle = {Thousand Oaks CA Sage},
edition = {Third},
isbn = {9781412975148},
issn = {9781412975148},
publisher = {Sage},
title = {{An R Companion to Applied Regression}},
url = {https://socialsciences.mcmaster.ca/jfox/Books/Companion/},
year = {2019}
}
@article{Helberger2018,
abstract = {{\textcopyright} 2016 The Author(s). Published by Informa UK Limited, trading as Taylor  {\&}  Francis Group. Personalized recommendations in search engines, social media and also in more traditional media increasingly raise concerns over potentially negative consequences for diversity and the quality of public discourse. The algorithmic filtering and adaption of online content to personal preferences and interests is often associated with a decrease in the diversity of information to which users are exposed. Notwithstanding the question of whether these claims are correct or not, this article discusses whether and how recommendations can also be designed to stimulate more diverse exposure to information and to break potential ‘filter bubbles' rather than create them. Combining insights from democratic theory, computer science and law, the article makes suggestions for design principles and explores the potential and possible limits of ‘diversity sensitive design'.},
author = {Helberger, Natali and Karppinen, Kari and D'Acunto, Lucia},
doi = {10.1080/1369118X.2016.1271900},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Helberger, Karppinen, D'Acunto - 2018 - Exposure diversity as a design principle for recommender systems.pdf:pdf},
issn = {14684462},
journal = {Inf. Commun. Soc.},
keywords = {Exposure diversity,autonomy,information diversity,nudging,recommender systems},
number = {2},
pages = {191--207},
publisher = {Taylor {\&} Francis},
title = {{Exposure diversity as a design principle for recommender systems}},
url = {https://doi.org/10.1080/1369118X.2016.1271900},
volume = {21},
year = {2018}
}
@article{Vilares2018,
abstract = {We explore how to detect people{\{}'{\}}s perspectives that occupy a certain proposition. We propose a Bayesian modelling approach where topics (or propositions) and their associated perspectives (or viewpoints) are modeled as latent variables. Words associated with topics or perspectives follow different generative routes. Based on the extracted perspectives, we can extract the top associated sentences from text to generate a succinct summary which allows a quick glimpse of the main viewpoints in a document. The model is evaluated on debates from the House of Commons of the UK Parliament, revealing perspectives from the debates without the use of labelled data and obtaining better results than previous related solutions under a variety of evaluations.},
author = {Vilares, David and He, Yulan},
doi = {10.18653/v1/d17-1165},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Vilares, He - 2018 - Detecting Perspectives in Political Debates.pdf:pdf},
pages = {1573--1582},
title = {{Detecting Perspectives in Political Debates}},
year = {2018}
}
@article{Levitan2014,
abstract = {The people we associate with everyday have an important influence on our exposure and reactions to political stimuli. Social network members in particular can have a dramatic impact on our political views and behavior. Prior research suggests that these attitudinal differences may reflect the information available in a social network: attitudinally congruent networks expose individuals to supporting positions, bolstering their views, while heterogeneous networks provide information on both sides of an issue, generating doubt and ambivalence. In contrast, the current studies examine the effects of individuals' networks in motivating them to find and engage with new political information on their own. Using ANES panel data, a laboratory-based information board session that examines behavior in detail, and an experimental design that manipulates network composition, we find that individuals in attitudinally heterogeneous social networks are more likely to seek out and attend to political information. They spend more time looking for political information, and then (having found it) spend more time reviewing that new information compared to those whose network members are more like-minded. An experimental study further demonstrates that network composition causally determines these information-seeking preferences. Implications for democratic citizenship in light of these findings are discussed.},
annote = {in this paper they describe three studies comparing how people behave in social networks that (1) confirm or (2) challenge their views; they find that if people are exposed to more diverse views spend more time engaging with content that they disagree with

- how they define "moderate view": they use 7-point likert scales but the categorization remains unclear
- how they measure user engagement:},
author = {Levitan, Lindsey and Wronski, Julie},
doi = {10.1007/s11109-013-9247-z},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Levitan, Wronski - 2014 - Social Context and Information Seeking Examining the Effects of Network Attitudinal Composition on Engagement.pdf:pdf},
issn = {01909320},
journal = {Polit. Behav.},
keywords = {Political cognition,Social networks},
number = {4},
pages = {793--816},
title = {{Social Context and Information Seeking: Examining the Effects of Network Attitudinal Composition on Engagement with Political Information}},
volume = {36},
year = {2014}
}
@article{Hessary,
author = {Hessary, Yasaman Kamyab and Calder, Bobby J and Malthouse, Edward C},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hessary, Calder, Malthouse - Unknown - Detecting Engagement with Digital Content.pdf:pdf},
keywords = {acm reference format,and edward c,bobby j,calder,clickstream data,digital news,user engagement,user experience,yasaman kamyab hessary,yayu zhou},
title = {{Detecting Engagement with Digital Content}}
}
@article{Sattarov2019,
abstract = {Trust in technology is an important factor for the design and use of technology in general. While there is growing interest in the role of trust on this general level, so far little attention has been given to the particularities of trust in persuasive technologies, i.e. technologies that serve to persuade users into certain behaviours. Those technologies are increasingly targeting the older adults, posing ethical questions that ask for sensitive investigation of trust. Here, we explore the specific character of trust in persuasive gerontechnology. We argue that the question of how to establish trust in technology, how to make trust lasting and enduring, requires considering user-centric and institution-centric approaches, and suggest an approach that is sensitive to wider social and institutional factors. The impact that persuasive gerontechnology can have depends on whether people can trust them, the designers, or the overall system. Drawing on studies of determinants of institutional trust, we identify four main strategies that can inform designers, technology assessors and policy makers in building trust between technology and users: (1) creating novel institutions, (2) creating incentives, (3) providing guarantees, and (4) ensuring transparency. We conclude the discussion with suggestions regarding future directions in researching trust and persuasive technology.},
author = {Sattarov, Faridun and Nagel, Saskia},
doi = {10.4017/gt.2019.18.1.001.00},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sattarov, Nagel - 2019 - Building trust in persuasive gerontechnology User-centric and institution-centric approaches.pdf:pdf},
issn = {1569111X},
journal = {Gerontechnology},
keywords = {E-health,Gerontechnology,Institutions,Persuasive technology,Trust},
number = {1},
pages = {1--14},
title = {{Building trust in persuasive gerontechnology: User-centric and institution-centric approaches}},
volume = {18},
year = {2019}
}
@article{Quraishi2018,
abstract = {The Web has evolved to a dominant platform where everyone has the opportunity to express their opinions, to interact with other users, and to debate on emerging events happening around the world. On the one hand, this has enabled the presence of different viewpoints and opinions about a - usually controversial - topic (like Brexit), but at the same time, it has led to phenomena like media bias, echo chambers and filter bubbles, where users are exposed to only one point of view on the same topic. Therefore, there is the need for methods that are able to detect and explain the different viewpoints. In this paper, we propose a graph partitioning method that exploits social interactions to enable the discovery of different communities (representing different viewpoints) discussing about a controversial topic in a social network like Twitter. To explain the discovered viewpoints, we describe a method, called Iterative Rank Difference (IRD), which allows detecting descriptive terms that characterize the different viewpoints as well as understanding how a specific term is related to a viewpoint (by detecting other related descriptive terms). The results of an experimental evaluation showed that our approach outperforms state-of-the-art methods on viewpoint discovery, while a qualitative analysis of the proposed IRD method on three different controversial topics showed that IRD provides comprehensive and deep representations of the different viewpoints.},
author = {Quraishi, Mainul and Fafalios, Pavlos and Herder, Eelco},
doi = {10.1145/3201064.3201076},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Quraishi, Fafalios, Herder - 2018 - Viewpoint discovery and understanding in social networks.pdf:pdf},
isbn = {9781450355636},
journal = {WebSci 2018 - Proc. 10th ACM Conf. Web Sci.},
keywords = {Social networks,Viewpoint discovery,Viewpoint understanding},
pages = {47--56},
title = {{Viewpoint discovery and understanding in social networks}},
volume = {3201076},
year = {2018}
}
@misc{JASP2020,
author = {JASP{\_}Team},
title = {{JASP (Version 0.14)}},
year = {2020}
}
@article{Auxier2019,
abstract = {With the influx of content being shared through social media, mobile apps, and other digital sources—including fake news and misinformation—most news consumers experience some degree of information overload. To combat these feelings of unease associated with the sheer volume of news content, some consumers tailor their news ecosystems and purposefully include or exclude content from specific sources or individuals. This study explores customization on social media and news platforms through a survey (N = 317) of adults regarding their digital news habits. Findings suggest that consumers who diversify their online news streams report lower levels of anxiety related to current events and highlight differences in reported anxiety levels and customization practices across the political spectrum. This study provides important insights into how perceived information overload, anxiety around current events, political affiliations and partisanship, and demographic characteristics may contribute to tailoring pract...},
annote = {this is about how people create echo chambers due to news / information overload; the idea is that the information is just too much, so people restrict themselves to content that they like or agree with

this goes in a very nice direction (and is very recent), but has again to do with news which doesn't go well with IBM

it could however have some implications that people turn to known sources for decision-making as well},
author = {Auxier, Brooke E. and Vitak, Jessica},
doi = {10.1177/2056305119847506},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Auxier, Vitak - 2019 - Factors Motivating Customization and Echo Chamber Creation Within Digital News Environments.pdf:pdf},
isbn = {2056305119},
issn = {2056-3051},
journal = {Soc. Media + Soc.},
keywords = {anxiety,customization,echo chambers,information overload,partisanship,social news},
number = {2},
pages = {205630511984750},
title = {{Factors Motivating Customization and Echo Chamber Creation Within Digital News Environments}},
volume = {5},
year = {2019}
}
@article{Belford2018,
abstract = {Topic models can provide us with an insight into the underlying latent structure of a large corpus of documents. A range of methods have been proposed in the literature, including probabilistic topic models and techniques based on matrix factorization. However, in both cases, standard implementations rely on stochastic elements in their initialization phase, which can potentially lead to different results being generated on the same corpus when using the same parameter values. This corresponds to the concept of “instability” which has previously been studied in the context of k-means clustering. In many applications of topic modeling, this problem of instability is not considered and topic models are treated as being definitive, even though the results may change considerably if the initialization process is altered. In this paper we demonstrate the inherent instability of popular topic modeling approaches, using a number of new measures to assess stability. To address this issue in the context of matrix factorization for topic modeling, we propose the use of ensemble learning strategies. Based on experiments performed on annotated text corpora, we show that a K-Fold ensemble strategy, combining both ensembles and structured initialization, can significantly reduce instability, while simultaneously yielding more accurate topic models.},
author = {Belford, Mark and {Mac Namee}, Brian and Greene, Derek},
doi = {10.1016/j.eswa.2017.08.047},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Belford, Mac Namee, Greene - 2018 - Stability of topic modeling via matrix factorization.pdf:pdf},
issn = {09574174},
journal = {Expert Syst. Appl.},
keywords = {LDA,NMF,Topic modeling,Topic stability},
pages = {159--169},
publisher = {Elsevier Ltd},
title = {{Stability of topic modeling via matrix factorization}},
url = {http://dx.doi.org/10.1016/j.eswa.2017.08.047},
volume = {91},
year = {2018}
}
@article{golebiewski2019data,
annote = {describes that users primarily engage with the first page of search results},
author = {{Golebiewski, Michael and Boyd}, Danah},
journal = {Data Soc.},
title = {{Data voids: Where missing data can easily be exploited}},
year = {2019}
}
@article{Hardt2016,
abstract = {We propose a criterion for discrimination against a specified sensitive attribute in supervised learning, where the goal is to predict some target based on available features. Assuming data about the predictor, target, and membership in the protected group are available, we show how to optimally adjust any learned predictor so as to remove discrimination according to our definition. Our framework also improves incentives by shifting the cost of poor classification from disadvantaged groups to the decision maker, who can respond by improving the classification accuracy. We enourage readers to consult the more complete manuscript on the arXiv.},
archivePrefix = {arXiv},
arxivId = {1610.02413},
author = {Hardt, Moritz and Price, Eric and Srebro, Nathan},
eprint = {1610.02413},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hardt, Price, Srebro - 2016 - Equality of opportunity in supervised learning.pdf:pdf},
issn = {10495258},
journal = {Adv. Neural Inf. Process. Syst.},
pages = {3323--3331},
title = {{Equality of opportunity in supervised learning}},
year = {2016}
}
@article{Alghamdi2015,
abstract = {—Topic models provide a convenient way to analyze large of unclassified text. A topic contains a cluster of words that frequently occur together. A topic modeling can connect words with similar meanings and distinguish between uses of words with multiple meanings. This paper provides two categories that can be under the field of topic modeling. First one discusses the area of methods of topic modeling, which has four methods that can be considerable under this category. These methods are Latent semantic analysis (LSA), Probabilistic latent semantic analysis (PLSA), Latent Dirichlet allocation (LDA), and Correlated topic model (CTM). The second category is called topic evolution models, which model topics by considering an important factor time. In the second category, different models are discussed, such as topic over time (TOT), dynamic topic models (DTM), multiscale topic tomography, dynamic topic correlation detection, detecting topic evolution in scientific literature, etc. Keywords—Topic Modeling; Methods of Topic Modeling; Latent semantic analysis (LSA); Probabilistic latent semantic analysis (PLSA); Latent Dirichlet allocation (LDA); Correlated topic model (CTM); Topic Evolution Modelin},
author = {Alghamdi, Rubayyi and Alfalqi, Khalid},
doi = {10.14569/ijacsa.2015.060121},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Alghamdi, Alfalqi - 2015 - A Survey of Topic Modeling in Text Mining.pdf:pdf},
issn = {2158107X},
journal = {Int. J. Adv. Comput. Sci. Appl.},
keywords = {analysis,correlated,ctm,latent dirichlet allocation,latent semantic analysis,lda,lsa,methods of topic modeling,plsa,probabilistic latent semantic,topic evolution modelin,topic model,topic modeling},
number = {1},
pages = {147--153},
title = {{A Survey of Topic Modeling in Text Mining}},
volume = {6},
year = {2015}
}
@article{Yue2018,
abstract = {Sentiments or opinions from social media provide the most up-to-date and inclusive information, due to the proliferation of social media and the low barrier for posting the message. Despite the growing importance of sentiment analysis, this area lacks a concise and systematic arrangement of prior efforts. It is essential to: (1) analyze its progress over the years, (2) provide an overview of the main advances achieved so far, and (3) outline remaining limitations. Several essential aspects, therefore, are addressed within the scope of this survey. On the one hand, this paper focuses on presenting typical methods from three different perspectives (task-oriented, granularity-oriented, methodology-oriented) in the area of sentiment analysis. Specifically, a large quantity of techniques and methods are categorized and compared. On the other hand, different types of data and advanced tools for research are introduced, as well as their limitations. On the basis of these materials, the essential prospects lying ahead for sentiment analysis are identified and discussed.},
author = {Yue, Lin and Chen, Weitong and Li, Xue and Zuo, Wanli and Yin, Minghao},
doi = {10.1007/s10115-018-1236-4},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Yue et al. - 2018 - A survey of sentiment analysis in social media.pdf:pdf},
issn = {02193116},
journal = {Knowl. Inf. Syst.},
keywords = {Data mining,Machine learning,Sentiment analysis,Social media,Survey},
number = {2},
pages = {1--47},
publisher = {Springer London},
title = {{A survey of sentiment analysis in social media}},
volume = {60},
year = {2018}
}
@article{Porto2007,
abstract = {This article identifies two basic models of citizen competence (the ignorant citizen and the rational citizen) in which normative theories of journalism and standards of news quality are grounded. I propose the interpreting citizen as an alternative view of citizen competence. According to this model, the availability of diverse interpretive frames in the public realm, particularly in the news media, is an important precondition for enhancing citizen competence. Given flaws in existing standards for evaluating journalism quality, the news media should be judged in terms of their performance in presenting diverse interpretive frames, rather than in terms of informational goals.},
author = {Porto, Mauro P.},
doi = {10.1080/07393180701560864},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Porto - 2007 - Frame diversity and citizen competence Towards a critical approach to news quality.pdf:pdf},
issn = {15295036},
journal = {Crit. Stud. Media Commun.},
keywords = {Citizen Competence,Diversity,Framing,News Quality,News Standards},
number = {4},
pages = {303--321},
title = {{Frame diversity and citizen competence: Towards a critical approach to news quality}},
volume = {24},
year = {2007}
}
@article{Fletcher2017,
abstract = {The move to a high choice online media environment has been associated with fears of audience fragmentation, and the end of a shared public agenda and common culture. Others have challenged this thesis by demonstrating high duplication among audiences for the most popular media outlets. However, this challenge has almost always been based on data from the United States alone, and has not fully accounted for cross-platform consumption. Using data from the 2016 Reuters Institute Digital News Report from six countries},
annote = {haven't read this article deeply yet, there may be more highlights},
author = {Fletcher, Richard and Nielsen, Rasmus Kleis},
doi = {10.1111/jcom.12315},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Fletcher, Nielsen - 2017 - Are News Audiences Increasingly Fragmented A Cross-National Comparative Analysis of Cross-Platform News Audie.pdf:pdf},
issn = {14602466},
journal = {J. Commun.},
keywords = {Audience Behavior,Comparative Research,Duplication,Fragmentation,News},
number = {4},
pages = {476--498},
title = {{Are News Audiences Increasingly Fragmented? A Cross-National Comparative Analysis of Cross-Platform News Audience Fragmentation and Duplication}},
volume = {67},
year = {2017}
}
@article{Baden2017,
abstract = {Journalistic news coverage plays an essential role for providing an audience with a diverse, multifaceted perspective upon public affairs. However, in the scholarly debate, most measures of viewpoint diversity do not distinguish between statements raising commensurable interpretations, and contributions that construct different meaning in a consequential sense. We provide an operationalization of viewpoint diversity that builds upon a tradition of identifying distinct interpretations through framing analysis. Going beyond frame diversity, we then distinguish between equivalent, complementary and competing, diverse interpretations: we consider as commensurable those frames that derive from the same interpretative repertoire', a notion borrowed from discourse studies. We propose a strategy for operationalization and the measurement of viewpoint diversity. Our focus on meaningfully different interpretations contributes to advancing research into journalism, political opinion formation, audience elaboration, and other important fields of study.},
annote = {viewpoint diversity should be assessed in a content-oriented way (i.e., not speaker-oriented)},
author = {Baden, Christian and Springer, Nina},
doi = {10.1177/1464884915605028},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Baden, Springer - 2017 - Conceptualizing viewpoint diversity in news discourse.pdf:pdf},
issn = {17413001},
journal = {Journalism},
keywords = {Discourse,framing,indexing,journalism,news,repertoires,viewpoint diversity},
number = {2},
pages = {176--194},
title = {{Conceptualizing viewpoint diversity in news discourse}},
volume = {18},
year = {2017}
}
@inproceedings{Fuglede2004,
author = {Fuglede, Bent and Tops{\o}e, Flemming},
booktitle = {IEEE Int. Symp. Inf. Theory - Proc.},
doi = {10.1109/isit.2004.1365067},
issn = {21578097},
pages = {31},
title = {{Jensen-Shannon divergence and Hubert space embedding}},
year = {2004}
}
@inproceedings{Labadie2008,
abstract = {Abstract-In this paper, we try to fathom the real impact of corpus quality on methods performances and their evaluations.The considered task is topic-based text segmentation, and two highly different unsupervised algorithms are compared: C99,a word-based system, augmented with LSA, and T ranseg, a sentence-based system. Two main characteristics of corpora have been investigated: Data quality (clean vs raw corpora), corpora manipulation (natural vs artificial data sets). The corpus size has also been subject to variation, and experiments related in this paper have shown that corpora characteristics highly impact recall and precision values for both algorithms.{\textcopyright}2008 IEEE.},
author = {Labadi{\'{e}}, Alexandre and Prince, Violaine},
booktitle = {Proc. Int. Multiconference Comput. Sci. Inf. Technol. IMCSIT 2008},
doi = {10.1109/IMCSIT.2008.4747258},
isbn = {9788360810149},
title = {{The impact of corpus quality and type on topic based text segmentation evaluation}},
year = {2008}
}
@inproceedings{Paul2010summarizing,
author = {Paul, Michael J and Girju, Roxana},
booktitle = {Proc. 2010 Conf. Empir. methods Nat. Lang. Process.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Paul, Girju - 2010 - Summarizing Contrastive Viewpoints in Opinionated Text Michael.pdf:pdf},
number = {October},
pages = {66--76},
publisher = {Association for Computational Linguistics},
title = {{Summarizing Contrastive Viewpoints in Opinionated Text Michael}},
year = {2010}
}
@inproceedings{Hofmann1999,
abstract = {Probabilistic Latente Semantic Analysis is a novel statistical technique for the analysis of two-mode and co-occurrence data, which has applications in information retrievaland filtering, natural language processing, machine learning fromtext,and in related areas. Compared to standard Latent Semantic Analysis which stems from linear algebra and performs a Singular VAlue Decomposition of co-occurrence tables, the proposed method is based on a mixture decomposition derived from a latent class model. Inorder to avoid overfitting, we propose a widely applicable generalization of maximumlikelihood model fitting by tempered EM. Our approach yields substantial and consistent improvements over Latent Semantic Analysis in a number of experiments.},
archivePrefix = {arXiv},
arxivId = {1301.6705},
author = {Hofmann, Thomas},
booktitle = {Proc. Fifteenth Conf. Uncertain. Artif. Intell.},
doi = {10.1.1.33.1187},
eprint = {1301.6705},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hofmann - 1999 - Probabilistic Latent Semantic Analysis.pdf:pdf},
isbn = {1581130961},
issn = {15206882},
pmid = {18989936},
publisher = {Morgan Kaufmann Publishers Inc.},
title = {{Probabilistic Latent Semantic Analysis}},
url = {http://ci.nii.ac.jp/ncid/BA6721422X},
year = {1999}
}
@article{Corbett-Davies2018,
abstract = {The nascent field of fair machine learning aims to ensure that decisions guided by algorithms are equitable. Over the last several years, three formal definitions of fairness have gained prominence: (1) anti-classification, meaning that protected attributes---like race, gender, and their proxies---are not explicitly used to make decisions; (2) classification parity, meaning that common measures of predictive performance (e.g., false positive and false negative rates) are equal across groups defined by the protected attributes; and (3) calibration, meaning that conditional on risk estimates, outcomes are independent of protected attributes. Here we show that all three of these fairness definitions suffer from significant statistical limitations. Requiring anti-classification or classification parity can, perversely, harm the very groups they were designed to protect; and calibration, though generally desirable, provides little guarantee that decisions are equitable. In contrast to these formal fairness criteria, we argue that it is often preferable to treat similarly risky people similarly, based on the most statistically accurate estimates of risk that one can produce. Such a strategy, while not universally applicable, often aligns well with policy objectives; notably, this strategy will typically violate both anti-classification and classification parity. In practice, it requires significant effort to construct suitable risk estimates. One must carefully define and measure the targets of prediction to avoid retrenching biases in the data. But, importantly, one cannot generally address these difficulties by requiring that algorithms satisfy popular mathematical formalizations of fairness. By highlighting these challenges in the foundation of fair machine learning, we hope to help researchers and practitioners productively advance the area.},
archivePrefix = {arXiv},
arxivId = {1808.00023},
author = {Corbett-Davies, Sam and Goel, Sharad},
eprint = {1808.00023},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Corbett-Davies, Goel - 2018 - The Measure and Mismeasure of Fairness A Critical Review of Fair Machine Learning.pdf:pdf},
journal = {arXiv Prepr. arXiv1808.00023},
keywords = {algorithms,anti-classification,bias,calibration,classification parity,decision analysis},
title = {{The Measure and Mismeasure of Fairness: A Critical Review of Fair Machine Learning}},
url = {http://arxiv.org/abs/1808.00023},
year = {2018}
}
@article{Blei2010,
abstract = {We present the nested Chinese restaurant process (nCRP), a stochastic process which assigns probability distributions to infinitely-deep, infinitely-branching trees. We show how this stochastic process can be used as a prior distribution in a Bayesian nonparametric model of document collections. Specifically, we present an application to information retrieval in which documents are modeled as paths down a random tree, and the preferential attachment dynamics of the nCRP leads to clustering of documents according to sharing of topics at multiple levels of abstraction. Given a corpus of documents, a posterior inference algorithm finds an approximation to a posterior distribution over trees, topics and allocations of words to levels of the tree. We demonstrate this algorithm on collections of scientific abstracts from several journals. This model exemplifies a recent trend in statistical machine learning--the use of Bayesian nonparametric methods to infer distributions on flexible data structures.},
author = {Blei, David M. and Griffiths, Thomas L. and Jordan, Michael I.},
doi = {10.1145/1667053.1667056},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Blei, Griffiths, Jordan - 2010 - The nested Chinese restaurant process and Bayesian nonparametric inference of topic hierarchies.pdf:pdf},
issn = {00045411},
journal = {J. ACM},
keywords = {Bayesian nonparametric statistics,Unsupervised learning},
number = {2},
pages = {1--30},
title = {{The nested Chinese restaurant process and Bayesian nonparametric inference of topic hierarchies}},
volume = {57},
year = {2010}
}
@article{Sun2017,
abstract = {As the prevalence of social media on the Internet, opinion mining has become an essential approach to analyzing so many data. Various applications appear in a wide range of industrial domains. Meanwhile, opinions have diverse expressions which bring along research challenges. Both of the practical demands and research challenges make opinion mining an active research area in recent years. In this paper, we present a review of Natural Language Processing (NLP) techniques for opinion mining. First, we introduce general NLP techniques which are required for text preprocessing. Second, we investigate the approaches of opinion mining for different levels and situations. Then we introduce comparative opinion mining and deep learning approaches for opinion mining. Opinion summarization and advanced topics are introduced later. Finally, we discuss some challenges and open problems related to opinion mining.},
author = {Sun, Shiliang and Luo, Chen and Chen, Junyu},
doi = {10.1016/j.inffus.2016.10.004},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sun, Luo, Chen - 2017 - A review of natural language processing techniques for opinion mining systems.pdf:pdf},
issn = {15662535},
journal = {Inf. Fusion},
keywords = {Deep learning,Machine learning,Natural language processing,Opinion mining,Sentiment analysis},
pages = {10--25},
publisher = {Elsevier B.V.},
title = {{A review of natural language processing techniques for opinion mining systems}},
url = {http://dx.doi.org/10.1016/j.inffus.2016.10.004},
volume = {36},
year = {2017}
}
@article{Sirrianni2019,
annote = {these authors argue that ideological diversity is good, and that although people don't like to interact with opposing ideas, they do so when the ideas are promoted by their social connections; thus the authors want to improve opinion diversity in social recommender systems

in their experiments, overarching topics and the associated positions were known beforehand; users then gave their opinion on EACH position in written text and indicated on a scale from -1 to 1 whether they agree or disagree with the position; from that the system inferred an opinion vector (that users opinion on all the different positions) and calculated distance between vectors... from there they diversified

differences to my work:
- this is about recommender systems, not IR
- they are focusing on opinion, not viewpoint
- potential positions on an issue seem to be required beforehand},
author = {Sirrianni, Joseph W and Liu, Xiaoqing Frank and Rahman, Mahfuzer and Adams, Douglas},
doi = {10.1109/ICCC.2019.00029},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sirrianni et al. - 2019 - An Opinion Diversity Enhanced Social Connection Recommendation Re-ranking Method based on Opinion Distance in.pdf:pdf},
isbn = {9781728127118},
journal = {2019 IEEE Int. Conf. Cogn. Comput.},
keywords = {-diversity of opinion,cyber argumentation,ranking,recommendation,recommendation re-,social connection,social networking},
number = {Iccc},
pages = {106--113},
publisher = {IEEE},
title = {{An Opinion Diversity Enhanced Social Connection Recommendation Re-ranking Method based on Opinion Distance in Cyber Argumentation with Social Networking}},
year = {2019}
}
@article{Dietvorst2018,
abstract = {Although evidence-based algorithms consistently outperform human forecasters, people often fail to use them after learning that they are imperfect, a phenomenon known as algorithm aversion. In this paper, we present three studies investigating how to reduce algorithm aversion. In incentivized forecasting tasks, participants chose between using their own forecasts or those of an algorithm that was built by experts. Participants were considerably more likely to choose to use an imperfect algorithm when they could modify its forecasts, and they performed better as a result. Notably, the preference for modifiable algorithms held even when participants were severely restricted in the modifications they could make (Studies 1-3). In fact, our results suggest that participants' preference for modifiable algorithms was indicative of a desire for some control over the forecasting outcome, and not for a desire for greater control over the forecasting outcome, as participants' preference for modifiable algorithms was relatively insensitive to the magnitude of the modifications they were able to make (Study 2). Additionally, we found that giving participants the freedom to modify an imperfect algorithm made them feel more satisfied with the forecasting process, more likely to believe that the algorithm was superior, and more likely to choose to use an algorithm to make subsequent forecasts (Study 3). This research suggests that one can reduce algorithm aversion by giving people some control-even a slight amount-over an imperfect algorithm's forecast.},
author = {Dietvorst, Berkeley J. and Simmons, Joseph P. and Massey, Cade},
doi = {10.1287/mnsc.2016.2643},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Dietvorst, Simmons, Massey - 2018 - Overcoming algorithm aversion People will use imperfect algorithms if they can (even slightly) modif.pdf:pdf},
issn = {15265501},
journal = {Manage. Sci.},
keywords = {Confidence,Decision AIDS,Decision making,Forecasting,Heuristics and biases},
number = {3},
pages = {1155--1170},
title = {{Overcoming algorithm aversion: People will use imperfect algorithms if they can (even slightly) modify them}},
volume = {64},
year = {2018}
}
@article{Ntoutsi2020,
abstract = {Artificial Intelligence (AI)-based systems are widely employed nowadays to make decisions that have far-reaching impact on individuals and society. Their decisions might affect everyone, everywhere, and anytime, entailing concerns about potential human rights issues. Therefore, it is necessary to move beyond traditional AI algorithms optimized for predictive performance and embed ethical and legal principles in their design, training, and deployment to ensure social good while still benefiting from the huge potential of the AI technology. The goal of this survey is to provide a broad multidisciplinary overview of the area of bias in AI systems, focusing on technical challenges and solutions as well as to suggest new research directions towards approaches well-grounded in a legal frame. In this survey, we focus on data-driven AI, as a large part of AI is powered nowadays by (big) data and powerful machine learning algorithms. If otherwise not specified, we use the general term bias to describe problems related to the gathering or processing of data that might result in prejudiced decisions on the bases of demographic features such as race, sex, and so forth. This article is categorized under: Commercial, Legal, and Ethical Issues {\textgreater} Fairness in Data Mining Commercial, Legal, and Ethical Issues {\textgreater} Ethical Considerations Commercial, Legal, and Ethical Issues {\textgreater} Legal Issues.},
author = {Ntoutsi, Eirini and Fafalios, Pavlos and Gadiraju, Ujwal and Iosifidis, Vasileios and Nejdl, Wolfgang and Vidal, Maria Esther and Ruggieri, Salvatore and Turini, Franco and Papadopoulos, Symeon and Krasanakis, Emmanouil and Kompatsiaris, Ioannis and Kinder-Kurlanda, Katharina and Wagner, Claudia and Karimi, Fariba and Fernandez, Miriam and Alani, Harith and Berendt, Bettina and Kruegel, Tina and Heinze, Christian and Broelemann, Klaus and Kasneci, Gjergji and Tiropanis, Thanassis and Staab, Steffen},
doi = {10.1002/widm.1356},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Ntoutsi et al. - 2020 - Bias in data-driven artificial intelligence systems—An introductory survey.pdf:pdf},
issn = {19424795},
journal = {Wiley Interdiscip. Rev. Data Min. Knowl. Discov.},
keywords = {fairness,fairness-aware AI,fairness-aware machine learning,interpretability,responsible AI},
number = {3},
pages = {1--14},
title = {{Bias in data-driven artificial intelligence systems—An introductory survey}},
volume = {10},
year = {2020}
}
@article{Joachims2018,
abstract = {Implicit feedback (e.g., clicks, dwell times, etc.) is an abundant source of data in human-interactive systems. While implicit feedback has many advantages (e.g., it is inexpensive to collect, user-centric, and timely), its inherent biases are a key obstacle to its effective use. For example, position bias in search rankings strongly influences how many clicks a result receives, so that directly using click data as a training signal in Learning-to-Rank (LTR) methods yields sub-optimal results. To overcome this bias problem, we present a counterfactual inference framework that provides the theoretical basis for unbiased LTR via Empirical Risk Minimization despite biased data. Using this framework, we derive a propensity-weighted ranking SVM for discriminative learning from implicit feedback, where click models take the role of the propensity estimator. Beyond the theoretical support, we show empirically that the proposed learning method is highly effective in dealing with biases, that it is robust to noise and propensity model mis-specification, and that it scales efficiently. We also demonstrate the real-world applicability of our approach on an operational search engine, where it substantially improves retrieval performance.},
archivePrefix = {arXiv},
arxivId = {1608.04468},
author = {Joachims, Thorsten and Swaminathan, Adith and Schnabel, Tobias},
doi = {10.24963/ijcai.2018/738},
eprint = {1608.04468},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Joachims, Swaminathan, Schnabel - 2018 - Unbiased learning-to-rank with biased feedback.pdf:pdf},
isbn = {9780999241127},
issn = {10450823},
journal = {IJCAI Int. Jt. Conf. Artif. Intell.},
pages = {5284--5288},
title = {{Unbiased learning-to-rank with biased feedback}},
volume = {2018-July},
year = {2018}
}
@article{VanDerLee2019,
abstract = {Currently, there is little agreement as to how Natural Language Generation (NLG) systems should be evaluated, with a particularly high degree of variation in the way that human evaluation is carried out. This paper provides an overview of how human evaluation is currently conducted, and presents a set of best practices, grounded in the literature. With this paper, we hope to contribute to the quality and consistency of human evaluations in NLG.},
annote = {the goal of this paper is to define some best practices for human evaluation of natural language generation (NLG) text

they discuss how human evaluation is commonly approached and some best practices

the best practices, especially with regard to research design and statistical analyses, are fantastic -- I could maybe write something like this for HCI or so at some point

---{\textgreater} I could write a paper like this for IR / RecSys!!! read evaluation stuff and see what I could contribute / how I could integrate that into my PhD},
author = {{Van Der Lee}, Chris and Gatt, Albert and {Van Miltenburg}, Emiel and Wubben, Sander and Krahmer, Emiel},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Van Der Lee et al. - 2019 - Best practices for the human evaluation of automatically generated text.pdf:pdf},
journal = {Proc. 12th Int. Conf. Nat. Lang. Gener.},
title = {{Best practices for the human evaluation of automatically generated text}},
year = {2019}
}
@inproceedings{Oinas-Kukkonen2008,
abstract = {A growing number of information technology systems and services are being developed for persuasive purposes, i.e. to change users' attitudes or behaviour or both. Despite the fact that attitudinal theories from social psychology have been quite extensively applied to the study of user intentions and behaviour, computer scientists and user interface designers are not very familiar with the theories related to attitude change. Moreover, these theories are not directly applicable for developing software and information systems. This paper builds upon the attitude change theories from social psychology recognising dimensions and approaches that help move towards a practical conceptual framework for understanding and designing persuasion in information systems. {\textcopyright} 2008 IEEE.},
annote = {Persuasive systems may be defined as “computerized software or information systems designed to reinforce, change or shape attitudes or behaviors or both without using coercion or deception"},
author = {Oinas-Kukkonen, Harri and Harjumaa, Marja},
booktitle = {Proc. 1st Int. Conf. Adv. Comput. Interact. ACHI 2008},
doi = {10.1109/ACHI.2008.31},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Oinas-Kukkonen, Harjumaa - 2008 - Towards deeper understanding of persuasion in software and information systems.pdf:pdf},
title = {{Towards deeper understanding of persuasion in software and information systems}},
year = {2008}
}
@article{Sattigeri2018,
abstract = {In this paper, we introduce the Fairness GAN, an approach for generating a dataset that is plausibly similar to a given multimedia dataset, but is more fair with respect to protected attributes in allocative decision making. We propose a novel auxiliary classifier GAN that strives for demographic parity or equality of opportunity and show empirical results on several datasets, including the CelebFaces Attributes (CelebA) dataset, the Quick, Draw!$\backslash$ dataset, and a dataset of soccer player images and the offenses they were called for. The proposed formulation is well-suited to absorbing unlabeled data; we leverage this to augment the soccer dataset with the much larger CelebA dataset. The methodology tends to improve demographic parity and equality of opportunity while generating plausible images.},
archivePrefix = {arXiv},
arxivId = {1805.09910},
author = {Sattigeri, Prasanna and Hoffman, Samuel C. and Chenthamarakshan, Vijil and Varshney, Kush R.},
eprint = {1805.09910},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sattigeri et al. - 2018 - Fairness GAN.pdf:pdf},
title = {{Fairness GAN}},
url = {http://arxiv.org/abs/1805.09910},
year = {2018}
}
@article{Rossi2019,
abstract = {Artificial Intelligence (AI) is a scientific discipline aimed at building machines that can perform many tasks that require human intelligence. AI started more than 60 years ago, and includes two main areas of research. One is based on rules, logic, and symbols; it is explainable; and it always finds a correct solution for a given problem, if that problem has been correctly specified. However, it can be used only when all possible scenarios for the problem at hand can be foreseen. The other area of research is based on examples, data analysis, and correlation. It can be applied in cases where there is an incomplete or ill-defined notion of the probl.....},
author = {Rossi, F.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Rossi - 2019 - Building trust in artificial intelligence.pdf:pdf},
journal = {J. Int. Aff.},
number = {1},
pages = {127--133},
title = {{Building trust in artificial intelligence}},
volume = {72},
year = {2019}
}
@article{Chen2019a,
annote = {this is interesting, but more related to news and news overload / well-being; therefore not too useful now for decision-making},
author = {Chen, Victoria Y. and {Masullo Chen}, Gina},
doi = {10.1080/15456870.2019.1616738},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Chen, Masullo Chen - 2019 - Shut down or turn off The interplay between news overload and consumption.pdf:pdf},
issn = {1545-6870},
journal = {Atl. J. Commun.},
number = {00},
pages = {1--13},
publisher = {Routledge},
title = {{Shut down or turn off? The interplay between news overload and consumption}},
url = {https://doi.org/10.1080/15456870.2019.1616738},
volume = {0},
year = {2019}
}
@article{Hernandez2013,
abstract = {One difficulty in persuasion is overcoming the confirmation bias, where people selectively seek evidence that is consistent with their prior beliefs and expectations. This biased search for information allows people to analyze new information in an efficient, but shallow way. The present research discusses how experienced difficultly in processing (disfluency) can reduce the confirmation bias by promoting careful, analytic processing. In two studies, participants with prior attitudes on an issue became less extreme after reading an argument on the issues in a disfluent format. The change occurred for both naturally occurring attitudes (i.e. political ideology) and experimentally assigned attitudes (i.e. positivity toward a court defendant). Importantly, disfluency did not reduce confirmation biases when participants were under cognitive load, suggesting that cognitive resources are necessary to overcome these biases. Overall, these results suggest that changing the style of an argument's presentation can lead to attitude change by promoting more comprehensive consideration of opposing views. {\textcopyright} 2012 Elsevier Inc.},
author = {Hernandez, Ivan and Preston, Jesse Lee},
doi = {10.1016/j.jesp.2012.08.010},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hernandez, Preston - 2013 - Disfluency disrupts the confirmation bias.pdf:pdf},
issn = {00221031},
journal = {J. Exp. Soc. Psychol.},
keywords = {Attitude change,Confirmation bias,Fluency,Persuasion},
number = {1},
pages = {178--182},
title = {{Disfluency disrupts the confirmation bias}},
volume = {49},
year = {2013}
}
@article{DeWinter2010,
abstract = {Likert questionnaires are widely used in survey research, but it is unclear whether the item data should be investigated by means of parametric or nonparametric procedures. This study compared the Type I and II error rates of the t test versus the MannWhitneyWilcoxon (MWW) for fivepoint Likert items. Fourteen population distributions were defined and pairs of samples were drawn from the populations and submitted to the t test and the t test on ranks, which yields the same results as MWW. The results showed that the two tests had equivalent power for most of the pairs. MWW had a power advantage when one of the samples was drawn from a skewed or peaked distribution. Strong power differences between the t test and MWW occurred when one of the samples was drawn from a multimodal distribution. Notably, the Type I error rate of both methods was never more than 3{\%} above the nominal rate of 5{\%}, even not when sample sizes were highly unequal. In conclusion, for fivepoint Likert items, the t test and MWW generally have similar power, and researchers do not have to worry about finding a difference whilst there is none in the population. Likert scales are widely used in various domains such as behavioral sciences, healthcare, marketing, and usability research. When responding to a Likert scale, participants specify their level of agreement to statements with typically five or seven ordered response levels. Likert item data have distinct characteristics: discrete instead of continuous values, tied numbers, and restricted range.},
annote = {t-test robust to likert scale data, or even preferred over non-parametric test},
author = {{De Winter}, Joost C F and Dodou, Dimitra},
file = {:Users/tim/Surfdrive/Research/Library/Literature/De Winter, Dodou - 2010 - Five Point Likert Items t test versus Mann Whitney Wilcoxon.pdf:pdf},
issn = {15317714},
journal = {Pract. Assessment, Res. Eval.},
keywords = {Comparative Analysis,Error Patterns,Evaluation Methods,Likert Scales,Nonparametric Statistics,Questionnaires,Statistical Analysis},
number = {11},
pages = {1--16},
title = {{Five Point Likert Items: t test versus Mann Whitney Wilcoxon}},
url = {https://pareonline.net/pdf/v15n11.pdf},
volume = {15},
year = {2010}
}
@article{Singh2018b,
abstract = {Rankings are ubiquitous in the online world today. As we have transitioned from finding books in libraries to ranking products, jobs, job applicants, opinions and potential romantic partners, there is a substantial precedent that ranking systems have a responsibility not only to their users but also to the items being ranked. To address these often conflicting responsibilities, we propose a conceptual and computational framework that allows the formulation of fairness constraints on rankings in terms of exposure allocation. As part of this framework, we develop efficient algorithms for finding rankings that maximize the utility for the user while provably satisfying a specifiable notion of fairness. Since fairness goals can be application specific, we show how a broad range of fairness constraints can be implemented using our framework, including forms of demographic parity, disparate treatment, and disparate impact constraints. We illustrate the effect of these constraints by providing empirical results on two ranking problems.},
archivePrefix = {arXiv},
arxivId = {1802.07281},
author = {Singh, Ashudeep and Joachims, Thorsten},
doi = {10.1145/3219819.3220088},
eprint = {1802.07281},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Singh, Joachims - 2018 - Fairness of exposure in rankings(2).pdf:pdf},
isbn = {9781450355520},
journal = {Proc. ACM SIGKDD Int. Conf. Knowl. Discov. Data Min.},
keywords = {Algorithmic bias,Equal opportunity,Fairness,Fairness in rankings,Position bias},
pages = {2219--2228},
title = {{Fairness of exposure in rankings}},
year = {2018}
}
@article{Severyn2016,
abstract = {In order to successfully apply opinion mining (OM) to the large amounts of user-generated content produced every day, we need robust models that can handle the noisy input well yet can easily be adapted to a new domain or language. We here focus on opinion mining for YouTube by (i) modeling classifiers that predict the type of a comment and its polarity, while distinguishing whether the polarity is directed towards the product or video; (ii) proposing a robust shallow syntactic structure (STRUCT) that adapts well when tested across domains; and (iii) evaluating the effectiveness on the proposed structure on two languages, English and Italian. We rely on tree kernels to automatically extract and learn features with better generalization power than traditionally used bag-of-word models. Our extensive empirical evaluation shows that (i) STRUCT outperforms the bag-of-words model both within the same domain (up to 2.6{\%} and 3{\%} of absolute improvement for Italian and English, respectively); (ii) it is particularly useful when tested across domains (up to more than 4{\%} absolute improvement for both languages), especially when little training data is available (up to 10{\%} absolute improvement) and (iii) the proposed structure is also effective in a lower-resource language scenario, where only less accurate linguistic processing tools are available.},
author = {Severyn, Aliaksei and Moschitti, Alessandro and Uryupina, Olga and Plank, Barbara and Filippova, Katja},
doi = {10.1016/j.ipm.2015.03.002},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Severyn et al. - 2016 - Multi-lingual opinion mining on YouTube.pdf:pdf},
issn = {03064573},
journal = {Inf. Process. Manag.},
keywords = {Natural Language Processing,Opinion mining,Social media},
number = {1},
pages = {46--60},
publisher = {Elsevier B.V.},
title = {{Multi-lingual opinion mining on YouTube}},
url = {http://dx.doi.org/10.1016/j.ipm.2015.03.002},
volume = {52},
year = {2016}
}
@article{Appelbaum2008,
abstract = {Standards recommended some modifications to the original standards. Examples of modifications include division of hypotheses, analyses, and conclusions into 3 groupings (primary, secondary, and exploratory) and some changes to the section on meta-analysis. Several new modules are included that report standards for observational studies, clinical trials, longitudinal studies, replication studies, and N-of-1 studies. In addition, standards for analytic methods with unique characteristics and output (structural equation modeling and Bayesian analysis) are included. These proposals were accepted by the Publications and Communications Board of APA and supersede the standards included in the 6th edition of the Publication Manual of the American Psychological Association (APA, 2010).},
author = {Appelbaum, Mark and Cooper, Harris and Kline, Rex B and Mayo-Wilson, Evan and Nezu, Arthur M and Rao, Stephen M},
doi = {10.1037/amp0000191},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Appelbaum et al. - 2008 - Communications Board Task Force Report.pdf:pdf},
isbn = {0022-4537},
issn = {1935-990X},
journal = {Commun. Board Work. Gr. J. Artic. Report. Stand.},
keywords = {APA Style,meta-analysis,reporting standards,research methods},
number = {1},
pages = {3--25},
pmid = {29345484},
title = {{Communications Board Task Force Report}},
url = {http://dx.doi.org/10.1037/amp0000191},
volume = {73},
year = {2008}
}
@article{Wang2018,
abstract = {A well-known challenge in learning from click data is its inherent bias and most notably position bias. Traditional click models aim to extract the (query, document) relevance and the estimated bias is usually discarded after relevance is extracted. In contrast, the most recent work on unbiased learning-to-rank can effectively leverage the bias and thus focuses on estimating bias rather than relevance [20, 31]. Existing approaches use search result randomization over a small percentage of production traffic to estimate the position bias. This is not desired because result randomization can negatively impact users' search experience. In this paper, we compare different schemes for result randomization (i.e., RandTopN and RandPair) and show their negative effect in personal search. Then we study how to infer such bias from regular click data without relying on randomization. We propose a regressionbased Expectation-Maximization (EM) algorithm that is based on a position bias click model and that can handle highly sparse clicks in personal search. We evaluate our EM algorithm and the extracted bias in the learning-to-rank setting. Our results show that it is promising to extract position bias from regular clicks without result randomization. The extracted bias can improve the learning-to-rank algorithms significantly. In addition, we compare the pointwise and pairwise learning-to-rank models. Our results show that pairwise models are more effective in leveraging the estimated bias.},
author = {Wang, Xuanhui and Golbandi, Nadav and Bendersky, Michael and Metzler, Donald and Najork, Marc},
doi = {10.1145/3159652.3159732},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Wang et al. - 2018 - Position bias estimation for unbiased learning to rank in personal search.pdf:pdf},
isbn = {9781450355810},
journal = {WSDM 2018 - Proc. 11th ACM Int. Conf. Web Search Data Min.},
keywords = {Expectation-maximization,Inverse propensity weighting,Position bias estimation},
pages = {610--618},
title = {{Position bias estimation for unbiased learning to rank in personal search}},
volume = {2018-Febua},
year = {2018}
}
@article{Chang2009,
abstract = {Probabilistic topic models are a popular tool for the unsupervised analysis of text, providing both a predictive model of future text and a latent topic representation of the corpus. Practitioners typically assume that the latent space is semantically meaningful. It is used to check models, summarize the corpus, and guide exploration of its contents. However, whether the latent space is interpretable is in need of quantitative evaluation. In this paper, we present new quantitative methods for measuring semantic meaning in inferred topics. We back these measures with large-scale user studies, showing that they capture aspects of the model that are undetected by previous measures of model quality based on held-out likelihood. Surprisingly, topic models which perform better on held-out likelihood may infer less semantically meaningful topics.},
author = {Chang, Jonathan and Boyd-Graber, Jordan and Gerrish, Sean and Wang, Chong and Blei, David M.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Chang et al. - 2009 - Reading tea leaves How humans interpret topic models.pdf:pdf},
isbn = {9781615679119},
journal = {Adv. Neural Inf. Process. Syst. 22 - Proc. 2009 Conf.},
pages = {288--296},
title = {{Reading tea leaves: How humans interpret topic models}},
year = {2009}
}
@article{Granka2004,
abstract = {We investigate how users interact with the results page of a WWW search engine using eye-tracking. The goal is to gain insight into how users browse the presented abstracts and how they select links for further exploration. Such understanding is valuable for improved interface design, as well as for more accurate interpretations of implicit feedback (e.g. clickthrough) for machine learning. The following presents initial results, focusing on the amount of time spent viewing the presented abstracts, the total number of abstract viewed, as well as measures of how thoroughly searchers evaluate their results set.},
author = {Granka, Laura A. and Joachims, Thorsten and Gay, Geri},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Granka, Joachims, Gay - 2004 - Eye-tracking analysis of user behavior in WWW search.pdf:pdf},
isbn = {1581138814},
journal = {Proc. Sheff. SIGIR - Twenty-Seventh Annu. Int. ACM SIGIR Conf. Res. Dev. Inf. Retr.},
keywords = {Eye-Tracking,Implicit Feedback,WWW Search},
pages = {478--479},
title = {{Eye-tracking analysis of user behavior in WWW search}},
year = {2004}
}
@article{Otterbacher2018,
abstract = {There is growing evidence that search engines produce results that are socially biased, reinforcing a view of the world that aligns with prevalent social stereotypes. One means to promote greater transparency of search algorithms - which are typically complex and proprietary - is to raise user awareness of biased result sets. However, to date, little is known concerning how users perceive bias in search results, and the degree to which their perceptions differ and/or might be predicted based on user attributes. One particular area of search that has recently gained attention, and forms the focus of this study, is image retrieval and gender bias. We conduct a controlled experiment via crowdsourcing using participants recruited from three countries to measure the extent to which workers perceive a given image results set to be subjective or objective. Demographic information about the workers, along with measures of sexism, are gathered and analysed to investigate whether (gender) biases in the image search results can be detected. Amongst other findings, the results confirm that sexist people are less likely to detect and report gender biases in image search results.},
annote = {here the authors looked at how different people perceive gender bias in image search;

that is, they assessed levels of sexism in participants and then looked whether that is related to judging image results sets;

the results also showed that sexist people are less likely to report a gender bias},
author = {Otterbacher, Jahna and Checco, Alessandro and Demartini, Gianluca and Clough, Paul},
doi = {10.1145/3209978.3210094},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Otterbacher et al. - 2018 - Investigating user perception of gender bias in image search The role of sexism.pdf:pdf},
isbn = {9781450356572},
journal = {41st Int. ACM SIGIR Conf. Res. Dev. Inf. Retrieval, SIGIR 2018},
keywords = {Gender stereotypes,Search engine bias,User perceptions},
pages = {933--936},
title = {{Investigating user perception of gender bias in image search: The role of sexism}},
year = {2018}
}
@inproceedings{Draws2020helping,
author = {Draws, Tim and Liu, Jody and Tintarev, Nava},
booktitle = {Int. Conf. Data Min. Work.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Draws, Liu, Tintarev - Unknown - Helping users discover perspectives Enhancing opinion mining with joint topic models.pdf:pdf},
keywords = {debated topics,els,joint topic mod-,perspective discovery,sentiment analysis,topic modeling},
publisher = {IEEE},
title = {{Helping users discover perspectives : Enhancing opinion mining with joint topic models}}
}
@article{Oosterhuis2018,
abstract = {Learning to Rank has traditionally considered settings where given the relevance information of objects, the desired order in which to rank the objects is clear. However, with today's large variety of users and layouts this is not always the case. In this paper, we consider so-called complex ranking settings where it is not clear what should be displayed, that is, what the relevant items are, and how they should be displayed, that is, where the most relevant items should be placed. These ranking settings are complex as they involve both traditional ranking and inferring the best display order. Existing learning to rank methods cannot handle such complex ranking settings as they assume that the display order is known beforehand. To address this gap we introduce a novel Deep Reinforcement Learning method that is capable of learning complex rankings, both the layout and the best ranking given the layout, from weak reward signals. Our proposed method does so by selecting documents and positions sequentially, hence it ranks both the documents and positions, which is why we call it the Double Rank Model (DRM). Our experiments show that DRM outperforms all existing methods in complex ranking settings, thus it leads to substantial ranking improvements in cases where the display order is not known a priori.},
annote = {authors formalize the complex ranking setting, in which not just relevance but also position is taken into account; that is, in some UIs, users are not (position) biased top to bottom, but for example right to left or center-biased

they propose an algorithm that can learn positions and relevance at the same time so that documents can be put in the positions that correspond with user attention},
archivePrefix = {arXiv},
arxivId = {1805.02404},
author = {Oosterhuis, Harrie and {De Rijke}, Maarten},
doi = {10.1145/3209978.3209992},
eprint = {1805.02404},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Oosterhuis, De Rijke - 2018 - Ranking for relevance and display preferences in complex presentation layouts.pdf:pdf},
isbn = {9781450356572},
journal = {41st Int. ACM SIGIR Conf. Res. Dev. Inf. Retrieval, SIGIR 2018},
keywords = {Complex ranking,Deep reinforcement learning,Learning to rank},
pages = {845--854},
title = {{Ranking for relevance and display preferences in complex presentation layouts}},
year = {2018}
}
@article{Arnold2019,
abstract = {Accuracy is an important concern for suppliers of artificial intelligence (AI) services, but considerations beyond accuracy, such as safety (which includes fairness and explainability), security, and provenance, are also critical elements to engender consumers' trust in a service. Many industries use transparent, standardized, but often not legally required documents called supplier's declarations of conformity (SDoCs) to describe the lineage of a product along with the safety and performance testing it has undergone. SDoCs may be considered multidimensional fact sheets that capture and quantify various aspects of the product and its development to make it worthy of consumers' trust. In this article, inspired by this practice, we propose FactSheets to help increase trust in AI services. We envision such documents to contain purpose, performance, safety, security, and provenance information to be completed by AI service providers for examination by consumers. We suggest a comprehensive set of declaration items tailored to AI in the Appendix of this article.},
archivePrefix = {arXiv},
arxivId = {1808.07261},
author = {Arnold, M. and Piorkowski, D. and Reimer, D. and Richards, J. and Tsay, J. and Varshney, K. R. and Bellamy, R. K.E. and Hind, M. and Houde, S. and Mehta, S. and Mojsilovic, A. and Nair, R. and Ramamurthy, K. Natesan and Olteanu, A.},
doi = {10.1147/JRD.2019.2942288},
eprint = {1808.07261},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Arnold et al. - 2019 - FactSheets Increasing trust in AI services through supplier's declarations of conformity.pdf:pdf},
issn = {21518556},
journal = {IBM J. Res. Dev.},
number = {4-5},
title = {{FactSheets: Increasing trust in AI services through supplier's declarations of conformity}},
volume = {63},
year = {2019}
}
@article{Yom-Tov2014,
abstract = {The ability of modern web services such as news aggregators and search engines to tailor their results to the tastes of individuals, together with people's preference for reading opinions which reinforce their own viewpoints, have raised concerns that people are nowadays exposed to a narrow range of view-points, a phenomenon referred to as the "filter bubble". In this paper we focus on increasing exposure to varied political opinions with a goal of improving civil discourse. We develop a method to algorithmically encourage people to read diverse political opinions and test it when people actively seek information. First, analyzing data from a popular search engine we show that people are indeed more likely to read opinions consistent with their own. Interestingly, they are more likely to read news from opposing sites when the language model of a particular news item is close to the language model of their own political leaning. Based on this finding, we describe a method for assisting people to read divergent opinions by choosing documents of opposing viewpoints that have a language model closer to their own language model. We test our method on a number of web searchers and show that pages of the opposing side which were more similar than the average persons' own language model tended to be clicked 38{\%} more than those below. We also describe the long-term effects of our method, showing that people who were shown more diverse results continued reading more diverse results and overall became more interested in news.},
annote = {unfortunately badly written; but this paper is quite cool -- the authors talk about the effects of intermingling opposing viewpoints in search results (democratic vs republican in the US)

their method: 
- people receive a score of political leaning based on their zip code based on how they voted; for example if 100{\%} of people in a zip code voted democratic, everyone from that zip code got a score of s{\_}i = 1.00
- each news site URL received a score based on the average of all queries that led to a click on that site; for example if 5 people clicked on a link to a particular news outlet based on the queries they issued, and their scores were [.2, .2, .4, .6, .6], the news outlet would receive a score of .4
- this was based on almost 200.000 queries and more than 23.000 news pages
- for each news page, a vector space model (weighted by TF-IDF) was created using the entire text of the page
- people who clicked on links that had an average score above (below) the average of all news outlets were considered democratic (republican) (the average was .56)
- based on person scores, they later also scored queries on political leaning; this way they were able to mingle the results of democratic queries into republican ones and vice versa (this makes at least some sense because depending on what people click on given a query, different content will be judged as relevant)
- taking the average of all vector space models for the two political leanings, the authors computed overall language models for democratic and republican content
- they had a control and a treatment group; control got normal search results, treatment got search results with results of opposing viewpoint intermingled at ranks 2, 4, 6, and so on; for example the query "obamacare" was scored republican, so they intermingled it with results from the democratic query "affordable care act summary"

Findings:
- people prefer to read news that are closer to their own viewpoint
- people are more likely to read opposing views if the language model of the article containing the opposing view is closer to the overall language model of their preferred view(!)
- long-term effects: people that were shown more diverse results (treatment group) continued reading more diverse news and were more interested in news in general},
author = {Yom-Tov, Elad and Dumais, Susan and Guo, Qi},
doi = {10.1177/0894439313506838},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Yom-Tov, Dumais, Guo - 2014 - Promoting Civil Discourse Through Search Engine Diversity.pdf:pdf},
issn = {15528286},
journal = {Soc. Sci. Comput. Rev.},
keywords = {diversity,filter bubble,information retrieval,media bias,political discourse,search engines,selective exposure},
number = {2},
pages = {145--154},
title = {{Promoting Civil Discourse Through Search Engine Diversity}},
volume = {32},
year = {2014}
}
@article{MohamadAli2018,
author = {{Mohamad Ali}, Nazlena and {Wan Ahmad}, Wan Nooraishya},
doi = {10.1504/ijbis.2018.10009818},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Mohamad Ali, Wan Ahmad - 2018 - A User Study on Trust Perception in Persuasive Technology.pdf:pdf},
issn = {1746-0972},
journal = {Int. J. Bus. Inf. Syst.},
number = {1},
pages = {1},
title = {{A User Study on Trust Perception in Persuasive Technology}},
volume = {29},
year = {2018}
}
@article{Haim2018,
abstract = {In offering personalized content geared towards users' individual interests, recommender systems are assumed to reduce news diversity and thus lead to partial information blindness (i.e., filter bubbles). We conducted two exploratory studies to test the effect of both implicit and explicit personalization on the content and source diversity of Google News. Except for small effects of implicit personalization on},
annote = {this is mostly about source {\&} topic diversity in RS... not really useful},
author = {Haim, Mario and Graefe, Andreas and Brosius, Hans Bernd},
doi = {10.1080/21670811.2017.1338145},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Haim, Graefe, Brosius - 2018 - Burst of the Filter Bubble Effects of personalization on the diversity of Google News.pdf:pdf},
issn = {2167082X},
journal = {Digit. Journal.},
keywords = {diversity,experiment,filter bubble,online news,personalization},
number = {3},
pages = {330--343},
publisher = {Routledge},
title = {{Burst of the Filter Bubble?: Effects of personalization on the diversity of Google News}},
volume = {6},
year = {2018}
}
@book{Cambria2017,
abstract = {Sentiment lexicons and datasets represent the knowledge base that lies at the foundation of a SA system. In its simplest form, a sentiment lexicon is a repository of words/phrases labelled with sentiment. Similarly, a sentimentannotated dataset consists of documents (tweets, sentences or longer documents) labelled with one or more sentiment labels. This chapter explores the philosophy, execution and utility of popular sentiment lexicons and datasets. We describe different labelling schemes that may be used.We then provide a detailed description of existing sentiment and emotion lexicons, and the trends underlying research in lexicon generation. This is followed by a survey of sentiment-annotated datasets and the nuances of labelling involved. We then show how lexicons and datasets created for one language can be transferred to a new language. Finally, we place these sentiment resources in the perspective of their classic applications to sentiment analysis.},
doi = {10.1007/978-3-319-55394-8_5},
editor = {Cambria, Erik and Das, Dipankar and Bandyopadhyay, Sivaji and Feraco, Antonio},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Unknown - 2017 - A Practical Guide to Sentiment Analysis.pdf:pdf},
isbn = {9783319553924},
title = {{A Practical Guide to Sentiment Analysis}},
year = {2017}
}
@incollection{bandwagonEffect2006colman,
address = {Oxford},
author = {Colman, Andrew M.},
booktitle = {A Dict. Psychol.},
edition = {2},
pages = {78},
publisher = {Oxford University Press},
title = {{Bandwagon effect}},
url = {https://archive.org/details/dictionaryofpsyc00colm{\_}0/page/78/mode/2up},
year = {2006}
}
@article{Fokkens2019,
abstract = {Research from communication science has shown that stereotypical ideas are often reflected in language use. Media coverage of different groups in society influences the perception people have about these groups and even increases distrust and polarization among different groups. Investigating the forms of (especially subtle) stereotyping can raise awareness to journalists and help prevent reinforcing oppositions between groups in society. Conducting large-scale, deep investigations to determine whether we are faced with stereotyping is time-consuming and costly. We propose to tackle this challenges through the means of microportraits: an impression of a target group or individual conveyed in a single text. We introduce the first system implementation for Dutch and show that microportraits allow social scientists to explore various dimensions of stereotyping. We explore the possibilities provided by microportraits by investigating stereotyping of Muslims in the Dutch media. Our (preliminary) results show that microportraits provide more detailed insights into stereotyping compared to more basic models such as word clouds.},
author = {Fokkens, Antske and Ruigrok, Nel and Beukeboom, Camiel and Gagestein, Sarah and {Van Atteveldt}, Wouter},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Fokkens et al. - 2019 - Studying muslim stereotyping through microportrait extraction.pdf:pdf},
isbn = {9791095546009},
journal = {Lr. 2018 - 11th Int. Conf. Lang. Resour. Eval.},
keywords = {Digital social science,Stereotyping,Text analysis},
pages = {3734--3741},
title = {{Studying muslim stereotyping through microportrait extraction}},
year = {2019}
}
@article{Kulshrestha2019,
abstract = {Users frequently use search systems on the Web as well as online social media to learn about ongoing events and public opinion on personalities. Prior studies have shown that the top-ranked results returned by these search engines can shape user opinion about the topic (e.g., event or person) being searched. In case of polarizing topics like politics, where multiple competing perspectives exist, the political bias in the top search results can play a significant role in shaping public opinion towards (or away from) certain perspectives.},
annote = {authors classified all media outlet as either supportive, neutral, or opposing democrats and republicans, and then checked if twitter and google search results contain more links of one of the group

they found that both the input data as well as the ranking algorithm are responsible for bias in the final search result

basically they just assigned every person and media to either having a democrat or republican bias (or being neutral); and then checked if both occur equally},
author = {Kulshrestha, Juhi and Eslami, Motahhare and Messias, Johnnatan and Zafar, Muhammad Bilal and Ghosh, Saptarshi and Gummadi, Krishna P. and Karahalios, Karrie},
doi = {10.1007/s10791-018-9341-2},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Kulshrestha et al. - 2019 - Search bias quantification investigating political bias in social media and web search.pdf:pdf},
issn = {15737659},
journal = {Inf. Retr. J.},
keywords = {Political bias inference,Search bias,Search bias quantification,Social media search,Sources of search bias,Web search},
number = {1-2},
pages = {188--227},
publisher = {Springer Netherlands},
title = {{Search bias quantification: investigating political bias in social media and web search}},
volume = {22},
year = {2019}
}
@misc{Lieber2014,
annote = {this article explains what a robo-advisor is and how/why they are on the rise},
author = {Lieber, Ron},
booktitle = {New York Times},
month = {apr},
title = {{Financial Advice for People Who Aren't Rich}},
url = {https://www.nytimes.com/2014/04/12/your-money/start-ups-offer-financial-advice-to-people-who-arent-rich.html},
year = {2014}
}
@article{Moller2018,
abstract = {ABSTRACTIn the debate about filter bubbles caused by algorithmic news recommendation, the conceptualization of the two core concepts in this debate, diversity and algorithms, has received little attention in social scientific research. This paper examines the effect of multiple recommender systems on different diversity dimensions. To this end, it maps different values that diversity can serve, and a respective set of criteria that characterizes a diverse information offer in this particular conception of diversity. We make use of a data set of simulated article recommendations based on actual content of one of the major Dutch broadsheet newspapers and its users (N=21,973 articles, N=500 users). We find that all of the recommendation logics under study proved to lead to a rather diverse set of recommendations that are on par with human editors and that basing recommendations on user histories can substantially increase topic diversity within a recommendation set.},
annote = {this paper is nice to establish that we don't need to worry about content diversity, RS are usually stable with that

M{\"{o}}ller et al. (2018) examined the effect of several RS's on different diversity dimensions. The authors discuss diversity as one of the core public values in media law and policy, and present a discussion similar to the one of Nguyen et al. (2014), concluding that so far, filter bubbles do not really exist as audiences still largely overlap between different media outlets (citing Fletcher {\&} Nielsen, 2017; although their study is more about news sources and the results are not very convincing). 

To test the effect of RS's on diversity, the authors first mapped different values that diversity can serve, including topic, tone, category, and tags (thus, they didn't look at viewpoint diversity). They looked at news recommendation for articles of one single newspaper, the Dutch Volkskrant, testing 7 different recommender methods including overall popularity and collaborative filtering. The authors found that the studied RS's yield diverse sets of recommendations that are on par with human editors (is that really surprising if you only consider one newspaper?). They claim that basing recommendations on past user behaviour (i.e., user-based collaborative filtering) can increase topic diversity.},
author = {M{\"{o}}ller, Judith and Trilling, Damian and Helberger, Natali and van Es, Bram},
doi = {10.1080/1369118X.2018.1444076},
file = {:Users/tim/Surfdrive/Research/Library/Literature/M{\"{o}}ller et al. - 2018 - Do not blame it on the algorithm an empirical assessment of multiple recommender systems and their impact on con.pdf:pdf},
issn = {14684462},
journal = {Inf. Commun. Soc.},
keywords = {News,automated content classification,diversity metrics,filter bubbles,recommender systems},
number = {7},
pages = {959--977},
publisher = {Taylor {\&} Francis},
title = {{Do not blame it on the algorithm: an empirical assessment of multiple recommender systems and their impact on content diversity}},
volume = {21},
year = {2018}
}
@article{Granka2010,
abstract = {In 'Shaping the Web: Why the Politics of Search Engines Matters,' Introna and Nissenbaum (2000) introduced scholars to the political, as well as technical, issues central to the development of online search engines. Since that time, scholars have critically evaluated the role that search engines play in structuring the scope of online information access for the rest of society, with an emphasis on the implications for a democratic and diverse Web. This article describes the thought behind search engine regulation, online diversity, and information bias, and it places these issues within the context of the technical and societal changes that have occurred in the online search industry. The author assesses which of the initial concerns expressed about online search engines remain relevant today and discusses how technical changes demand a new approach to measuring online diversity and democracy. The author concludes with a proposal to direct the research and thought in online search going forward. [ABSTRACT FROM AUTHOR]},
author = {Granka, Laura A.},
doi = {10.1080/01972243.2010.511560},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Granka - 2010 - The politics of search A decade retrospective.pdf:pdf},
issn = {01972243},
journal = {Inf. Soc.},
keywords = {Democracy,Diversity,Information retrieval,Internet search,Transparency},
number = {5},
pages = {364--374},
title = {{The politics of search: A decade retrospective}},
volume = {26},
year = {2010}
}
@article{DEZS2012,
abstract = {We argue that female representation in top management brings informational and social diversity benefits to the top management team, enriches the behaviors exhibited by managers throughout the firm, and motivates women in middle management. The result should be improved managerial task performance and thus better firm performance. We test our theory using 15 years of panel data on the top management teams of the S{\&}P 1,500 firms. We find that female representation in top management improves firm performance but only to the extent that a firm's strategy is focused on innovation, in which context the informational and social benefits ofgender diversity and the behaviors associated with women in management are likely to be especially important for managerial task performance.},
author = {Dezs, Christian L. and Ross, David Gaddis},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Dezs, Ross - 2012 - Does female representation in top management improve firm performance A panel data investigation.pdf:pdf},
journal = {Strateg. Manag. J.},
keywords = {business,business groups,capital,correspondence to,e-mail,gachibowli,hyderabad - 500032,india,indian school of,institutional voids,market efficiency,organizational structure,raveendra chittoor},
pages = {1072--1089},
title = {{Does female representation in top management improve firm performance? A panel data investigation}},
volume = {33},
year = {2012}
}
@article{Puschmann2018,
abstract = {Search engines are among the most popular online services used in a range of contexts, including to find information on political issues. As such, they increasingly act as powerful mediators between news organizations and their audiences. The claim that search results are politically biased, while hardly new, has also recently received fresh support from President Donald Trump, who has blamed Google for unfairly prioritizing news outlets critical of his policies. In the context of elections, search engines may serve to inform citizens and have been argued to sway the choices of undecided voters. I examine two related issues: How political parties and candidates are represented in Google Search results and how strongly results in both Google Search and Google News are personalized in the run up to the 2017 German general elections. My results suggest that some parties and candi- dates are able to exert greater influence over how they are repre- sented in search results than others, through a combination of local branch websites and social media presences. I furthermore find only a small share of results which differ from the main- stream, while controlling for time, language, and location, calling into question the validity of the filter bubble concept.},
annote = {this paper is nice because it is about IR instead of recommender systems; however it only explores source and topic diversity},
author = {Puschmann, Cornelius},
doi = {10.1080/21670811.2018.1539626},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Puschmann - 2018 - Beyond the Bubble Assessing the Diversity of Political Search Results.pdf:pdf},
issn = {2167082X},
journal = {Digit. Journal.},
keywords = {Bias,Germany,algorithms,elections,filter bubble,search engines},
pages = {1--20},
publisher = {Routledge},
title = {{Beyond the Bubble: Assessing the Diversity of Political Search Results}},
year = {2018}
}
@article{Olson2007,
abstract = {Basing their hypotheses on information processing theory, the authors incorporate important group processes within strategic decision making. They examine the interrelationships of cognitive diversity, task conflict, and competence-based trust and their effects on decision outcomes. Their survey includes top management teams from 85 U.S. hospitals. They found that cognitive diversity has a strong positive relationship with task conflict and that competence-based trust strengthens this relationship. In addition, these results suggest that task conflict mediates the effects of cognitive diversity on decision outcomes. {\textcopyright} 2007 Sage Publications.},
annote = {Cognitive diversity is positively related to decision quality in teams},
author = {Olson, Bradley J. and Parayitam, Satyanarayana and Bao, Yongjian},
doi = {10.1177/0149206306298657},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Olson, Parayitam, Bao - 2007 - Strategic decision making The effects of cognitive diversity, conflict, and trust on decision outcomes.pdf:pdf},
issn = {01492063},
journal = {J. Manage.},
keywords = {Conflict,Diversity,Executive decision making,Trust},
number = {2},
pages = {196--222},
title = {{Strategic decision making: The effects of cognitive diversity, conflict, and trust on decision outcomes}},
volume = {33},
year = {2007}
}
@inproceedings{Lurie2020,
address = {New York, NY, USA},
annote = {this is not about ranking bias, but about how people use search engines in a biased way; this is a qualitative analysis of a few data sets containing political queries etc.},
author = {Mustafaraj, Eni and Lurie, Emma and Devine, Claire},
booktitle = {Conf. Fairness, Accountability, andTransparency},
doi = {10.1145/3351095.3372835},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Mustafaraj, Lurie, Devine - 2020 - The Case for Voter-Centered Audits of Search Engines During Political Elections.pdf:pdf},
isbn = {9781450369367},
keywords = {Google,algorithm audits,search engines,voters},
pages = {559--569},
publisher = {Association for Computing Machinery},
series = {FAT* '20},
title = {{The Case for Voter-Centered Audits of Search Engines During Political Elections}},
year = {2020}
}
@article{Liu2018,
abstract = {Detecting topics from Twitter has been widely studied for understanding social events. There are two types of topics, i.e., global topics attracting widespread tweets with larger volume and local topics drawing attention of limited tweets of somewhere. However, most of existent works neglect the difference between them and suffer from the Long Tail Effect, resulting in the inability to detect the local one. In this paper, we distinguish global and local topics by associating each tweet with both of them simultaneously. We propose a probabilistic graphical model to extract global and local topics related to social events in a unified framework at the same time. Our model learns global topics using tweets scattered around all locations, while studies local topics merely utilizing tweets within the corresponding location. We collect two tweet datasets on Twitter from several cities in USA and evaluate our model over them. The experimental results show significant improvement of our model compared to baseline methods.},
author = {Liu, Huan and Ge, Yong and Zheng, Qinghua and Lin, Rongcheng and Li, Huayu},
doi = {10.1016/j.neucom.2017.07.056},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Liu et al. - 2018 - Detecting global and local topics via mining twitter data.pdf:pdf},
issn = {18728286},
journal = {Neurocomputing},
keywords = {Global and local topic,Probabilistic graphical model,Social event,Twitter},
pages = {120--132},
publisher = {Elsevier B.V.},
title = {{Detecting global and local topics via mining twitter data}},
volume = {273},
year = {2018}
}
@article{Bozdag2015,
abstract = {Online web services such as Google and Facebook started using personalization algorithms. Because information is customized per user by the algorithms of these services, two users who use the same search query or have the same friend list may get different results. Online services argue that by using personalization algorithms, they may show the most relevant information for each user, hence increasing user satisfaction. However, critics argue that the opaque filters used by online services will only show agreeable political viewpoints to the users and the users never get challenged by opposing perspectives. Considering users are already biased in seeking like-minded perspectives, viewpoint diversity will diminish and the users may get trapped in a “filter bubble”. This is an undesired behavior for almost all democracy models. In this thesis we first analyzed the filter bubble phenomenon conceptually, by identifying internal processes and factors in online web services that might cause filter bubbles. Later, we analyzed this issue empirically. We first studied existing metrics in viewpoint diversity research of the computer science literature. We also extended these metrics by adding a new one, namely minority access from media and communication studies. After conducting an empirical study for Dutch and Turkish Twitter users, we showed that minorities cannot reach a large percentage of users in Turkish Twittersphere. We also analyzed software tools and design attempts to combat filter bubbles. We showed that almost all of the tools implement norms required by two popular democracy models. We argue that democracy is essentially a contested concept, and other less popular democracy models should be included in the design of such tools as well.},
annote = {chapter 3 is on viewpoint diversity in social networks!},
author = {Bozdag, Engin},
doi = {10.4233/uuid:87bde0a2-c391-4c77-8457-97cba93abf45},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Bozdag - 2015 - Bursting the Filter Bubble Democracy, Design, and Ethics.pdf:pdf},
journal = {Repository.Tudelft.Nl},
title = {{Bursting the Filter Bubble: Democracy, Design, and Ethics}},
url = {http://repository.tudelft.nl/view/ir/uuid:87bde0a2-c391-4c77-8457-97cba93abf45/{\%}0Ahttp://repository.tudelft.nl/islandora/object/uuid:87bde0a2-c391-4c77-8457-97cba93abf45/datastream/OBJ/download},
year = {2015}
}
@article{Desmet2016,
abstract = {This paper introduces Pick-A-Mood, a character-based pictorial scale for reporting and expressing moods. Pick-A-Mood consists of three characters that each express eight mood states, representing four main categories: excited and cheerful (for energised-pleasant), irritated and tense (for energised-unpleasant), relaxed and calm (for calm-pleasant), and bored and sad (for calm-unpleasant). Using Pick-A-Mood requires little effort on the part of respondents, making it suitable for design research applications in which people often have little time or motivation to report their moods. Contrary to what is often assumed, mood and emotion are distinct phenomena with different measurable manifestations. These differences are discussed, and a review of existing methods is provided, indicating to what extent current methods that measure emotion are suitable for measuring mood. The development and validation of Pick-A-Mood is reported, and application examples and research opportunities are discussed. Keywords: mood measurement; design for mood; measurement method review; pictorial affect scale. Reference to this paper should be made as follows: Desmet, P.M.A., Vastenburg, M.H. and Romero, N. (2016) 'Mood measurement with Pick-A-Mood: review of current methods and design of a pictorial self-report scale',},
author = {Desmet, Pieter M.A. and Romero, Natalia and Vastenburg, Martijn H.},
doi = {10.1504/jdr.2016.10000563},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Desmet, Romero, Vastenburg - 2016 - Mood measurement with Pick-A-Mood review of current methods and design of a pictorial self-report sc.pdf:pdf},
issn = {1748-3050},
journal = {J. Des. Res.},
number = {3},
pages = {241},
title = {{Mood measurement with Pick-A-Mood: review of current methods and design of a pictorial self-report scale}},
volume = {14},
year = {2016}
}
@article{Bucinca2020,
abstract = {Explainable artificially intelligent (XAI) systems form part of sociotechnical systems, e.g., human+AI teams tasked with making decisions. Yet, current XAI systems are rarely evaluated by measuring the performance of human+AI teams on actual decision-making tasks. We conducted two online experiments and one in-person think-aloud study to evaluate two currently common techniques for evaluating XAI systems: (1) using proxy, artificial tasks such as how well humans predict the AI's decision from the given explanations, and (2) using subjective measures of trust and preference as predictors of actual performance. The results of our experiments demonstrate that evaluations with proxy tasks did not predict the results of the evaluations with the actual decision-making tasks. Further, the subjective measures on evaluations with actual decision-making tasks did not predict the objective performance on those same tasks. Our results suggest that by employing misleading evaluation methods, our field may be inadvertently slowing its progress toward developing human+AI teams that can reliably perform better than humans or AIs alone.},
annote = {AI Decision support systems are often evaluated using either proxy tasks ("can you say what the AI would predict here?") or subjective measures (trust etc.) -- these authors test two different styles of AI Decision support systems, inductive and deductive, in terms of these evaluations 

in a second study, they then test these same AI styles in an actual decision task and look at what people really use

they find that although people prefer the inductive style according to the common evaluations, they seem to prefer the deductive style when they actually have to make the decisions; this mismatch could have to do with different focuses in these evaluations

however, there are many problems here:
- p-values not corrected for multiple testing
- reporting of 'marginal significance'
- low sample sizes and odd participant allocation in study 2
- and IMPORTANTLY: why does study 1 not predict the results in study 2? just because these two independent studies have contradictory results doesn't mean that there is no predictive power, that should be tested as well

interesting paper and well-structured, but the data analysis is bad},
archivePrefix = {arXiv},
arxivId = {2001.08298},
author = {Bu{\c{c}}inca, Zana and Lin, Phoebe and Gajos, Krzysztof Z. and Glassman, Elena L.},
doi = {10.1145/3377325.3377498},
eprint = {2001.08298},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Bu{\c{c}}inca et al. - 2020 - Proxy tasks and subjective measures can be misleading in evaluating explainable AI systems.pdf:pdf},
isbn = {9781450371186},
journal = {Int. Conf. Intell. User Interfaces, Proc. IUI},
keywords = {artificial intelligence,explanations,trust},
pages = {454--464},
title = {{Proxy tasks and subjective measures can be misleading in evaluating explainable AI systems}},
year = {2020}
}
@article{Mary2019,
abstract = {We address the problem of algorithmic fairness: ensuring that the outcome of a classifier is not biased towards certain values of sensitive variables such as age, race or gender. As common fairness metrics can be expressed as measures of (conditional) independence between variables, we propose to use the R{\'{e}}nyi maximum correlation coefficient to generalize fairness measurement to continuous variables. We exploit Witsenhausen's characterization of the R{\'{e}}nyi correlation coefficient to propose a differentiable implementation linked to {\$}f{\$}-divergences. This allows us to generalize fairness-aware learning to continuous variables by using a penalty that upper bounds this coefficient. Theses allows fairness to be extented to variables such as mixed ethnic groups or financial status without thresholds effects. This penalty can be estimated on mini-batches allowing to use deep nets. Experiments show favorable comparisons to state of the art on binary variables and prove the ability to protect continuous ones},
annote = {this is about ML fairness for continuous protected attributes using the Renyi maximum correlation coefficient; 

they handle an equal odds fairness notion and try to quantify independence of protected attribute and outcome variable as a measure of fairness

I can't use this for ranking bias because we don't have the outcome variable (i.e., ranking) but it is interesting for regression ML algorithms},
author = {Mary, J{\'{e}}r{\'{e}}mie Jeremie and Calauz{\`{e}}nes, Cl{\'{e}}ment and Karoui, Noureddine El},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Mary, Calauz{\`{e}}nes, Karoui - 2019 - Fairness-Aware Learning for Continuous Attributes and Treatments.pdf:pdf},
journal = {Icml},
pages = {4382--4391},
title = {{Fairness-Aware Learning for Continuous Attributes and Treatments}},
url = {http://proceedings.mlr.press/v97/mary19a.html{\%}0Ahttps://github.com/},
volume = {97},
year = {2019}
}
@article{Welty2008,
annote = {adopting metrology (science of measurement and application) to evaluate AI systems; we evaluate AI using data sets, but how good are these data sets for such measurements?

they analyze the WordSim data set according to the metrology framework; each subsection of (5) is an element of metrology

we can analyze measurement instruments (e.g., data sets) in this way (metrology) and take precision, resolution, reproducibility into account to see whether they make good measurements},
archivePrefix = {arXiv},
arxivId = {arXiv:1911.01875v1},
author = {Welty, Chris and Paritosh, Praveen and Aroyo, Lora},
eprint = {arXiv:1911.01875v1},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Welty, Paritosh, Aroyo - 2008 - Metrology for AI From Benchmarks to Instruments.pdf:pdf},
title = {{Metrology for AI : From Benchmarks to Instruments}},
year = {2008}
}
@article{Bellamy2019,
abstract = {Fairness is an increasingly important concern as machine learning models are used to support decision making in high-stakes applications such as mortgage lending, hiring, and prison sentencing. This article introduces a new open-source Python toolkit for algorithmic fairness, AI Fairness 360 (AIF360), released under an Apache v2.0 license (https://github.com/ibm/aif360). The main objectives of this toolkit are to help facilitate the transition of fairness research algorithms for use in an industrial setting and to provide a common framework for fairness researchers to share and evaluate algorithms. The package includes a comprehensive set of fairness metrics for datasets and models, explanations for these metrics, and algorithms to mitigate bias in datasets and models. It also includes an interactive Web experience that provides a gentle introduction to the concepts and capabilities for line-of-business users, researchers, and developers to extend the toolkit with their new algorithms and improvements and to use it for performance benchmarking. A built-in testing infrastructure maintains code quality.},
archivePrefix = {arXiv},
arxivId = {arXiv:1810.01943v1},
author = {Bellamy, R. K.E. and Mojsilovic, A. and Nagar, S. and Ramamurthy, K. Natesan and Richards, J. and Saha, D. and Sattigeri, P. and Singh, M. and Varshney, K. R. and Zhang, Y. and Dey, K. and Hind, M. and Hoffman, S. C. and Houde, S. and Kannan, K. and Lohia, P. and Martino, J. and Mehta, S.},
doi = {10.1147/JRD.2019.2942287},
eprint = {arXiv:1810.01943v1},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Bellamy et al. - 2019 - AI Fairness 360 An extensible toolkit for detecting and mitigating algorithmic bias.pdf:pdf},
issn = {21518556},
journal = {IBM J. Res. Dev.},
number = {4-5},
title = {{AI Fairness 360: An extensible toolkit for detecting and mitigating algorithmic bias}},
volume = {63},
year = {2019}
}
@inproceedings{Draws2020assessing,
abstract = {The way pages are ranked in search results influences whether the users of search engines are exposed to more homogeneous, or rather to more diverse viewpoints. However, this viewpoint diversity is not trivial to assess. In this paper we use existing and novel ranking fairness metrics to evaluate viewpoint diversity in search result rankings. We conduct a controlled simulation study that shows how ranking fairness metrics can be used for viewpoint diversity, how their outcome should be interpreted, and which metric is most suitable depending on the situation. This paper lays out important ground work for future research to measure and assess viewpoint diversity in real search result rankings.},
author = {Draws, Tim and Tintarev, Nava and Gadiraju, Ujwal and Bozzon, Alessandro and Timmermans, Benjamin},
booktitle = {Informal Proc. Bias Fairness AI Work. ECML-PKDD (BIAS 2020)},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Draws et al. - 2020 - Assessing Viewpoint Diversity in Search Results Using Ranking Fairness Metrics.pdf:pdf},
keywords = {ranking fairness,viewpoint diversity,web search},
title = {{Assessing Viewpoint Diversity in Search Results Using Ranking Fairness Metrics}},
url = {https://sites.google.com/view/bias-2020},
year = {2020}
}
@article{Krippendorff2004,
abstract = {In a recent article in this journal, Lombard, Snyder-Duch, and Bracken (2002) surveyed 200 content analyses for their reporting of reliability tests, compared the virtues and drawbacks of five popular reliability measures, and proposed guidelines and standards for their use. Their discussion revealed that numerous misconceptions circulate in the content analysis literature regarding how these measures behave and can aid or deceive content analysts in their effort to ensure the reliability of their data. This article proposes three conditions for statistical mea- sures to serve as indices of the reliability of data and examines the mathematical structure and the behavior of the five coefficients discussed by the authors, as well as two others. It compares common beliefs about these coefficients with what they actually do and concludes with alter- native recommendations for testing reliability in content analysis and similar data-making efforts.},
author = {Krippendorff, Klaus},
doi = {10.1111/j.1468-2958.2004.tb00738.x},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Krippendorff - 2004 - Reliability in Content Analysis.pdf:pdf},
issn = {0360-3989},
journal = {Hum. Commun. Res.},
number = {3},
pages = {411--433},
title = {{Reliability in Content Analysis.}},
volume = {30},
year = {2004}
}
@inproceedings{Asudeh2019,
abstract = {Items from a database are often ranked based on a combination of criteria. The weight given to each criterion in the combination can greatly affect the fairness of the produced ranking, for example, preferring men over women. A user may have the flexibility to choose combinations that weigh these criteria differently, within limits. In this paper, we develop a system that helps users choose criterion weights that lead to greater fairness. We consider ranking functions that compute the score of each item as a weighted sum of (numeric) attribute values, and then sort items on their score. Each ranking function can be expressed as a point in a multidimensional space. For a broad range of fairness criteria, including proportionality, we show how to efficiently identify regions in this space that satisfy these criteria. Using this identification method, our system is able to tell users whether their proposed ranking function satisfies the desired fairness criteria and, if it does not, to suggest the smallest modification that does. Our extensive experiments on real datasets demonstrate that our methods are able to find solutions that satisfy fairness criteria effectively (usually with only small changes to proposed weight vectors) and efficiently (in interactive time, after some initial pre-processing).},
archivePrefix = {arXiv},
arxivId = {1712.09752},
author = {Asudeh, Abolfazl and Jagadish, H. V. and Stoyanovich, Julia and Das, Gautam},
booktitle = {Proc. ACM SIGMOD Int. Conf. Manag. Data},
doi = {10.1145/3299869.3300079},
eprint = {1712.09752},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Asudeh et al. - 2019 - Designing fair ranking schemes.pdf:pdf},
isbn = {9781450356435},
keywords = {Data Ethics,Fairness,Responsible Data Management},
pages = {1259--1276},
title = {{Designing fair ranking schemes}},
year = {2019}
}
@article{Sakai2010,
abstract = {Traditional information retrieval research has mostly focussed on satisfying clearly specified information needs. However, in reality, queries are often ambiguous and/or underspeci- fied. In light of this, evaluating search result diversity is beginning to receive attention. We propose simple evalu- ation metrics for diversified Web search results. Our pre- sumptions are that one or more interpretations (or intents) are possible for each given query, and that graded relevance assessments are available for intent-document pairs (as op- posed to query-document pairs). Our goals are (a) to re- trieve documents that cover as many intents as possible; and (b) to rank documents that are highly relevant to more popular intents higher than those that are marginally rele- vant to less popular intents. Unlike the Intent-Aware (IA) metrics proposed by Agrawal et al. , our metrics successfully avoid ignoring minor intents. Unlike $\alpha$ -nDCG proposed by Clarke et al. , our metrics can accomodate (i) which intents are more likely than others for a given query; and (ii) graded relevance within each intent. Furthermore, unlike these ex- isting metrics, our metrics do not require approximation, and they range between 0 and 1. Experiments with the binary-relevance Diversity Task data from the TREC 2009 Web Track suggest that our metrics corrrelate well with ex- isting metrics but can be more intuitive. Hence, we argue that our metrics are suitable for diversity evaluation given either the intent likelihood information or per-intent graded relevance, or preferably both.},
author = {Sakai, Tetsuya and Craswell, Nick and Song, Ruihua and Robertson, Stephen and Dou, Zhicheng and Lin, Chin-yew},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sakai et al. - 2010 - Simple Evaluation Metrics for Diversified Search Results.pdf:pdf},
journal = {EVIA 2010, Tokyo},
keywords = {ambiguity,diversity,evaluation,novelty,test collection},
title = {{Simple Evaluation Metrics for Diversified Search Results}},
year = {2010}
}
@inproceedings{Purpura2011,
author = {Purpura, Stephen and Schwanda, Victoria and Williams, Kaiton and Stubler, William and Sengers, Phoebe},
booktitle = {Proc. SIGCHI Conf. Hum. factors Comput. Syst.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Purpura et al. - 2011 - Fit4Life The Design of a Persuasive Technology Promoting Healthy Behavior and Ideal Weight.pdf:pdf},
isbn = {9781450302678},
pages = {423--432},
title = {{Fit4Life: The Design of a Persuasive Technology Promoting Healthy Behavior and Ideal Weight}},
year = {2011}
}
@inproceedings{Feldman2015,
author = {Feldman, Michael and Friedler, Sorelle A and Moeller, John and Scheidegger, Carlos and Venkatasubramanian, Suresh},
booktitle = {Proc. 21th ACM SIGKDD Int. Conf. Knowl. Discov. data Min.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Feldman et al. - 2015 - Certifying and Removing Disparate Impact.pdf:pdf},
isbn = {9781450336642},
keywords = {author ordering on this,corresponding author,disparate impact,fairness,machine learning,paper is alphabetical},
pages = {259----268},
title = {{Certifying and Removing Disparate Impact}},
year = {2015}
}
@inproceedings{Otterbacher2017,
address = {New York, NY, USA},
annote = {the authors investigate gender bias in image search

first they train an image classifier that can tell whether an image depicts a man or a woman (performance is reasonable and similar for both genders)

they then look what is the gender distribution for the query "person" and find that there are way more men

lastly they analyse a bunch of queries based on character traits such as "competent", "warm", "ration al" and record gender distributions for all of them; then they perform a cluster analysis on the gender distributions; they find that the women-cluster},
author = {Otterbacher, Jahna and Bates, Jo and Clough, Paul},
booktitle = {Proc. 2017 CHI Conf. Hum. Factors Comput. Syst.},
doi = {10.1145/3025453.3025727},
file = {:Users/tim/Surfdrive/Research/Library/Literature//Otterbacher, Bates, Clough - 2017 - Competent Men and Warm Women Gender Stereotypes and Backlash in Image Search Results.pdf:pdf},
isbn = {9781450346559},
pages = {6620--6631},
publisher = {Association for Computing Machinery},
series = {CHI '17},
title = {{Competent Men and Warm Women: Gender Stereotypes and Backlash in Image Search Results}},
url = {https://doi.org/10.1145/3025453.3025727},
year = {2017}
}
@article{Olteanu,
author = {Olteanu, Alexandra and Garcia-gathright, Jean and Rijke, Maarten De and Ekstrand, Michael D and Roegiest, Adam and Lipani, Aldo and Beutel, Alex and Olteanu, Alexandra and Lucic, Ana and Stoica, Ana-andreea and Das, Anubrata and Biega, Asia and Voorn, Bart and Hauff, Claudia and Spina, Damiano and Lewis, David and Oard, Douglas W and Yilmaz, Emine and Hasibi, Faegheh and Kazai, Gabriella and Mcdonald, Graham and Haned, Hinda and Ounis, Iadh and Linden, Ilse Van Der and Garcia-gathright, Jean and Baan, Joris and Lau, Kamuela N and Balog, Krisztian and Rijke, Maarten De and Sayed, Mahmoud and Panteli, Maria and Sanderson, Mark and Lease, Matthew and Ekstrand, Michael D and Lahoti, Preethi},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Olteanu et al. - Unknown - FACTS-IR Fairness , Accountability , Confidentiality , Transparency , and Safety in Information Retrieval Ed.pdf:pdf},
title = {{FACTS-IR : Fairness , Accountability , Confidentiality , Transparency , and Safety in Information Retrieval Editors}}
}
@article{Knijnenburg2012,
abstract = {Research on recommender systems typically focuses on the accuracy of prediction algorithms. Because accuracy only partially constitutes the user experience of a recommender system, this paper proposes a framework that takes a user-centric approach to recommender system evaluation. The framework links objective system aspects to objective user behavior through a series of perceptual and evaluative constructs (called subjective system aspects and experience, respectively). Furthermore, it incorporates the influence of personal and situational characteristics on the user experience. This paper reviews how current literature maps to the framework and identifies several gaps in existing work. Consequently, the framework is validated with four field trials and two controlled experiments and analyzed using Structural Equation Modeling. The results of these studies show that subjective system aspects and experience variables are invaluable in explaining why and how the user experience of recommender systems comes about. In all studies we observe that perceptions of recommendation quality and/or variety are important mediators in predicting the effects of objective system aspects on the three components of user experience: process (e.g. perceived effort, difficulty), system (e.g. perceived system effectiveness) and outcome (e.g. choice satisfaction). Furthermore, we find that these subjective aspects have strong and sometimes interesting behavioral correlates (e.g. reduced browsing indicates higher system effectiveness). They also show several tradeoffs between system aspects and personal and situational characteristics (e.g. the amount of preference feedback users provide is a tradeoff between perceived system usefulness and privacy concerns). These results, as well as the validated framework itself, provide a platform for future research on the user-centric evaluation of recommender systems. {\textcopyright} Springer Science+Business Media B.V. 2012.},
author = {Knijnenburg, Bart P. and Willemsen, Martijn C. and Gantner, Zeno and Soncu, Hakan and Newell, Chris},
doi = {10.1007/s11257-011-9118-4},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Knijnenburg et al. - 2012 - Explaining the user experience of recommender systems.pdf:pdf},
issn = {09241868},
journal = {User Model. User-adapt. Interact.},
keywords = {Decision support systems-user experience,Decision-making,Human-computer interaction,Preference elicitation,Privacy,Recommender systems,User testing,User-centric evaluation},
number = {4-5},
pages = {441--504},
title = {{Explaining the user experience of recommender systems}},
volume = {22},
year = {2012}
}
@article{Eskens2017,
abstract = {More and more news is personalised, based on our personal data and interests. As a result, the focus of media regulation moves from the news producer to the news recipient. This research asks what the fundamental right to receive information means for personalised news consumers and the obligation it imposes on states. However, the right to receive information is under- theorised. Therefore, we develop a framework to understand this right, starting from case law of the European Court of Human Rights. On this basis, we identify five perspectives on the right to receive information: political debate, truth finding, social cohesion, avoidance of censorship and self- development. We evaluate how news personalisation affects the right to receive information, considering these five different perspectives. Our research reveals important policy choices that must be made regarding personalised news considering news consumers' rights.},
author = {Eskens, Sarah and Helberger, Natali and Moeller, Judith},
doi = {10.1080/17577632.2017.1387353},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Eskens, Helberger, Moeller - 2017 - Challenged by news personalisation five perspectives on the right to receive information.pdf:pdf},
issn = {17577640},
journal = {J. Media Law},
keywords = {European Convention on Human Rights,News personalisation,filter bubbles,media diversity,right to receive information},
number = {2},
pages = {259--284},
publisher = {Taylor {\&} Francis},
title = {{Challenged by news personalisation: five perspectives on the right to receive information}},
volume = {9},
year = {2017}
}
@article{Tsirakis2017,
abstract = {Companies that collect and analyze data from social media, news and other data streams are faced with several challenges that concern storage and processing of huge amounts of data. When they want to serve the processed information to their customers and moreover, when they want to cover different information needs for each customer, they need solutions that process data in near real time in order to gain insights on the data in motion. The volume and volatility of opinionated data that is published in social media, in combination with the variety of data sources has created a demanding ecosystem for stream processing. Although, there are several solutions that can handle information of static nature and small volume quite efficiently, they usually do not scale up properly because of their high complexity. Moreover, such solutions have been designed to run once or to run in a fixed dataset and they are not sufficient for processing huge volumes of streamed data. To address this problem, a platform for real-time opinion mining is proposed. Based on prior research and real application services that have been developed, a new platform called “PaloPro” is presented to cover the needs for brand monitoring.},
author = {Tsirakis, Nikos and Poulopoulos, Vasilis and Tsantilas, Panagiotis and Varlamis, Iraklis},
doi = {10.1016/j.jss.2016.06.012},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Tsirakis et al. - 2017 - Large scale opinion mining for social, news and blog data.pdf:pdf},
issn = {01641212},
journal = {J. Syst. Softw.},
keywords = {News streams,Opinion mining,Social media},
pages = {237--248},
publisher = {Elsevier Inc.},
title = {{Large scale opinion mining for social, news and blog data}},
url = {http://dx.doi.org/10.1016/j.jss.2016.06.012},
volume = {127},
year = {2017}
}
@article{Joachims2005,
abstract = {This paper examines the reliability of implicit feedback generated from clickthrough data in WWW search. Analyzing the users' decision process using eyetracking and comparing implicit feedback against manual relevance judgments, we conclude that clicks are informative but biased. While this makes the interpretation of clicks as absolute relevance judgments difficult, we show that relative preferences derived from clicks are reasonably accurate on average. {\textcopyright} 2005 ACM.},
author = {Joachims, Thorsten and Granka, Laura and Pan, Bing and Hembrooke, Helene and Gay, Geri},
doi = {10.1145/1076034.1076063},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Joachims et al. - 2005 - Accurately interpreting clickthrough data as implicit feedback.pdf:pdf},
isbn = {1595930345},
journal = {SIGIR 2005 - Proc. 28th Annu. Int. ACM SIGIR Conf. Res. Dev. Inf. Retr.},
keywords = {WWW search,clickthrough,eyetracking,implicit feedback},
number = {1},
pages = {154--161},
title = {{Accurately interpreting clickthrough data as implicit feedback}},
volume = {51},
year = {2005}
}
@book{Hutchison1973,
abstract = {This book fills this void by including a collection of representative articles, which gives an up-to-date and comprehensive snapshot of the Peer-to-Peer field. One of the main challenges that faces any book covering such a vast and relatively new territory is how to structure the material. This book resolves this conundrum by dividing the material into roughly three parts. The first part of the book covers the basics of Peer-to-Peer designs, un- structured and structured systems, and presents a variety of applications in- cluding e-mail, multicast, Grid computing, andWeb services. The book then goes beyond describing traditional systems, by discussing general aspects of the Peer-to-Peer systems, namely the self-organization nature of the Peer- to-Peer systems, and the all-important topic of evaluating these systems. In addition, the book illustrates the broad applicability of Peer-to-Peer by dis- cussing the impact of the Peer-to-Peer technologies in two computer-science areas, namely searching and information retrieval, and mobile computing. No Peer-to-Peer book would be complete without discussing the business model, accounting, and security. This book touches on these topics in the last part.},
archivePrefix = {arXiv},
arxivId = {9780201398298},
author = {Hutchison, David and Mitchell, John C},
booktitle = {Lect. Notes Comput. Sci.},
doi = {10.1016/0020-7101(78)90038-7},
eprint = {9780201398298},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hutchison, Mitchell - 1973 - Lecture Notes in Computer Science.pdf:pdf},
isbn = {9783642206290},
issn = {03029743},
keywords = {and j,edited by g,goos,hartmanis,j,science,ture notes in computer,van leeuwen},
number = {3},
pages = {242--242},
pmid = {4520227},
title = {{Lecture Notes in Computer Science}},
url = {http://www.mendeley.com/research/lecture-notes-computer-science-2/},
volume = {9},
year = {1973}
}
@article{Redding2001,
author = {Redding, Richard E.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Redding - 2001 - Sociopolitical diversity in psychology.pdf:pdf},
journal = {Am. Psychol.},
number = {3},
pages = {205--215},
title = {{Sociopolitical diversity in psychology}},
volume = {56},
year = {2001}
}
@article{Lawrence2015,
abstract = {In this paper, we look at three different meth- ods of extracting the argumentative structure from a piece of natural language text. These methods cover linguistic features, changes in the topic being discussed and a supervised machine learning approach to identify the components of argumentation schemes, pat- terns of human reasoning which have been detailed extensively in philosophy and psy- chology. For each of these approaches we achieve results comparable to those previously reported, whilst at the same time achieving a more detailed argument structure. Finally, we use the results from these individual tech- niques to apply them in combination, further improving the argument structure identification.},
author = {Lawrence, John and Reed, Chris},
doi = {10.3115/v1/w15-0516},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Lawrence, Reed - 2015 - Combining Argument Mining Techniques.pdf:pdf},
pages = {127--136},
title = {{Combining Argument Mining Techniques}},
year = {2015}
}
@inproceedings{Zehlike2017,
abstract = {We present a formal problem definition and an algorithm to solve the Fair Top-k Ranking problem. The problem consists of creating a ranking of k elements out of a pool of n {\textgreater}{\textgreater} k candidates. The objective is to maximize utility, and maximization is subject to a ranked group fairness constraint. Our definition of ranked group fairness uses the standard notion of protected group to extend the concept of group fairness. It ensures that every prefix of the rank contains a number of protected candidates that is statistically indistinguishable from a given target proportion, or exceeds it. The utility objective favors rankings in which every candidate included in the ranking is more qualified than any candidate not included, and rankings in which candidates are sorted by decreasing qualifications. We describe an efficient algorithm for this problem, which is tested on a series of existing datasets, as well as new datasets. Experimentally, this approach yields a ranking that is similar to the so-called "color-blind" ranking, while respecting the fairness criteria. To the best of our knowledge, FA*IR is the first algorithm grounded in statistical tests that can be used to mitigate biases in ranking against an under-represented group.},
annote = {the authors present a ranking algorithm that ranks documents according to utility (i.e, relevance in Web Search) but is subjects to fairness constraints; 

this algorithm aims for statistical parity; specifically, at any rank k a fairness criterion can be calculated which is a binomial null hypothesis significance test that analyzes whether the data was generated from a fair system (theta = 1/number of categories)

for example, if we have male and female images, the fairness criterion at rank 10 (6 males, 4 females) will test whether this ranking could have been generated from a distribution with mean 0.5; if the test is significant the ranking is deemed unfair, and the algorithm corrects for it -- otherwise items are ranked according to utility

(this is of course a problem at some point if the population is not equal to .5)

this is useful for creating fair rankings but if I work with web search, the big question is: where do I get the relevance scores from, the utility according to which the documents should be ranked?},
author = {Zehlike, Meike and Bonchi, Francesco and Castillo, Carlos and Hajian, Sara and Megahed, Mohamed and Baeza-Yates, Ricardo},
booktitle = {Admit One},
doi = {10.2307/j.ctt1b7x5pt.3},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Zehlike et al. - 2017 - FAIR A Fair Top-k Ranking Algorithm.pdf:pdf},
isbn = {9781450349185},
keywords = {algorithmic fairness,bias in computer systems,ranking,top-k,•Applied computing  Law,•Information systems  Top-k retrieval in databases},
pages = {1--18},
title = {{FA*IR: A Fair Top-k Ranking Algorithm}},
year = {2017}
}
@article{Nguyen2014,
abstract = {Eli Pariser coined the term 'filter bubble' to describe the potential for online personalization to effectively isolate people from a diversity of viewpoints or content. Online recom-mender systems -built on algorithms that attempt to pre-dict which items users will most enjoy consuming -are one family of technologies that potentially suffers from this ef-fect. Because recommender systems have become so preva-lent, it is important to investigate their impact on users in these terms. This paper examines the longitudinal im-pacts of a collaborative filtering-based recommender system on users. To the best of our knowledge, it is the first paper to measure the filter bubble effect in terms of content diver-sity at the individual level. We contribute a novel metric to measure content diversity based on information encoded in user-generated tags, and we present a new set of methods to examine the temporal effect of recommender systems on the user experience. We do find that recommender systems expose users to a slightly narrowing set of items over time. However, we also see evidence that users who actually con-sume the items recommended to them experience lessened narrowing effects and rate items more positively.},
annote = {Main thing: evaluated at the MovieLens data set, filter bubbles do not seem to exist

Nguyen et al. (2014) examined the longitudinal effects of recommender systems on content diversity. They present an interesting discussion about recommender systems and their contribution to filter bubbles in which they summarise the main arguments from both sides. Critics remark that recommender systems promote an extreme personalisation of content that traps users in unchanging environments and increasingly prevents humans from having shared experiences. Conversely, other contributors suggest that users can use recommender systems in ways that let them learn and explore, and because users cannot search for things they are not aware of, recommender systems may in fact promote content diversity. 

The authors measure similarity between two movies by vectorizing various features about them and then taking the Euclidean distance. Diversity of content can then be calculated by aggregating the similarities between all movies in a given set. Evaluating the MovieLens data set, the authors find that recommender systems slightly lower the diversity over time, but that people that use the recommender system are nevertheless exposed to a greater diversity than people who don't use it. Also, people who use it are happier with the movies they watch, so the recommender system seems to do its job. 
After reading this paper, my first thought was that movies may be a different story than news or polarised topics. Movies are entertainment products that I can like or dislike, but that are not connected to my identity. Therefore, I don't mind diversity; in fact, I actually want as much novelty as I want good content. My opinion on a polarised topic, however, is part of my identity. Here, I don't seek novelty because to be exposed to different viewpoints than my own is exhausting and potentially threatening to my identity and beliefs. Naturally, I am more protective of my views than what kind of movies I watch. },
author = {Nguyen, Tien T and Maxwell, Pik-mai Hui F and Loren, Harper and Joseph, Terveen},
doi = {10.1145/2566486.2568012},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Nguyen et al. - 2014 - Exploring the Filter Bubble The Effect of Using Recommender Systems on Content Diversity.pdf:pdf},
isbn = {9781450327442},
journal = {Proc. 23rd Int. Conf. World wide web,},
keywords = {content diversity,experience,filter bubble,longitudinal data,offerings,recommender system,sonalized product and information,tag-genome,they play a,user},
pages = {677--686},
title = {{Exploring the Filter Bubble : The Effect of Using Recommender Systems on Content Diversity}},
year = {2014}
}
@article{Napoli1999,
abstract = {This article presents an examination of the diversity principle in communications policy. Given the Federal Communication Commission's recent emphasis on diversity as a policy objective, diversity assessments must return to the forefront of communications policy analysis. To provide an analytical framework for such research, the diversity principle is broken into three distinct components (source, content, and exposure diversity), and multiple subcomponents. In the spirit of the FCC's empirical commitment to the diversity principle, this analysis focuses on diversity as a measurable concept, with potentially interacting dimensions and numerous means of assessment.},
author = {Napoli, Philip M.},
doi = {10.1111/j.1460-2466.1999.tb02815.x},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Napoli - 1999 - Deconstructing the diversity principle.pdf:pdf},
issn = {00219916},
journal = {J. Commun.},
number = {4},
pages = {7--34},
title = {{Deconstructing the diversity principle}},
volume = {49},
year = {1999}
}
@article{Atteveldt2014,
author = {Atteveldt, Wouter Van and Sheafer, Tamir and Shenhav, Shaul R and Fogel-dror, Yair},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Atteveldt et al. - 2014 - Clause analysis Using syntactic information to automatically extract source , subject , and predicate from.pdf:pdf},
pages = {1--15},
title = {{Clause analysis : Using syntactic information to automatically extract source , subject , and predicate from texts with an application to the 2008-2009 Gaza War ∗ W outer van A tteveldt}},
year = {2014}
}
@article{Doumit2011,
abstract = {It is widely recognized that every media outlet has its own ”spin” on news, and this bias has been described in many ways and at many levels. In political news for example, the bias can be liberal, conservative, moderate, corporate, etc. In addition, recent research has focused on the 'sentiment dimension' to further identify and categorize news bias. This is achieved through analysis of the adjective and adverb terms found in the news texts. The accuracy and generality of these models depend on the evaluation methods used to appraise the intensity and emotional weights of the adjectives and adverbs, thus rendering the results open to controversy. In this paper we propose a unifying system to extract information from political news texts and analyze it within a cognitive network. We view the different news media sources as agents with unique personalities, which we assume are latent within their texts. We use a combination Latent Dirichlet Allocation (LDA) and natural language processing (NLP) methods to identify the different agents' personality traits with respect to various topics or concepts. An agent's personality traits affect its inclination to word a certain event in a specific way. Using the common concepts stored in the cognitive network, our system can compare the different agents on a unified and normalized platform. 1},
author = {Doumit, Sarjoun and Minai, Ali A and Minai, Ali},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Doumit, Minai, Minai - 2011 - Online News Media Bias Analysis using an LDA-NLP Approach.pdf:pdf},
journal = {Int. Conf. Complex Syst.},
number = {May 2012},
pages = {251--265},
title = {{Online News Media Bias Analysis using an LDA-NLP Approach}},
url = {https://www.researchgate.net/publication/267559458},
year = {2011}
}
@article{Zapf2016,
abstract = {Background: Reliability of measurements is a prerequisite of medical research. For nominal data, Fleiss' kappa (in the following labelled as Fleiss' K) and Krippendorff's alpha provide the highest flexibility of the available reliability measures with respect to number of raters and categories. Our aim was to investigate which measures and which confidence intervals provide the best statistical properties for the assessment of inter-rater reliability in different situations. Methods: We performed a large simulation study to investigate the precision of the estimates for Fleiss' K and Krippendorff's alpha and to determine the empirical coverage probability of the corresponding confidence intervals (asymptotic for Fleiss' K and bootstrap for both measures). Furthermore, we compared measures and confidence intervals in a real world case study. Results: Point estimates of Fleiss' K and Krippendorff's alpha did not differ from each other in all scenarios. In the case of missing data (completely at random), Krippendorff's alpha provided stable estimates, while the complete case analysis approach for Fleiss' K led to biased estimates. For shifted null hypotheses, the coverage probability of the asymptotic confidence interval for Fleiss' K was low, while the bootstrap confidence intervals for both measures provided a coverage probability close to the theoretical one. Conclusions: Fleiss' K and Krippendorff's alpha with bootstrap confidence intervals are equally suitable for the analysis of reliability of complete nominal data. The asymptotic confidence interval for Fleiss' K should not be used. In the case of missing data or data or higher than nominal order, Krippendorff's alpha is recommended. Together with this article, we provide an R-script for calculating Fleiss' K and Krippendorff's alpha and their corresponding bootstrap confidence intervals.},
author = {Zapf, Antonia and Castell, Stefanie and Morawietz, Lars and Karch, Andr{\'{e}}},
doi = {10.1186/s12874-016-0200-9},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Zapf et al. - 2016 - Measuring inter-rater reliability for nominal data - Which coefficients and confidence intervals are appropriate.pdf:pdf},
issn = {14712288},
journal = {BMC Med. Res. Methodol.},
keywords = {Bootstrap,Confidence interval,Fleiss' K,Fleiss' kappa,Inter-rater heterogeneity,Krippendorff's alpha},
number = {1},
pmid = {27495131},
publisher = {BMC Medical Research Methodology},
title = {{Measuring inter-rater reliability for nominal data - Which coefficients and confidence intervals are appropriate?}},
url = {http://dx.doi.org/10.1186/s12874-016-0200-9},
volume = {16},
year = {2016}
}
@article{Baeckstrom2018,
abstract = {To date little attention has been paid to how social cognitive bias can influence how financial advisors interpret and respond to the needs of millionaire investors, and if this varies depending on the gender of the investor. This research investigates whether experienced professional financial advisors who work with millionaire investors make different attributions for the control and knowledge that investors have of their investments, and if they make different investment portfolio recommendations to equivalent male and female investors. Using methodology novel to finance, this vignette-based study that controls for gender finds evidence that professional financial advisors judge millionaire female investors to have less control over their investment portfolios relative to men. Empirical results also show that female advisors judge women to be less knowledgeable about investments than men. Despite such perceptual differences, advisors recommend equally risky portfolios to male and female investors. These results have implications for wealth management institutions and the monitoring of financial advisors for millionaire individuals.},
annote = {professional financial advisors are often biased in unfavourable ways; this paper shows that they judge female investors to have less control over their money},
author = {Baeckstr{\"{o}}m, Ylva and Silvester, Jo and Pownall, Rachel A.J.},
doi = {10.1080/1351847X.2018.1438301},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Baeckstr{\"{o}}m, Silvester, Pownall - 2018 - Millionaire investors financial advisors, attribution theory and gender differences.pdf:pdf},
issn = {14664364},
journal = {Eur. J. Financ.},
keywords = {Portfolio choice,financial advice,gender,investment decisions,risk-taking},
number = {15},
pages = {1333--1349},
title = {{Millionaire investors: financial advisors, attribution theory and gender differences}},
volume = {24},
year = {2018}
}
@article{Promberger2006,
abstract = {In two studies, we inquired whether patients accept medical recommendations that come from a computer program rather than from a physician. In study 1, we found that subjects, when deciding whether to have an operation or not in different medical scenarios, were more likely to follow a recommendation that came from a physician than one that came from a computer program. Subjects stated that they would feel less responsible when following a recommendation than when deciding against it. Following a physician's recommendation reduced the feeling of responsibility more than following that of a computer program. The difference in feeling of responsibility when following versus when not following a recommendation partly mediated subjects' inclination to follow the physician more. In our second study, we found that subjects were more decision seeking when they received a recommendation or decision from a computer program, and they were more decision seeking when they had to accept a decision than when they received a recommendation. Subjects also trusted the physician more than the computer program to make a good recommendation or decision. Copyright {\textcopyright} 2006 John Wiley {\&} Sons, Ltd.},
author = {Promberger, Marianne and Baron, Jonathan},
doi = {10.1002/bdm.542},
issn = {10990771},
journal = {J. Behav. Decis. Mak.},
keywords = {Advice gluing,Medical conditions,Recommendations},
number = {5},
pages = {455--468},
publisher = {John Wiley and Sons Ltd},
title = {{Do patients trust computers?}},
volume = {19},
year = {2006}
}
@article{Lee2018,
abstract = {Algorithms increasingly make managerial decisions that people used to make. Perceptions of algorithms, regardless of the algorithms' actual performance, can significantly influence their adoption, yet we do not fully understand how people perceive decisions made by algorithms as compared with decisions made by humans. To explore perceptions of algorithmic management, we conducted an online experiment using four managerial decisions that required either mechanical or human skills. We manipulated the decision-maker (algorithmic or human), and measured perceived fairness, trust, and emotional response. With the mechanical tasks, algorithmic and human-made decisions were perceived as equally fair and trustworthy and evoked similar emotions; however, human managers' fairness and trustworthiness were attributed to the manager's authority, whereas algorithms' fairness and trustworthiness were attributed to their perceived efficiency and objectivity. Human decisions evoked some positive emotion due to the possibility of social recognition, whereas algorithmic decisions generated a more mixed response – algorithms were seen as helpful tools but also possible tracking mechanisms. With the human tasks, algorithmic decisions were perceived as less fair and trustworthy and evoked more negative emotion than human decisions. Algorithms' perceived lack of intuition and subjective judgment capabilities contributed to the lower fairness and trustworthiness judgments. Positive emotion from human decisions was attributed to social recognition, while negative emotion from algorithmic decisions was attributed to the dehumanizing experience of being evaluated by machines. This work reveals people's lay concepts of algorithmic versus human decisions in a management context and suggests that task characteristics matter in understanding people's experiences with algorithmic technologies.},
author = {Lee, Min Kyung},
doi = {10.1177/2053951718756684},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Lee - 2018 - Understanding perception of algorithmic decisions Fairness, trust, and emotion in response to algorithmic management.pdf:pdf},
issn = {20539517},
journal = {Big Data Soc.},
keywords = {Algorithmic management,emotion,fairness,folk theory,perception,trust},
number = {1},
pages = {1--16},
title = {{Understanding perception of algorithmic decisions: Fairness, trust, and emotion in response to algorithmic management}},
volume = {5},
year = {2018}
}
@inproceedings{Nickel2012,
abstract = {Mobile Health (mHealth) is currently a topic of great interest world-wide. The major goal of most mHealth projects is to induce long-lasting behavior change among healthcare providers or patients or both. Clearly integration of Persuasive features has great potential for enhancing the effectiveness of mHealth solutions. In this paper we report the results of a systematic review of peer-reviewed papers describing mHealth interventions with a view to identifying the persuasive features employed, either explicitly or implicitly. Results have been summarized using descriptive statistics including cross-tabulations with types of mHealth interventions. Our results provide insights into the persuasive features that have been deemed to be useful across mHealth implementations in general and also across specific types of mHealth interventions.},
author = {Nickel, Philip and Spahn, Andreas},
booktitle = {Persuas. Technol. Des. Heal. Safety; 7th Int. Conf. Persuas. Technol. 2012},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Nickel, Spahn - 2012 - Trust, Discourse Ethics, and Persuasive Technology.pdf:pdf},
isbn = {1650-3686 (print)},
keywords = {discourse ethics,ethics,persuasive technology,speech act,trust},
pages = {37----40},
publisher = {Link{\"{o}}ping University Electronic Press},
title = {{Trust, Discourse Ethics, and Persuasive Technology}},
year = {2012}
}
@article{Benjamin2018,
abstract = {We propose to change the default P-value threshold for statistical significance from 0.05 to 0.005 for claims of new discoveries.},
author = {Benjamin, Daniel J. and Berger, James O. and Johannesson, Magnus and Nosek, Brian A. and Wagenmakers, E. J. and Berk, Richard and Bollen, Kenneth A. and Brembs, Bj{\"{o}}rn and Brown, Lawrence and Camerer, Colin and Cesarini, David and Chambers, Christopher D. and Clyde, Merlise and Cook, Thomas D. and {De Boeck}, Paul and Dienes, Zoltan and Dreber, Anna and Easwaran, Kenny and Efferson, Charles and Fehr, Ernst and Fidler, Fiona and Field, Andy P. and Forster, Malcolm and George, Edward I. and Gonzalez, Richard and Goodman, Steven and Green, Edwin and Green, Donald P. and Greenwald, Anthony G. and Hadfield, Jarrod D. and Hedges, Larry V. and Held, Leonhard and {Hua Ho}, Teck and Hoijtink, Herbert and Hruschka, Daniel J. and Imai, Kosuke and Imbens, Guido and Ioannidis, John P.A. and Jeon, Minjeong and Jones, James Holland and Kirchler, Michael and Laibson, David and List, John and Little, Roderick and Lupia, Arthur and Machery, Edouard and Maxwell, Scott E. and McCarthy, Michael and Moore, Don A. and Morgan, Stephen L. and Munaf{\'{o}}, Marcus and Nakagawa, Shinichi and Nyhan, Brendan and Parker, Timothy H. and Pericchi, Luis and Perugini, Marco and Rouder, Jeff and Rousseau, Judith and Savalei, Victoria and Sch{\"{o}}nbrodt, Felix D. and Sellke, Thomas and Sinclair, Betsy and Tingley, Dustin and {Van Zandt}, Trisha and Vazire, Simine and Watts, Duncan J. and Winship, Christopher and Wolpert, Robert L. and Xie, Yu and Young, Cristobal and Zinman, Jonathan and Johnson, Valen E.},
doi = {10.1038/s41562-017-0189-z},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Benjamin et al. - 2018 - Redefine statistical significance.pdf:pdf},
issn = {23973374},
journal = {Nat. Hum. Behav.},
number = {1},
pages = {6--10},
publisher = {Springer US},
title = {{Redefine statistical significance}},
url = {http://dx.doi.org/10.1038/s41562-017-0189-z},
volume = {2},
year = {2018}
}
@article{Malthouse2019,
author = {Malthouse, Edward C and Zhou, Yayu and Calder, Bobby J},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Malthouse, Zhou, Calder - 2019 - Increasing Engagement with Real News.pdf:pdf},
pages = {1--10},
title = {{Increasing Engagement with Real News}},
year = {2019}
}
@article{OBrien2018,
abstract = {User engagement (UE) and its measurement have been of increasing interest in human-computer interaction (HCI). The User Engagement Scale (UES) is one tool developed to measure UE, and has been used in a variety of digital domains. The original UES consisted of 31-items and purported to measure six dimensions of engagement: aesthetic appeal, focused attention, novelty, perceived usability, felt involvement, and endurability. A recent synthesis of the literature questioned the original six-factors. Further, the ways in which the UES has been implemented in studies suggests there may be a need for a briefer version of the questionnaire and more effective documentation to guide its use and analysis. This research investigated and verified a four-factor structure of the UES and proposed a Short Form (SF). We employed contemporary statistical tools that were unavailable during the UES' development to re-analyze the original data, consisting of 427 and 779 valid responses across two studies, and examined new data (N=344) gathered as part of a three-year digital library project. In this paper we detail our analyses, present a revised long and short form (SF) version of the UES, and offer guidance for researchers interested in adopting the UES and UES-SF in their own studies.},
author = {O'Brien, Heather L. and Cairns, Paul and Hall, Mark},
doi = {10.1016/j.ijhcs.2018.01.004},
file = {:Users/tim/Surfdrive/Research/Library/Literature/O'Brien, Cairns, Hall - 2018 - A practical approach to measuring user engagement with the refined user engagement scale (UES) and new UE.pdf:pdf},
issn = {10959300},
journal = {Int. J. Hum. Comput. Stud.},
keywords = {Measurement,Questionnaires,Reliability,User engagement,Validity},
number = {July 2017},
pages = {28--39},
publisher = {Elsevier Ltd},
title = {{A practical approach to measuring user engagement with the refined user engagement scale (UES) and new UES short form}},
url = {https://doi.org/10.1016/j.ijhcs.2018.01.004},
volume = {112},
year = {2018}
}
@article{Jo2019,
abstract = {The purpose of this paper is to understand the factors involved when a human judges the credibility of information and to develop a classification model for weblogs, a primary source of information for many people. Considering both computational and human-centered approaches, we conducted a user study designed to consider two cognitive procedures--(1) visceral, behavioral and (2) reflective assessments--in the evaluation of information credibility. The results of the 80-participant study highlight that human cognitive processing varies according to an individual's purpose and that humans consider the structures and styles of content in their reflective assessments. We experimentally proved these findings through the development and analysis of classification models using 16,304 real blog posts written by 2,944 bloggers. Our models yield greater accuracy and efficiency than the models with well-known best features identified in prior research},
annote = {they want to understand how humans judge whether or not a blog is credible and use these features to improve computational models that predict credibility

the authors summarized previous literature of computational models and human assessments; then they used human assessment of blogs to figure out the most important features to improve the computational models with; afterwards checked whether the models improved

methodology is shaky:
- their operationalization of coherence is weird (e.g., article length = coherency?)
- multilevel structure in the human assessment (80 participants, each rates 6 blogs)
- they don't report any statistics of the human assessment, merely a ranking of items that were relevant according to the authors
- we don't get any numbers on feature importance
- model comparison is performed by just looking at the bare performance numbers; not by actual statistical comparison

furthermore, this was quite exploratory; I think they should have confirmed the importance of coherence in a regular hypothesis test (seeing whether a change in coherence causes a change in perceived credibility)},
author = {Jo, Yonggeol and Kim, Minwoo and Han, Kyungsik},
doi = {10.1145/3290605.3300904},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Jo, Kim, Han - 2019 - How do humans access the credibility of weblogs Qualifying and verifying human factors with machine learning.pdf:pdf},
isbn = {9781450359702},
journal = {Conf. Hum. Factors Comput. Syst. - Proc.},
keywords = {Cognitive machine learning,Information credibility,Social networking services,Weblogs},
pages = {1--12},
title = {{How do humans access the credibility of weblogs: Qualifying and verifying human factors with machine learning}},
year = {2019}
}
@article{Lin2009,
abstract = {Sentiment analysis or opinion mining aims to use automated tools to detect subjective information such as opinions, attitudes, and feelings expressed in text. This paper proposes a novel probabilistic modeling framework based on Latent Dirichlet Allocation (LDA), called joint sentiment/topic model (JST), which detects sentiment and topic simultaneously from text. Unlike other machine learning approaches to sentiment classification which often require labeled corpora for classifier training, the proposed JST model is fully unsupervised. The model has been evaluated on the movie review dataset to classify the review sentiment polarity and minimum prior information have also been explored to further improve the sentiment classification accuracy. Preliminary experiments have shown promising results achieved by JST.},
annote = {$\backslash$citeA{\{}Lin2009{\}} introduced the $\backslash$emph{\{}joint sentiment/topic{\}} (JST) model as an extension to LDA. Next to topic discovery, JST is also able to detect sentiment in text. This is achieved by adding another step into the generative process of LDA. In JST, first a topic, then a sentiment is chosen. The sentiment can be negative, neutral, or positive, and words are subsequently chosen from the joint topic-sentiment. The results show that JST was able to compete with the state of the art at the time in terms of sentiment analysis. In combination with the discovered topics, this allowed for a more in-depth interpretation of documents. A drawback of JST is that it is entirely based on bag-of-words, which means that it will likely consider ``not a bad movie'' as a negative sentiment, and ``not a good movie'' as a positive sentiment.},
author = {Lin, Chenghua and He, Yulan},
doi = {10.1145/1645953.1646003},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Lin, He - 2009 - Joint sentimenttopic model for sentiment analysis.pdf:pdf},
isbn = {9781605585123},
journal = {Int. Conf. Inf. Knowl. Manag. Proc.},
keywords = {Joint sentiment/topic model,Latent dirichlet allocation,Opinion mining,Sentiment analysis},
pages = {375--384},
title = {{Joint sentiment/topic model for sentiment analysis}},
year = {2009}
}
@article{Palic2019,
abstract = {In this paper, we demonstrate the system built to solve the SemEval-2019 task 4: Hyperpar-tisan News Detection (Kiesel et al., 2019), the task of automatically determining whether an article is heavily biased towards one side of the political spectrum. Our system receives an article in its raw, textual form, analyzes it, and predicts with moderate accuracy whether the article is hyperpartisan. The learning model used was primarily trained on a manually pre-labeled dataset containing news articles. The system relies on the previously constructed SVM model, available in the Python Scikit-Learn library. We ranked 6th in the competition of 42 teams with an accuracy of 79.1{\%} (the winning team had 82.2{\%}).},
author = {Pali´c, Niko and Vladika, Juraj and Dominikˇ, Dominik{\v{c}}ubeli´c and Dominik{\v{c}}ubeli´c, Dominik{\v{c}}ubeli´ and Lovren{\v{c}}i´c, Ivan Lovren{\v{c}}i´ and Buljan, Maja and Snajder, Jaň},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Pali´c et al. - 2019 - TakeLab at SemEval-2019 Task 4 Hyperpartisan News Detection.pdf:pdf},
journal = {Proc. 13th Int. Work. Semant. Eval.},
pages = {995--998},
title = {{TakeLab at SemEval-2019 Task 4: Hyperpartisan News Detection}},
url = {https://spacy.io},
year = {2019}
}
@article{Etz2016,
abstract = {In this guide, we present a reading list to serve as a concise introduction to Bayesian data analysis. The introduction is geared toward reviewers, editors, and interested researchers who are new to Bayesian statistics. We provide commentary for eight recommended sources, which together cover the theoretical and practical cornerstones of Bayesian statistics in psychology and related sciences. The resources are presented in an incremental order, starting with theoretical foundations and moving on to applied issues. In addition, we outline an additional 28 articles and books that can be consulted to gain background knowledge about various theoretical specifics and Bayesian approaches to frequently used models. Our goal is to offer researchers a starting point for understanding the core tenets of Bayesian analysis, while requiring a low level of time commitment. After consulting our guide and the outlined articles, the reader should understand how and why Bayesian methods work, and feel able to evaluate their use in the behavioral and social sciences.},
author = {Etz, Alexander and Etz, Alexander and Gronau, Quentin F and Dablander, Fabian and Baribault, Beth},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Etz et al. - 2016 - How to become a Bayesian in eight easy steps An annotated reading list How to become a Bayesian in eight easy steps.pdf:pdf},
journal = {Psychon. Bull. Rev.},
number = {May},
pages = {1--28},
title = {{How to become a Bayesian in eight easy steps : An annotated reading list How to become a Bayesian in eight easy steps : An annotated reading list}},
year = {2016}
}
@article{Yang2020,
abstract = {We investigated the effects of example-based explanations for a machine learning classifier on end users' appropriate trust. We explored the effects of spatial layout and visual representation in an in-person user study with 33 participants. We measured participants' appropriate trust in the classifier, quantified the effects of different spatial layouts and visual representations, and observed changes in users' trust over time. The results show that each explanation improved users' trust in the classifier, and the combination of explanation, human, and classification algorithm yielded much better decisions than the human and classification algorithm separately. Yet these visual explanations lead to different levels of trust and may cause inappropriate trust if an explanation is difficult to understand. Visual representation and performance feedback strongly affect users' trust, and spatial layout shows a moderate effect. Our results do not support that individual differences (e.g., propensity to trust) affect users' trust in the classifier. This work advances the state-of-the-art in trust-able machine learning and informs the design and appropriate use of automated systems.},
author = {Yang, Fumeng and Huang, Zhuanyi and Scholtz, Jean and Arendt, Dustin L.},
doi = {10.1145/3377325.3377480},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Yang et al. - 2020 - How do visual explanations foster end users' appropriate trust in machine learning.pdf:pdf},
isbn = {9781450371186},
journal = {Int. Conf. Intell. User Interfaces, Proc. IUI},
keywords = {classification,explainable artificial intelligence,human-machine collaboration,information visualization,supervised-learning,trust,trust calibration},
pages = {189--201},
title = {{How do visual explanations foster end users' appropriate trust in machine learning?}},
year = {2020}
}
@article{kullback1951information,
author = {Kullback, Solomon and Leibler, Richard A},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Kullback, Leibler - 1951 - On information and sufficiency.pdf:pdf},
journal = {Ann. Math. Stat.},
number = {1},
pages = {79--86},
title = {{On information and sufficiency}},
volume = {22},
year = {1951}
}
@article{Biega2018,
abstract = {Rankings of people and items are at the heart of selection-making, match-making, and recommender systems, ranging from employment sites to sharing economy platforms. As ranking positions influence the amount of attention the ranked subjects receive, biases in rankings can lead to unfair distribution of opportunities and resources such as jobs or income. This paper proposes new measures and mechanisms to quantify and mitigate unfairness from a bias inherent to all rankings, namely, the position bias which leads to disproportionately less attention being paid to low-ranked subjects. Our approach differs from recent fair ranking approaches in two important ways. First, existing works measure unfairness at the level of subject groups while our measures capture unfairness at the level of individual subjects, and as such subsume group unfairness. Second, as no single ranking can achieve individual attention fairness, we propose a novel mechanism that achieves amortized fairness, where attention accumulated across a series of rankings is proportional to accumulated relevance. We formulate the challenge of achieving amortized individual fairness subject to constraints on ranking quality as an online optimization problem and show that it can be solved as an integer linear program. Our experimental evaluation reveals that unfair attention distribution in rankings can be substantial, and demonstrates that our method can improve individual fairness while retaining high ranking quality.},
archivePrefix = {arXiv},
arxivId = {1805.01788},
author = {Biega, Asia J. and Gummadi, Krishna P. and Weikum, Gerhard},
doi = {10.1145/3209978.3210063},
eprint = {1805.01788},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Biega, Gummadi, Weikum - 2018 - Equity of attention Amortizing individual fairness in rankings.pdf:pdf},
isbn = {9781450356572},
journal = {41st Int. ACM SIGIR Conf. Res. Dev. Inf. Retrieval, SIGIR 2018},
keywords = {Algorithmic fairness,Amortized fairness,Attention,Exposure,Fair ranking,Individual fairness,Position bias},
pages = {405--414},
title = {{Equity of attention: Amortizing individual fairness in rankings}},
year = {2018}
}
@article{Allison2001,
author = {Allison, Paul D.},
doi = {10.1377/hlthaff.2011.0678},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Allison - 2001 - Missing Data - chapter 4.pdf:pdf},
issn = {1544-5208},
journal = {Missing Data},
number = {7},
pages = {104},
pmid = {21734215},
title = {{Missing Data - chapter 4}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/21756330},
volume = {30},
year = {2001}
}
@article{OBrien2006,
abstract = {There are important cognitive issues surrounding the searching of lists of results returned to search engine queries that could significantly impact system and interface design. In this paper, we focus on result-list search examining two key issues: the influence of relevance topology of the list on first- $\backslash$nclick behavior, and the question of whether trust-bias occurs in such search. On both issues we advance some empirical and modeling results. These results are discussed in terms of their practical implications for Web designers and $\backslash$npractitioners generally.},
author = {O'Brien, Maeve and Keane, Mark T.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/O'Brien, Keane - 2006 - Modeling result-list searching in the world wide web The role of relevance topologies and trust bias.pdf:pdf},
journal = {Proc. 28th Annu. Conf. Cogn. Sci. Soc.},
keywords = {empirical tests,information,predictive user modeling,search behavior},
pages = {1881--1886},
title = {{Modeling result-list searching in the world wide web: The role of relevance topologies and trust bias}},
year = {2006}
}
@article{Trabelsi2018,
annote = {this is about modeling stances in online debates / forums},
author = {Trabelsi, Amine and Za{\"{i}}ane, Osmar R.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Trabelsi, Za{\"{i}}ane - 2018 - Unsupervised model for topic viewpoint discovery in online debates leveraging author interactions.pdf:pdf},
isbn = {9781577357988},
journal = {12th Int. AAAI Conf. Web Soc. Media, ICWSM 2018},
keywords = {Full Papers},
number = {Icwsm},
pages = {425--433},
title = {{Unsupervised model for topic viewpoint discovery in online debates leveraging author interactions}},
year = {2018}
}
@article{Chen2014,
abstract = {With the evolution of the Web and development of web-based search engines, online searching has become a common method for obtaining information. Given this popularity, the question arises as to how much time people save by using search engines for their information needs compared to offline sources, as well as how online searching affects both search experiences and search outcomes. Using a random sample of queries from a major search engine and a sample of reference questions from the Internet Public Library (IPL), we conduct a real-effort experiment to compare online and offline search experiences and outcomes. We find that participants are significantly more likely to find an answer on the Web (100 {\%}), compared to offline searching (between 87 {\%} and 90 {\%}). Restricting our analysis to the set of questions in which participants find answers in both treatments, a Web search takes on average 7 (9) minutes, whereas the corresponding offline search takes 22 (19) minutes for a search-engine (IPL) question. Furthermore, while raters judge library sources to be significantly more trustworthy and authoritative than the corresponding Web sources, they judge Web sources as significantly more relevant. Balancing all factors, we find that the overall source quality is not significantly different between the two treatments for the set of search-engine questions. However, for IPL questions, we find that non-Web sources are judged to have significantly higher overall quality than the corresponding Web sources. In comparison, for factual questions, Web search results are significantly more likely to be correct (66 {\%} vs. 43 {\%}). Lastly, post-search questionnaires reveal that participants find online searching more enjoyable than offline searching.},
author = {Chen, Yan and Jeon, Grace Young Joo and Kim, Yong Mi},
doi = {10.1007/s10683-013-9381-9},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Chen, Jeon, Kim - 2014 - A day without a search engine an experimental study of online and offline searches.pdf:pdf},
issn = {13864157},
journal = {Exp. Econ.},
keywords = {Experiment,Productivity,Search},
number = {4},
pages = {512--536},
title = {{A day without a search engine: an experimental study of online and offline searches}},
volume = {17},
year = {2014}
}
@article{Hutson2018,
abstract = {![Figure][1]{\textless}/img{\textgreater} The same algorithm can learn to walk in wildly different ways. IMAGES: YUVAL TASSA Last year, computer scientists at the University of Montreal (U of M) in Canada were eager to show off a new speech recognition algorithm, and they wanted to compare it to a benchmark, an algorithm from a well-known scientist. The only problem: The benchmark's source code wasn't published. The researchers had to recreate it from the published description. But they couldn't get their version to match the benchmark's claimed performance, says Nan Rosemary Ke, a Ph.D. student in the U of M lab. “We tried for 2 months and we couldn't get anywhere close.” The booming field of artificial intelligence (AI) is grappling with a replication crisis, much like the ones that have afflicted psychology, medicine, and other fields over the past decade. AI researchers have found it difficult to reproduce many key results, and that is leading to a new conscientiousness about research methods and publication protocols. “I think people outside the field might assume that because we have code, reproducibility is kind of guaranteed,” says Nicolas Rougier, a computational neuroscientist at France's National Institute for Research in Computer Science and Automation in Bordeaux. “Far from it.” Last week, at a meeting of the Association for the Advancement of Artificial Intelligence (AAAI) in New Orleans, Louisiana, reproducibility was on the agenda, with some teams diagnosing the problem—and one laying out tools to mitigate it. The most basic problem is that researchers often don't share their source code. At the AAAI meeting, Odd Erik Gundersen, a computer scientist at the Norwegian University of Science and Technology in Trondheim, reported the results of a survey of 400 algorithms presented in papers at two top AI conferences in the past few years. He found that only 6{\%} of the presenters shared the algorithm's code. Only a third shared the data they tested their algorithms on, and just half shared “pseudocode”—a limited summary of an algorithm. (In many cases, code is also absent from AI papers published in journals, including Science and Nature .) Researchers say there are many reasons for the missing details: The code might be a work in progress, owned by a company, or held tightly by a researcher eager to stay ahead of the competition. It might be dependent on other code, itself unpublished. Or it might be that the code is simply lost, on a crashed disk or stolen laptop—what Rougier calls the “my dog ate my program” problem. Assuming you can get and run the original code, it still might not do what you expect. In the area of AI called machine learning, in which computers derive expertise from experience, the training data for an algorithm can influence its performance. Ke suspects that not knowing the training for the speech-recognition benchmark was what tripped up her group. “There's randomness from one run to another,” she says. You can get “really, really lucky and have one run with a really good number,” she adds. “That's usually what people report.” At the AAAI meeting, Peter Henderson, a computer scientist at McGill University in Montreal, showed that the performance of AIs designed to learn by trial and error is highly sensitive not only to the exact code used, but also to the random numbers generated to kick off training, and to “hyperparameters”—settings that are not core to the algorithm but that affect how quickly it learns. He ran several of these “reinforcement learning” algorithms under different conditions and found wildly different results. For example, a virtual “half-cheetah”—a stick figure used in motion algorithms—could learn to sprint in one test but would flail around on the floor in another. Henderson says researchers should document more of these key details. “We're trying to push the field to have better experimental procedures, better evaluation methods,” he says. ![Figure][1]{\textless}/img{\textgreater} CREDITS: (GRAPHIC) E. HAND/ SCIENCE ; (DATA) GUNDERSEN AND KJENSMO, ASSOCIATION FOR THE ADVANCEMENT OF ARTIFICIAL INTELLIGENCE 2018 Henderson's experiment was conducted in a test bed for reinforcement learning algorithms called Gym, created by OpenAI, a nonprofit based in San Francisco, California. John Schulman, a computer scientist at OpenAI who helped create Gym, says that it helps standardize experiments. “Before Gym, a lot of people were working on reinforcement learning, but everyone kind of cooked up their own environments for their experiments, and that made it hard to compare results across papers,” he says. IBM Research presented another tool at the AAAI meeting to aid replication: a system for recreating unpublished source code automatically, saving researchers days or weeks of effort. It's a neural network—a machine learning algorithm made of layers of small computational units, analogous to neurons—that is designed to recreate other neural networks. It scans an AI research paper looking for a chart or diagram describing a neural net, parses those data into layers and connections, and generates the network in new code. The tool has now reproduced hundreds of published neural networks, and IBM is planning to make them available in an open, online repository. Joaquin Vanschoren, a computer scientist at Eindhoven University of Technology in the Netherlands, has created another repository for would-be replicators: a website called OpenML. It hosts not only algorithms, but also data sets and more than 8 million experimental runs with all their attendant details. “The exact way that you run your experiments is full of undocumented assumptions and decisions,” Vanschoren says. “A lot of this detail never makes it into papers.” Psychology has dealt with its reproducibility crisis in part by creating a culture that favors replication, and AI is starting to do the same. In 2015, Rougier helped start ReScience , a computer science journal dedicated to replications. The large Neural Information Processing Systems conference has started linking from its website to papers' source code when available. And Ke is helping organize a “reproducibility challenge,” in which researchers are invited to try to replicate papers submitted for an upcoming conference. Ke says nearly 100 replications are in progress, mostly by students, who may receive academic credit for their efforts. Yet AI researchers say the incentives are still not aligned with reproducibility. They don't have time to test algorithms under every condition, or the space in articles to document every hyperparameter they tried. They feel pressure to publish quickly, given that many papers are posted online to arXiv every day without peer review. And many are reluctant to report failed replications. At ReScience , for example, all the published replications have so far been positive. Rougier says he's been told of failed attempts, but young researchers often don't want to be seen as criticizing senior researchers. That's one reason why Ke declined to name the researcher behind the speech recognition algorithm she wanted to use as a benchmark. Gundersen says the culture needs to change. “It's not about shaming,” he says. “It's just about being honest.” [1]: pending:yes},
author = {Hutson, Matthew},
doi = {10.1126/science.359.6377.725},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hutson - 2018 - Artificial intelligence faces reproducibility crisis.pdf:pdf},
issn = {0036-8075},
journal = {Science (80-. ).},
number = {6377},
pages = {725--726},
title = {{Artificial intelligence faces reproducibility crisis}},
volume = {359},
year = {2018}
}
@article{Baeza-Yates2018,
abstract = {OUR INHERENT HUMAN tendency of favoring one thing or opinion over another is reflected in every aspect of our lives, creating both latent and overt biases toward everything we see, hear, and do. Any remedy for bias must start with awareness that bias exists; for example, most mature societies raise awareness of social bias through affirmative-action programs, and, while awareness alone does not completely alleviate the problem, it helps guide us toward a solution. Bias on the Web reflects both societal and internal biases within ourselves, emerging in subtler ways. This article aims to increase awareness of the potential effects imposed on us all through bias present in Web use and content. We must thus consider and account for it in the design of Web systems that truly address people's needs.},
author = {Baeza-Yates, Ricardo},
doi = {10.1145/3209581},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Baeza-Yates - 2018 - Bias on the web.pdf:pdf},
issn = {15577317},
journal = {Commun. ACM},
number = {6},
pages = {54--61},
title = {{Bias on the web}},
volume = {61},
year = {2018}
}
@incollection{Petty2012,
abstract = {Attitude change involves modifying an individual's overall evaluation (good-bad) of a person, object, or issue. Change can be induced in relatively thoughtful or nonthoughtful ways, and any persuasion variable (e.g., source credibility, recipient happiness) can lead to attitude change by any of a small number of mechanisms described. High thought attitude change involves modifying the number, valence, or confidence people have in their thoughts about the attitude object. Low thought change involves associating the attitude object with affect or invoking a simple decision rule or heuristic.},
author = {Petty, Richard E and Brinol, Pablo},
booktitle = {Adv. Soc. Psychol. state Sci.},
chapter = {7},
doi = {10.1016/B978-0-12-375000-6.00040-9},
editor = {Baumeister, R. F. and Finkel, E. J.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Petty, Brinol - 2010 - Attitude Change.pdf:pdf},
isbn = {9780123750006},
keywords = {Attitude,Attitude change,Attitude strength,Behavior,Central route,Dissonance,Dual process theories,Elaboration,Evaluation,Peripheral route,Persuasion,Resistance},
pages = {217--259},
publisher = {Oxford University Press},
title = {{Attitude Change}},
year = {2010}
}
@article{Barocas2016,
author = {{Barocas, Solon and Selbst}, Andrew D},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Barocas, Solon and Selbst - 2016 - Big data's disparate impact.pdf:pdf},
journal = {Calif. Law Rev.},
number = {671},
pages = {671--732},
title = {{Big data's disparate impact}},
volume = {104},
year = {2016}
}
@article{Deerwester1990,
abstract = {A new method for automatic indexing and retrieval is$\backslash$ndescribed. The approach is to take advantage of$\backslash$nimplicit higher-order structure in the association of$\backslash$nterms with documents (``semantic structure'') in order$\backslash$nto improve the detection of relevant documents on the$\backslash$nbasis of terms found in queries. The particular$\backslash$ntechnique used is singular-value decomposition, in$\backslash$nwhich a large term by document matrix is decomposed$\backslash$ninto a set of ca. 100 orthogonal factors from which the$\backslash$noriginal matrix can be approximated by linear$\backslash$ncombination. Documents are represented by ca. 100 item$\backslash$nvectors of factor weights. Queries are represented as$\backslash$npseudo-document vectors formed from weighted$\backslash$ncombinations of terms, and documents with$\backslash$nsupra-threshold cosine values are returned. Initial$\backslash$ntests find this completely automatic method for$\backslash$nretrieval to be promising.},
author = {Deerwester, Scott and Dumais, Susan T. and Furnas, George W. and Landauer, Thomas K. and Harshman, Richard},
doi = {10.1002/(SICI)1097-4571(199009)41:6<391::AID-ASI1>3.0.CO;2-9},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Deerwester et al. - 1990 - Indexing by latent semantic analysis.pdf:pdf},
issn = {10974571},
journal = {J. Am. Soc. Inf. Sci.},
number = {6},
pages = {391--407},
title = {{Indexing by latent semantic analysis}},
volume = {41},
year = {1990}
}
@article{Ahmad2018,
abstract = {A successful persuasive technology is able to persuade people to change from one state to a more well known state. Therefore, to allow for a change, persuasive technology must be able to affect users' emotion and make the user trust the technology so that they will adopt the persuasive technology into their daily life routine, as well as continue to use the technology for long period. This paper is aimed to study the relation between users' emotion with trust and persuasion and how they may contribute to the success of changing a person attitude or behavior towards a certain context or issue. Twenty five participants have completed the study in 6 weeks by using two types of persuasive technology that were assessed at three different interaction stages: pre, during and post. Result shows that emotions have a significant effect on trust, whereas the effect of emotions on persuasion using the persuasive technology was mediated by trust.},
author = {Ahmad, Wan Nooraishya Wan and Ali, Nazlena Mohamad},
doi = {10.9781/ijimai.2018.02.010},
issn = {1989-1660},
journal = {Int. J. Interact. Multimed. Artif. Intell.},
number = {1},
pages = {57--61},
title = {{A Study on Persuasive Technologies: The Relationship between User Emotions, Trust and Persuasion}},
volume = {5},
year = {2018}
}
@inproceedings{Bardhan2016,
abstract = {It is generally argued that the current state of degradation to environment is predominantly due to lack of appropriate human behaviour. Members of the civil society are slowly awakening to the ill-effects of inefficient waste disposal and are trying to contribute to the well-being and maintenance of the world we live in. While rules and regulations have been formulated by the governing bodies for segregating waste, efforts in this direction have not translated into a veritable pro-environmental behaviour among citizens. Pro-environmental behaviour (PEB) refers to behaviour that benefits the environment or harms the environment as little as possible. Many social processes and norms exert influence over our behavior. According to a popular thesis on human behaviour, known as the theory of planned behaviour (TPB), an individual's intention towards behavior, subjective norms and perceived control over his/her behaviour together leads to intentions and behavior [1]. School children exhibit a responsibility to induce changes in social norms for environmental friendly behaviours and are also natural early adopters of technology in this endeavor. We explore the use of persuasive technologies where behaviour-oriented design techniques are employed to change behaviors of users through persuasion and social influence. In this paper, we propose an approach for designing persuasive technologies for stoking pro-environmental behaviour and initiating waste segregation at source.},
author = {Bardhan, Ronita and Bahuman, Chaitra and Pathan, Imrankhan and Ramamritham, Krithi},
booktitle = {IEEE Reg. 10 Humanit. Technol. Conf. R10-HTC 2015 - co-located with 8th Int. Conf. Humanoid, Nanotechnology, Inf. Technol. Commun. Control. Environ. Manag. HNICEM 2015},
doi = {10.1109/R10-HTC.2015.7391844},
title = {{Designing a game based persuasive technology to promote pro-environmental behaviour (PEB)}},
year = {2016}
}
@article{Elwyn2010,
abstract = {Objectives In this article, we examine definitions of suggested approaches to measure the concept of good decisions, highlight the ways in which they converge, and explain why we have concerns about their emphasis on post-hoc estimations and post-decisional outcomes, their prescriptive concept of knowledge, and their lack of distinction between the process of deliberation, and the act of decision determination. Background There has been a steady trend to involve patients in decision making tasks in clinical practice, part of a shift away from paternalism towards the concept of informed choice. An increased understanding of the uncertainties that exist in medicine, arising from a weak evidence base and, in addition, the stochastic nature of outcomes at the individual level, have contributed to shifting the responsibility for decision making from physicians to patients. This led to increasing use of decision support and communication methods, with the ultimate aim of improving decision making by patients. Interest has therefore developed in attempting to define good decision making and in the development of measurement approaches. Method We pose and reflect whether decisions can be judged good or not, and, if so, how this goodness might be evaluated. Results We hypothesize that decisions cannot be measured by reference to their outcomes and offer an alternative means of assessment, which emphasizes the deliberation process rather than the decision's end results. We propose decision making comprises a pre-decisional process and an act of decision determination and consider how this model of decision making serves to develop a new approach to evaluating what constitutes a good decision making process. We proceed to offer an alternative, which parses decisions into the pre-decisional deliberation process, the act of determination and post-decisional outcomes. Discussion Evaluating the deliberation process, we propose, should comprise of a subjective sufficiency of knowledge, as well as emotional processing and affective forecasting of the alternatives. This should form the basis for a good act of determination. {\textcopyright} 2009 Blackwell Publishing Ltd.},
annote = {nice and well-cited paper from the medical field on measuring patient decision making

they argue that the decision-making process should be measured apart from the decision itself (deliberation, then determination)},
author = {Elwyn, Glyn and Miron-Shatz, Talya},
doi = {10.1111/j.1369-7625.2009.00572.x},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Elwyn, Miron-Shatz - 2010 - Deliberation before determination The definition and evaluation of good decision making.pdf:pdf},
issn = {13696513},
journal = {Heal. Expect.},
keywords = {Decision quality,Evaluation,Measurement,Patient involvement,Shared decision making},
number = {2},
pages = {139--147},
title = {{Deliberation before determination: The definition and evaluation of good decision making}},
volume = {13},
year = {2010}
}
@article{Cramer2016,
abstract = {Many psychologists do not realize that exploratory use of the popular multiway analysis of variance harbors a multiple-comparison problem. In the case of two factors, three separate null hypotheses are subject to test (i.e., two main effects and one interaction). Consequently, the probability of at least one Type I error (if all null hypotheses are true) is 14 {\%} rather than 5 {\%}, if the three tests are independent. We explain the multiple-comparison problem and demonstrate that researchers almost never correct for it. To mitigate the problem, we describe four remedies: the omnibus F test, control of the familywise error rate, control of the false discovery rate, and preregistration of the hypotheses.},
archivePrefix = {arXiv},
arxivId = {1412.3416},
author = {Cramer, Ang{\'{e}}lique O.J. and van Ravenzwaaij, Don and Matzke, Dora and Steingroever, Helen and Wetzels, Ruud and Grasman, Raoul P.P.P. and Waldorp, Lourens J. and Wagenmakers, Eric Jan},
doi = {10.3758/s13423-015-0913-5},
eprint = {1412.3416},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Cramer et al. - 2016 - Hidden multiplicity in exploratory multiway ANOVA Prevalence and remedies.pdf:pdf},
issn = {15315320},
journal = {Psychon. Bull. Rev.},
keywords = {Benjamini–Hochberg procedure,Factorial ANOVA,False discovery rate,Familywise error rate,Multiple comparison problem,Multiway ANOVA,Preregistration,Sequential Bonferroni,Type I error},
number = {2},
pages = {640--647},
title = {{Hidden multiplicity in exploratory multiway ANOVA: Prevalence and remedies}},
volume = {23},
year = {2016}
}
@article{Aczel2020,
annote = {this might be a handy checklist for creating transparent research; the authors also introduce a form that can be completed online},
author = {Aczel, Balazs and Szaszi, Barnabas and Sarafoglou, Alexandra and Kekecs, Zoltan and Kucharsk{\'{y}}, {\v{S}}imon and Benjamin, Daniel and Chambers, Christopher D. and Fisher, Agneta and Gelman, Andrew and Gernsbacher, Morton A. and Ioannidis, John P. and Johnson, Eric and Jonas, Kai and Kousta, Stavroula and Lilienfeld, Scott O. and Lindsay, D. Stephen and Morey, Candice C. and Munaf{\`{o}}, Marcus and Newell, Benjamin R. and Pashler, Harold and Shanks, David R. and Simons, Daniel J. and Wicherts, Jelte M. and Albarracin, Dolores and Anderson, Nicole D. and Antonakis, John and Arkes, Hal R. and Back, Mitja D. and Banks, George C. and Beevers, Christopher and Bennett, Andrew A. and Bleidorn, Wiebke and Boyer, Ty W. and Cacciari, Cristina and Carter, Alice S. and Cesario, Joseph and Clifton, Charles and Conroy, Ron{\'{a}}n M. and Cortese, Mike and Cosci, Fiammetta and Cowan, Nelson and Crawford, Jarret and Crone, Eveline A. and Curtin, John and Engle, Randall and Farrell, Simon and Fearon, Pasco and Fichman, Mark and Frankenhuis, Willem and Freund, Alexandra M. and Gaskell, M. Gareth and Giner-Sorolla, Roger and Green, Don P. and Greene, Robert L. and Harlow, Lisa L. and de la Guardia, Fernando Hoces and Isaacowitz, Derek and Kolodner, Janet and Lieberman, Debra and Logan, Gordon D. and Mendes, Wendy B. and Moersdorf, Lea and Nyhan, Brendan and Pollack, Jeffrey and Sullivan, Christopher and Vazire, Simine and Wagenmakers, Eric Jan},
doi = {10.1038/s41562-019-0772-6},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Aczel et al. - 2020 - A consensus-based transparency checklist.pdf:pdf},
issn = {23973374},
journal = {Nat. Hum. Behav.},
number = {1},
pages = {4--6},
pmid = {31792401},
publisher = {Springer US},
title = {{A consensus-based transparency checklist}},
url = {http://dx.doi.org/10.1038/s41562-019-0772-6},
volume = {4},
year = {2020}
}
@article{Sanderson2009,
abstract = {This paper describes a study on diversity in image search results. One of the first test collections explicitly built to study diversity – the ImageCLEFPhoto 2008 collection – was used in an evaluation exercise in the summer of 2008. Analyzing 200 of the runs submitted by 24 research groups enabled the relationship between precision and result diversity to be studied. In addition, the level of diversity present in search results produced by retrieval systems built without explicit support for diversity was computed. The remaining potential to improve on diversity was calculated and finally, a significant preference by users for diverse search results was shown.},
author = {Sanderson, Mark and Tang, Jiayu and Arni, Thomas and Clough, Paul},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Sanderson et al. - 2009 - What Else Is There Search Diversity Examined.pdf:pdf},
journal = {Adv. Inf. Retr.},
pages = {562--569},
title = {{What Else Is There? Search Diversity Examined}},
url = {http://www.mendeley.com/research/lecture-notes-computer-science-2/},
year = {2009}
}
@article{Gelman2006,
abstract = {It is common to summarize statistical comparisons by declarations of statistical significance or nonsignificant. Here we discuss one problem with such declarations, namely that changes in statistical significance are often not themselves statistically significant. By this, we are not merely making the commonplace observation that any particular threshold is arbitrary - for example, only a small change is required to move an estimate from a 5.1{\%} significance level to 4.9{\%}, thus moving it into statistical significance. Rather, we are pointing out that even large changes in significance levels can correspond to small, nonsignificant changes in the underlying quantities. The error we describe is conceptually different from other oftcited problems - that statistical significance is not the same as practical importance, that dichotomization into significant and nonsignificant results encourages the dismissal of observed differences in favor of the usually less interesting null hypothesis of no difference, and that any particular threshold for declaring significance is arbitrary. We are troubled by all of these concerns and do not intend to minimize their importance. Rather, our goal is to bring attention to this additional error of interpretation. We illustrate with a theoretical example and two applied examples. The ubiquity of this statistical error leads us to suggest that students and practitioners be made more aware that the difference between "significant" and "not significant" is not itself statistically significant. {\textcopyright} American Statisticial Association.},
author = {Gelman, Andrew and Stern, Hal},
doi = {10.1198/000313006X152649},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Gelman, Stern - 2006 - The difference between significant and not significant is not itself statistically significant.pdf:pdf},
issn = {00031305},
journal = {Am. Stat.},
keywords = {Hypothesis testing,Meta-analysis,Pairwise comparison,Replication},
number = {4},
pages = {328--331},
title = {{The difference between "significant" and "not significant" is not itself statistically significant}},
volume = {60},
year = {2006}
}
@article{Schmitt2018,
abstract = {As the Internet provides massive amounts of heterogeneous information, people may perceive this medium as challenging. The difficulty to evaluate and select relevant information increases as more and more diverse sources and content are available. Information overload (IO) may be the consequence. The research presented here gives a first comprehensive overview of possible indicators for IO in the context of online news exposure. Based on an online survey (N=419), we found that younger people with less information-seeking self-efficacy were more susceptible to experience IO. Additionally, we identified motivations for media consumption and information retrieval strategies in the Internet that imply IO. With our results, we contribute to a further understanding of IO and provide an important basis for future research needed to face the challenges resulting from the rising media diversity.},
author = {Schmitt, Josephine B. and Debbelt, Christina A. and Schneider, Frank M.},
doi = {10.1080/1369118X.2017.1305427},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Schmitt, Debbelt, Schneider - 2018 - Too much information Predictors of information overload in the context of online news exposure.pdf:pdf},
issn = {14684462},
journal = {Inf. Commun. Soc.},
keywords = {Information overload,information retrieval strategies,motivations for media consumption,online news exposure,self-efficacy},
number = {8},
pages = {1151--1167},
title = {{Too much information? Predictors of information overload in the context of online news exposure}},
volume = {21},
year = {2018}
}
@article{Roder2015,
abstract = {Quantifying the coherence of a set of statements is a long standing problem with many potential applications that has attracted researchers from different sciences. The special case of measuring coherence of topics has been recently studied to remedy the problem that topic models give no guaranty on the interpretablity of their output. Several benchmark datasets were produced that record human judgements of the interpretability of topics. We are the first to propose a framework that allows to construct existing word based coherence measures as well as new ones by combining elementary components. We conduct a systematic search of the space of coherence measures using all publicly available topic relevance data for the evaluation. Our results show that new combinations of components outperform existing measures with respect to correlation to human ratings. Finally, we outline how our results can be transferred to further applications in the context of text mining, information retrieval and the world wide web.},
author = {R{\"{o}}der, Michael and Both, Andreas and Hinneburg, Alexander},
doi = {10.1145/2684822.2685324},
file = {:Users/tim/Surfdrive/Research/Library/Literature/R{\"{o}}der, Both, Hinneburg - 2015 - Exploring the space of topic coherence measures.pdf:pdf},
isbn = {9781450333177},
journal = {WSDM 2015 - Proc. 8th ACM Int. Conf. Web Search Data Min.},
keywords = {Topic coherence,Topic evaluation,Topic model},
pages = {399--408},
title = {{Exploring the space of topic coherence measures}},
year = {2015}
}
@article{Speier-Pero2019,
abstract = {Decision makers are accustomed to using decision support systems to support decision making using summarized or aggregate data. Although aggregate data minimizes the amount of data a decision maker must examine, it may not provide all the details he/she would like to have. In addition, transforming aggregate data to disaggregate data can result in aggregation bias and greater variance in decision outcomes. Alternatively, providing a decision maker with highly detailed information may result in information overload and ineffective information processing. Earlier studies examining data aggregation have ignored the influence of limited time availability, a reality found in many organizations today. A laboratory experiment using a 2x2x2 factorial design was conducted to investigate the effects of time availability, information presentation and decision task strategy on decision-making performance. Results from the experiment indicate a main effect for each of the three factors and an interaction effect between information presentation and time availability.},
annote = {this is about an intervention for people to cope with information overload; the intervention is aggregating data instead of presenting it all on its own

the author investigates the effects of time availability, information presentation and decision task strategy on decision making performance

I can take a lot from this, for example the decision making strategies and decision task operationalizations},
author = {Speier-Pero, Cheri},
doi = {10.1080/12460125.2019.1623533},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Speier-Pero - 2019 - Using aggregated data under time pressure a mechanism for coping with information overload.pdf:pdf},
issn = {21167052},
journal = {J. Decis. Syst.},
keywords = {Decision support systems,aggregation bias,information overload,time pressure},
number = {2},
pages = {82--100},
publisher = {Taylor {\&} Francis},
title = {{Using aggregated data under time pressure: a mechanism for coping with information overload}},
url = {https://doi.org/10.1080/12460125.2019.1623533},
volume = {28},
year = {2019}
}
@article{Lippi2015,
abstract = {Argumentation mining aims to automatically identify structured argument data from unstructured natural language text. This challenging, multifaceted task is recently gaining a growing attention, especially due to its many potential applications. One particularly important aspect of argumentation mining is claim identification. Most of the current approaches are engineered to address specific domains. However, argumentative sentences are often characterized by common rhetorical structures, independently of the domain. We thus propose a method that exploits structured parsing information to detect claims without resorting to contextual information, and yet achieve a performance comparable to that of state-of-the-art methods that heavily rely on the context.},
author = {Lippi, Marco and Torroni, Paolo},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Lippi, Torroni - 2015 - Context-independent claim detection for argument mining.pdf:pdf},
isbn = {9781577357384},
issn = {10450823},
journal = {IJCAI Int. Jt. Conf. Artif. Intell.},
keywords = {Technical Papers — Artificial Intellligence and So},
number = {Ijcai},
pages = {185--191},
title = {{Context-independent claim detection for argument mining}},
volume = {2015-Janua},
year = {2015}
}
@article{Hu2015,
abstract = {{\textcopyright} 2015 ACM. A large percentage of queries issued to search engines are broad or ambiguous. Search result diversification aims to solve this problem, by returning diverse results that can fulfill as many different information needs as possible. Most existing intent-aware search result diversification algorithms formulate user intents for a query as a flat list of subtopics. In this paper, we introduce a new hierarchical structure to represent user intents and propose two general hierarchical diversification models to leverage hierarchical intents. Experimental results show that our hierarchical diversification models outperform state-of-the-art diversification methods that use traditional flat subtopics.},
author = {Hu, Sha and Dou, Zhicheng and Wang, Xiaojie and Sakai, Tetsuya and Wen, Ji Rong},
doi = {10.1145/2806416.2806455},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hu et al. - 2015 - Search result diversification based on hierarchical intents.pdf:pdf},
isbn = {9781450337946},
journal = {Int. Conf. Inf. Knowl. Manag. Proc.},
keywords = {Hierarchical diversification,Hierarchical intents,Search result diversification},
pages = {63--72},
title = {{Search result diversification based on hierarchical intents}},
volume = {19-23-Oct-},
year = {2015}
}
@article{Qiu2013,
abstract = {{\textcopyright} 2013 Association for Computational Linguistics. Threaded discussion forums provide an important social media platform. Its rich user generated content has served as an important source of public feedback. To automatically discover the viewpoints or stances on hot issues from forum threads is an important and useful task. In this paper, we propose a novel latent variable model for viewpoint discovery from threaded forum posts. Our model is a principled generative latent variable model which captures three important factors: viewpoint specific topic preference, user identity and user interactions. Evaluation results show that our model clearly outperforms a number of baseline models in terms of both clustering posts based on viewpoints and clustering users with different viewpoints.},
annote = {not really useful to me because it takes into account user interactions in forums; I need to infer viewpoints from pure text and maybe author data},
author = {Qiu, Minghui and Jiang, Jing},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Qiu, Jiang - 2013 - A latent variable model for viewpoint discovery from threaded forum posts.pdf:pdf},
isbn = {9781937284473},
journal = {NAACL HLT 2013 - 2013 Conf. North Am. Chapter Assoc. Comput. Linguist. Hum. Lang. Technol. Proc. Main Conf.},
pages = {1031--1040},
title = {{A latent variable model for viewpoint discovery from threaded forum posts}},
year = {2013}
}
@article{Budzynska2019,
abstract = {This survey presents the current state of the art in Argument Mining research, concerned with automati-cally identifying arguments and relationships amongst them in natural text. The paper is structured along the following lines. (1) We give a brief introduction to Argumentation concepts and motivate the need for Argument Mining. (2) We discuss the major challenges that researchers face when developing Argument Mining solutions. (3) We present relevant theories that have had an impact on the field; (4) We give concrete examples of Argument Mining systems, algorithms and corpora/ontologies. We conclude the paper with a discussion on how theory and practice have been brought together in the past and how they may be in the future to face the challenges of this field.},
author = {Budzynska, Katarzyna and Reed, Chris},
doi = {10.18653/v1/p19-4008},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Budzynska, Reed - 2019 - Advances in Argument Mining.pdf:pdf},
pages = {39--42},
title = {{Advances in Argument Mining}},
year = {2019}
}
@article{Hefer2007,
author = {Hefer, A},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hefer - 2007 - GEMMS A Generic and Extensible Metadata Management System for Data Lakes.pdf:pdf},
number = {1921},
pages = {13--17},
title = {{GEMMS: A Generic and Extensible Metadata Management System for Data Lakes}},
year = {2007}
}
@article{Ely2001,
abstract = {This paper develops theory about the conditions under which cultural diversity enhances or detracts from work group functioning. From qualitative research in three culturally diverse organizations, we identified three different perspectives on workforce diversity: the integration-and-learning perspective, the access-and-legitimacy perspective, and the discrimination-and-fairness perspective. The perspective on diversity a work group held influenced how people expressed and managed tensions related to diversity, whether those who had been traditionally underrepresented in the organization felt respected and valued by their colleagues, and how people interpreted the meaning of their racial identity at work. These, in turn, had implications for how well the work group and its members functioned. All three perspectives on diversity had been successful in motivating managers to diversify their staffs, but only the integration-and-learning perspective provided the rationale and guidance needed to achieve sustained benefits from diversity. By identifying the conditions that intervene between the demographic composition of a work group and its functioning, our research helps to explain mixed results on the relationship between cultural diversity and work group outcomes.},
author = {Ely, Robin J. and Thomas, David A.},
doi = {10.2307/2667087},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Ely, Thomas - 2001 - Cultural diversity at work The effects of diversity perspectives on work group processes and outcomes.pdf:pdf},
issn = {00018392},
journal = {Adm. Sci. Q.},
number = {2},
pages = {229--273},
title = {{Cultural diversity at work: The effects of diversity perspectives on work group processes and outcomes}},
volume = {46},
year = {2001}
}
@article{Germano2019,
abstract = {Ranking algorithms play a crucial role in online platforms ranging from search engines to recommender systems. In this paper, we identify a surprising consequence of popularity-based rankings: the fewer the items reporting a given signal, the higher the share of the overall traffic they collectively attract. This few-get-richer effect emerges in settings where there are few distinct classes of items (e.g., left-leaning news sources versus right-leaning news sources), and items are ranked based on their popularity. We demonstrate analytically that the few-get-richer effect emerges when people tend to click on top-ranked items and have heterogeneous preferences for the classes of items. Using simulations, we analyze how the strength of the effect changes with assumptions about the setting and human behavior. We also test our predictions experimentally in an online experiment with human participants. Our findings have important implications to understand the spread of misinformation.},
annote = {The few-get-richer effect describes a phenomenon that comes with popularity-based ranking algorithms; in which the total share of web traffic (i.e., the proportion of clicks) allocated to a given class of search result items (e.g., left or right news sources, dog or cat images) decreases with the number of items that belong to this class. For example, if there are 50 items, the total number of clicks allocated to left-leaning items will be larger when there are just 3 items of that class than when there are 17 of them.
This is because as the number of items in that class decreases, the same number of people that are looking for items of that class have fewer items to choose from, and we assume that they find them somehow. When such few items get such massive amounts of clicks, they will be ranked higher and therefore attract increasing amounts of clicks due to mere position bias. This could mean that fake news could be ranked unfairly high in rankings if enough people search for and find them somehow.
The few-get-richer effect is related to the "rich-get-richer" effect observed in information retrieval, which describes that item at the top of the list will be clicked more due to position bias, which reinforces their position at the top.
the authors show in simulation and user studies that this effect does indeed occur; they discuss important implications of this effect -- not just relevant for search but also recommender systems},
archivePrefix = {arXiv},
arxivId = {1902.02580},
author = {Germano, Fabrizio and G{\'{o}}mez, Vicen{\c{c}} and {Le Mens}, Ga{\"{e}}l},
doi = {10.1145/3308558.3313693},
eprint = {1902.02580},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Germano, G{\'{o}}mez, Le Mens - 2019 - The few-get-richer A surprising consequence of popularity-based rankings.pdf:pdf},
isbn = {9781450366748},
journal = {Web Conf. 2019 - Proc. World Wide Web Conf. WWW 2019},
pages = {2764--2770},
title = {{The few-get-richer: A surprising consequence of popularity-based rankings}},
year = {2019}
}
@techreport{niklas2015profiling,
author = {Niklas, Jedrzej and Sztandar-Sztanderska, Karolina and Szymielewicz, Katarzyna},
institution = {Fundacja Panoptykon},
title = {{Profiling the unemployed in Poland: social and political implications of algorithmic decision making}},
url = {https://panoptykon.org/sites/default/files/leadimage-biblioteka/panoptykon{\_}profiling{\_}report{\_}final.pdf},
year = {2015}
}
@phdthesis{Santos,
abstract = {Queries submitted to a web search engine are typically short and often ambiguous. With the enormous size of the Web, a misunderstanding of the information need underlying an ambiguous query can misguide the search engine, ultimately leading the user to abandon the originally submitted query. In order to overcome this problem, a sensible approach is to diversify the documents retrieved for the user's query. As a result, the likelihood that at least one of these documents will satisfy the user's actual information need is increased.$\backslash$r$\backslash$n$\backslash$r$\backslash$nIn this thesis, we argue that an ambiguous query should be seen as representing not one, but multiple information needs. Based upon this premise, we propose xQuAD---Explicit Query Aspect Diversification, a novel probabilistic framework for search result diversification. In particular, the xQuAD framework naturally models several dimensions of the search result diversification problem in a principled yet practical manner. To this end, the framework represents the possible information needs underlying a query as a set of keyword-based sub-queries. Moreover, xQuAD accounts for the overall coverage of each retrieved document with respect to the identified sub-queries, so as to rank highly diverse documents first. In addition, it accounts for how well each sub-query is covered by the other retrieved documents, so as to promote novelty---and hence penalise redundancy---in the ranking. The framework also models the importance of each of the identified sub-queries, so as to appropriately cater for the interests of the user population when diversifying the retrieved documents. Finally, since not all queries are equally ambiguous, the xQuAD framework caters for the ambiguity level of different queries, so as to appropriately trade-off relevance for diversity on a per-query basis.$\backslash$r$\backslash$n$\backslash$r$\backslash$nThe xQuAD framework is general and can be used to instantiate several diversification models, including the most prominent models described in the literature. In particular, within xQuAD, each of the aforementioned dimensions of the search result diversification problem can be tackled in a variety of ways. In this thesis, as additional contributions besides the xQuAD framework, we introduce novel machine learning approaches for addressing each of these dimensions. These include a learning to rank approach for identifying effective sub-queries as query suggestions mined from a query log, an intent-aware approach for choosing the ranking models most likely to be effective for estimating the coverage and novelty of multiple documents with respect to a sub-query, and a selective approach for automatically predicting how much to diversify the documents retrieved for each individual query. In addition, we perform the first empirical analysis of the role of novelty as a diversification strategy for web search.$\backslash$r$\backslash$n$\backslash$r$\backslash$nAs demonstrated throughout this thesis, the principles underlying the xQuAD framework are general, sound, and effective. In particular, to validate the contributions of this thesis, we thoroughly assess the effectiveness of xQuAD under the standard experimentation paradigm provided by the diversity task of the TREC 2009, 2010, and 2011 Web tracks. The results of this investigation demonstrate the effectiveness of our proposed framework. Indeed, xQuAD attains consistent and significant improvements in comparison to the most effective diversification approaches in the literature, and across a range of experimental conditions, comprising multiple input rankings, multiple sub-query generation and coverage estimation mechanisms, as well as queries with multiple levels of ambiguity. Altogether, these results corroborate the state-of-the-art diversification performance of xQuAD.},
author = {Santos, Rodrygo L.T.},
doi = {10.1145/2492189.2492205},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Santos - Unknown - Explicit web search result diversification.pdf:pdf},
issn = {01635840},
school = {University of Glasgow},
title = {{Explicit web search result diversification}}
}
@misc{BayesFactorR,
abstract = {A suite of functions for computing various Bayes factors for simple designs, including contingency tables, one- and two-sample designs, one-way designs, general ANOVA designs, and linear regression.},
author = {Morey, Richard D. and Rouder, Jeffrey N.},
booktitle = {R Packag. version 0.9.12-4.2},
title = {{BayesFactor: Computation of Bayes Factors for Common Designs}},
url = {https://cran.r-project.org/package=BayesFactor},
year = {2018}
}
@article{Siau2018,
author = {Siau, Keng and Wang, Weiyu},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Siau, Wang - 2018 - Building trust in artificial intelligence, machine learning, and robotics.pdf:pdf},
issn = {24753742},
journal = {Cut. Bus. Technol. J.},
number = {2},
pages = {47--53},
title = {{Building trust in artificial intelligence, machine learning, and robotics}},
volume = {31},
year = {2018}
}
@article{Greenland2016,
abstract = {Misinterpretation and abuse of statistical tests, confidence intervals, and statistical power have been decried for decades, yet remain rampant. A key problem is that there are no interpretations of these concepts that are at once simple, intuitive, correct, and foolproof. Instead, correct use and interpretation of these statistics requires an attention to detail which seems to tax the patience of working scientists. This high cognitive demand has led to an epidemic of shortcut definitions and interpretations that are simply wrong, sometimes disastrously so—and yet these misinterpretations dominate much of the scientific literature. In light of this problem, we provide definitions and a discussion of basic statistics that are more general and critical than typically found in traditional introductory expositions. Our goal is to provide a resource for instructors, researchers, and consumers of statistics whose knowledge of statistical theory and technique may be limited but who wish to avoid and spot misinterpretations. We emphasize how violation of often unstated analysis protocols (such as selecting analyses for presentation based on the P values they produce) can lead to small P values even if the declared test hypothesis is correct, and can lead to large P values even if that hypothesis is incorrect. We then provide an explanatory list of 25 misinterpretations of P values, confidence intervals, and power. We conclude with guidelines for improving statistical interpretation and reporting.},
author = {Greenland, Sander and Senn, Stephen J. and Rothman, Kenneth J. and Carlin, John B. and Poole, Charles and Goodman, Steven N. and Altman, Douglas G.},
doi = {10.1007/s10654-016-0149-3},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Greenland et al. - 2016 - Statistical tests, P values, confidence intervals, and power a guide to misinterpretations.pdf:pdf},
issn = {15737284},
journal = {Eur. J. Epidemiol.},
keywords = {Confidence intervals,Hypothesis testing,Null testing,P value,Power,Significance tests,Statistical testing},
number = {4},
pages = {337--350},
publisher = {Springer Netherlands},
title = {{Statistical tests, P values, confidence intervals, and power: a guide to misinterpretations}},
volume = {31},
year = {2016}
}
@article{Hasan2013,
abstract = {Determining the stance expressed by an author from a post written for a two-sided debate in an online debate forum is a relatively new problem. We seek to improve Anand et al.'s (2011) approach to debate stance classification by model-ing two types of soft extra-linguistic con-straints on the stance labels of debate posts, user-interaction constraints and ide-ology constraints. Experimental results on four datasets demonstrate the effectiveness of these inter-post constraints in improv-ing debate stance classification.},
author = {Hasan, Kazi Saidul and Ng, Vincent},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hasan, Ng - 2013 - Extra-linguistic constraints on stance recognition in ideological debates.pdf:pdf},
isbn = {9781937284510},
journal = {ACL 2013 - 51st Annu. Meet. Assoc. Comput. Linguist. Proc. Conf.},
pages = {816--821},
title = {{Extra-linguistic constraints on stance recognition in ideological debates}},
volume = {2},
year = {2013}
}
@inproceedings{Fraser2019,
abstract = {Push-notifications have the potential to reinforce positive behaviours when applied in an intelligent manner. This paper explores a method of improving the delivery process of push-notifications by extracting scrutable persuasive features and refining prediction of notification outcomes. Additionally, a method is proposed for generating recommended notifications, based on the extracted persuasive features, to maximise potential engagement for scenarios such as behavioural interventions. The results illustrate that the persuasive features extracted contributed toward improved push-notification action prediction and that the personalised persuasive notifications recommended vastly increased the Click Through Rate (CTR) of notifications.},
address = {Cham},
author = {Fraser, Kieran and Yousuf, Bilal and Conlan, Owen},
booktitle = {Persuas. Technol. Dev. Persuas. Behav. Chang. Support Syst.},
editor = {{Oinas-Kukkonen H., Win K., Karapanos E., Karppinen P.}, Kyza E.},
issn = {16113349},
pages = {67----73},
publisher = {Springer International Publishing},
title = {{Scrutable and persuasive push-notifications}},
year = {2019}
}
@article{Yang2018,
abstract = {Algorithmic decisions often result in scoring and ranking individuals to determine credit worthiness, qualifications for college admissions and employment, and compatibility as dating partners. While automatic and seemingly objective, ranking algorithms can discriminate against individuals and protected groups, and exhibit low diversity. Furthermore, ranked results are often unstable-small changes in the input data or in the ranking methodology may lead to drastic changes in the output, making the result uninformative and easy to manipulate. Similar concerns apply in cases where items other than individuals are ranked, including colleges, academic departments, or products. In this demonstration we present Ranking Facts, a Web-based application that generates a "nutritional label" for rankings. Ranking Facts is made up of a collection of visual widgets that implement our latest research results on fairness, stability, and transparency for rankings, and that communicate details of the ranking methodology, or of the output, to the end user. We will showcase Ranking Facts on real datasets from different domains, including college rankings, criminal risk assessment, and financial services.},
annote = {authors present a web application that provides "nutritional labels" for rankings; for example the widgets in this app can show the user how fair the ranking is etc.

they claim that showing these "Ranking Facts" to users might mitigate user biases by increasing transparency},
archivePrefix = {arXiv},
arxivId = {1804.07890},
author = {Yang, Ke and Stoyanovich, Julia and Asudeh, Abolfazl and Howe, Bill and Jagadish, H. V. and Miklau, Gerome},
doi = {10.1145/3183713.3193568},
eprint = {1804.07890},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Yang et al. - 2018 - A nutritional label for rankings.pdf:pdf},
isbn = {9781450317436},
issn = {07308078},
journal = {Proc. ACM SIGMOD Int. Conf. Manag. Data},
number = {Section 2},
pages = {1773--1776},
title = {{A nutritional label for rankings}},
year = {2018}
}
@inproceedings{Zhai2003,
abstract = {We present a non-traditional retrieval problem we call subtopic re- trieval. The subtopic retrieval problem is concerned with finding documents that cover many different subtopics of a query topic. This means that the utility of a document in a ranking is depen- dent on other documents in the ranking, violating the assumption of independent relevance which is assumed in most traditional re- trieval methods. Subtopic retrieval poses challenges for evaluating performance, as well as for developing effective algorithms. We propose a framework for evaluating subtopic retrieval which gen- eralizes the traditional precision and recall metrics by accounting for intrinsic topic difficulty as well as redundancy in documents. We propose and systematically evaluate several methods for per- forming subtopic retrieval using statistical language models and a maximal marginal relevance (MMR) ranking strategy. A mixture model combined with query likelihood relevance ranking is shown to modestly outperform a baseline relevance ranking on a data set used in the TREC interactive track.},
author = {Zhai, Cheng Xiang and Cohen, William W and Lafferty, John},
booktitle = {Proc. 26th Annu. Int. ACM SIGIR Conf. Res. Dev. informaion Retr.},
doi = {10.1145/2795403.2795405},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Zhai, Cohen, Lafferty - 2003 - Beyond independent relevance methods and evaluation metrics for subtopic retrieval.pdf:pdf},
issn = {01635840},
keywords = {language models,maximal marginal relevance,subtopic retrieval},
pages = {10----17},
publisher = {ACM},
title = {{Beyond independent relevance: methods and evaluation metrics for subtopic retrieval}},
year = {2003}
}
@article{Matthes2008,
abstract = {The main purpose of this study was to shed light on methodological problems in the content analysis of media frames. After a review of 5 common methods, we will present an alternative procedure that aims at improving reliability and validity. Based on the definition of frames advanced by R. M. Entman (1993), we propose that previously defined frame elements systematically group together in a specific way. This pattern of frame elements can be identified across several texts by means of cluster analysis. The proposed method is demonstrated with data on the coverage of the issue of biotechnology in The New York Times. It is concluded that the proposed method yields better results in terms of reliability and validity compared to previous methods. {\textcopyright} 2008 International Communication Association.},
author = {Matthes, J{\"{o}}rg and Kohring, Matthias},
doi = {10.1111/j.1460-2466.2008.00384.x},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Matthes, Kohring - 2008 - The content analysis of media frames Toward improving reliability and validity.pdf:pdf},
issn = {00219916},
journal = {J. Commun.},
number = {2},
pages = {258--279},
title = {{The content analysis of media frames: Toward improving reliability and validity}},
volume = {58},
year = {2008}
}
@article{Borra2015,
abstract = {Collaborative content creation inevitably reaches situations where different points of view lead to conflict. We focus on Wikipedia, the free encyclopedia anyone may edit, where disputes about content in controversial articles often reflect larger societal debates. While Wikipedia has a public edit history and discussion section for every article, the substance of these sections is difficult to phantom for Wikipedia users interested in the development of an article and in locating which topics were most controversial. In this paper we present Contropedia, a tool that augments Wikipedia articles and gives insight into the development of controversial topics. Contropedia uses an efficient language agnostic measure based on the edit history that focuses on wiki links to easily identify which topics within a Wikipedia article have been most controversial and when.},
annote = {only read half of it because it is not really relevant to what I'm doing

they are introducing contropedia, a tool that measures to what degree wikipedia articles are disputed / inherit controversies; 

might be a useful tool to quickly find which topics are disputed at all; e.g., global warming is a highly disputed topic according to contropedia},
author = {Borra, Erik and Weltevrede, Esther and Ciuccarelli, Paolo and Kaltenbrunner, Andreas and Laniado, David and Magni, Giovanni and Mauri, Michele and Rogers, Richard and Venturini, Tommaso},
doi = {10.1145/2702123.2702436},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Borra et al. - 2015 - Societal Controversies in Wikipedia Articles.pdf:pdf},
isbn = {9781450331456},
pages = {193--196},
title = {{Societal Controversies in Wikipedia Articles}},
year = {2015}
}
@article{Drosou2010,
abstract = {Result diversification has recently attracted much attention as a means of increasing user satisfaction in recommender systems and web search. Many different approaches have been proposed in the related literature for the diversification problem. In this paper, we survey, classify and comparatively study the various definitions, algorithms and metrics for result diversification.},
author = {Drosou, Marina and Pitoura, Evaggelia},
doi = {10.1145/1860702.1860709},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Drosou, Pitoura - 2010 - Search result diversification.pdf:pdf},
issn = {01635808},
journal = {SIGMOD Rec.},
number = {1},
pages = {41--47},
title = {{Search result diversification}},
volume = {39},
year = {2010}
}
@article{Meek2007,
annote = {t-test robust to 5 point likert scale data},
author = {Meek, Gary E. and Ozgur, Ceyhun and Dunning, Kenneth},
doi = {10.22237/jmasm/1177992540},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Meek, Ozgur, Dunning - 2007 - Comparison of the t vs. Wilcoxon Signed-Rank Test for Likert Scale Data and Small Samples.pdf:pdf},
journal = {J. Mod. Appl. Stat. Methods},
keywords = {likert scales,nonparametric,one sample t-test,s signed-rank test,type i and,type ii error rates,wilcoxon},
number = {1},
pages = {91--106},
title = {{Comparison of the t vs. Wilcoxon Signed-Rank Test for Likert Scale Data and Small Samples}},
volume = {6},
year = {2007}
}
@article{Wang2016,
abstract = {Aspect-level sentiment analysis or opinion mining consists of several core sub-Tasks: Aspect extraction, opinion identification, polarity classification, and separation of general and aspect-specific opinions. Various topic models have been proposed by researchers to address some of these sub-Tasks. However, there is little work on modeling all of them together. In this paper, we first propose a holistic fine-grained topic model, called the JAST (Joint Aspectbased Sentiment Topic) model, that can simultaneously model all of above problems under a unified framework. To further improve it, we incorporate the idea of lifelong machine learning and propose a more advanced model, called the LAST (Lifelong Aspectbased Sentiment Topic) model. LAST automatically mines the prior knowledge of aspect, opinion, and their correspondence from other products or domains. Such knowledge is automatically extracted and incorporated into the proposed LAST model without any human involvement. Our experiments using reviews of a large number of product domains show major improvements of the proposed models over state-of-The-Art baselines.},
author = {Wang, Shuai and Chen, Zhiyuan and Liu, Bing},
doi = {10.1145/2872427.2883086},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Wang, Chen, Liu - 2016 - Mining aspect-specific opinion using a holistic lifelong topic model.pdf:pdf},
isbn = {9781450341431},
journal = {25th Int. World Wide Web Conf. WWW 2016},
keywords = {Aspect-Specific Opinion,Lifelong Machine Learning,Opinion Mining,Topic Model},
pages = {167--176},
title = {{Mining aspect-specific opinion using a holistic lifelong topic model}},
year = {2016}
}
@article{Schrenk1969,
abstract = {Despite an increasing capability for automating various tasks there continues to be a requirement for man to serve as the decision element in many complex systems. The complexity and far-reaching consequences of many decisions impels a concern for improving decision-making performance in man-machine systems. In this paper current knowledge regarding human decision behaviour and methods for aiding this behaviour are briefly reviewed. A tentative, conceptual model of an idealized process of decision making is presented. This model, which is based on both empirical and theoretical research, contains throe phases. These are (1) problem recognition, (2) problem diagnosis, and (3) action selection. The model is intended primarily to provide a guide to system designers in structuring decision tasks and a framework for organizing knowledge about decision-making behaviour. {\textcopyright} 1969 Walter de Gruyter. All rights reserved.},
annote = {old paper(!) but nice conceptualization of the general decision-making process; flowcharts available (could be used at some point)},
author = {Schrenk, L. P.},
doi = {10.1080/00140136908931079},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Schrenk - 1969 - Aiding the Decision Maker—A Decision Process Model.pdf:pdf},
issn = {13665847},
journal = {Ergonomics},
number = {4},
pages = {543--557},
title = {{Aiding the Decision Maker—A Decision Process Model}},
volume = {12},
year = {1969}
}
@article{Chandar2013,
abstract = {Novel and diverse document ranking is an effective strategy that involves reducing redundancy in a ranked list to maximize the amount of novel and relevant information available to users. Evaluation for novelty and diversity typically involves an assessor judging each document for relevance against a set of pre-identified subtopics, which may be disambiguations of the query, facets of an information need, or nuggets of information. Alternately, when expressing a $\backslash$emph{\{}preference{\}} for document A or document B, users may implicitly take subtopics into account, but may also take into account other factors such as recency, readability, length, and so on, each of which may have more or less importance depending on user. A $\backslash$emph{\{}user profile{\}} contains information about the extent to which each factor, including subtopic relevance, plays a role in the user's preference for one document over another. A preference-based evaluation can then take this user profile information into account to better model utility to the space of users. In this work, we propose an evaluation framework that not only can consider implicit factors but also handles differences in user preference due to varying underlying information need. Our proposed framework is based on the idea that a user scanning a ranked list from top to bottom and stopping at rank k gains some utility from every document that is relevant their information need. Thus, we model the expected utility of a ranked list by estimating the utility of a document at a given rank using preference judgments and define evaluation measures based on the same. We validate our framework by comparing it to existing measures such as $\alpha$-nDCG, ERR-IA, and subtopic recall that require explicit subtopic judgments We show that our proposed measures correlate well with existing measures while having the potential to capture various other factors when real data is used. We also show that the proposed measures can easily handle relevance assessments against multiple user profiles, and that they are robust to noisy and incomplete judgments.},
author = {Chandar, Praveen and Carterette, Ben},
doi = {10.1145/2484028.2484094},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Chandar, Carterette - 2013 - Preference based evaluation measures for novelty and diversity.pdf:pdf},
isbn = {9781450320344},
journal = {SIGIR 2013 - Proc. 36th Int. ACM SIGIR Conf. Res. Dev. Inf. Retr.},
keywords = {Evaluation,Novelty and diversity},
pages = {413--422},
title = {{Preference based evaluation measures for novelty and diversity}},
year = {2013}
}
@article{Catlett1991,
abstract = {The large real-world datasets now commonly tackled by machine learning algorithms are often described in terms of attributes whose values are real numbers on some continuous interval, rather than being taken from a small number of discrete values. Many algorithms are able to handle continuous attributes, but learning requires far more CPU time than for a corresponding task with discrete attributes. This paper describes how continuous attributes can be converted economically into ordered discrete attributes before being given to the learning system. Experimental results from a wide variety of domains suggest this change of representation does not often result in a significant loss of accuracy (in fact it sometimes significantly improves accuracy), but offers large reductions in learning time, typically more than a factor of 10 in domains with a large number of continuous attributes.},
author = {Catlett, J.},
doi = {10.1007/BFb0017012},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Catlett - 1991 - On changing continuous attributes into ordered discrete attribute.pdf:pdf},
isbn = {9783540538165},
issn = {16113349},
journal = {Lect. Notes Comput. Sci. (including Subser. Lect. Notes Artif. Intell. Lect. Notes Bioinformatics)},
keywords = {Discretisation,Empirical concept learning,Induction of decision trees},
number = {1989},
pages = {164--178},
title = {{On changing continuous attributes into ordered discrete attribute}},
volume = {482 LNAI},
year = {1991}
}
@misc{R,
abstract = {R Core Team (2018). R: A language and environment for statistical computing. R Foundation for Statistical Computing, Vienna, Austria. URL http://www.R-project.org/.},
author = {{R Core Team}},
booktitle = {R Found. Stat. Comput.},
pages = {https://www.R--project.org},
publisher = {Foundation for Statistical Computing},
title = {{A Language and Environment for Statistical Computing}},
url = {http://www.r-project.org},
year = {2020}
}
@misc{Napierala2012,
abstract = {The Bonferroni correction is an adjustment made to P values when several dependent or independent statistical tests are being performed simultaneously on a single data set. To perform a Bonferroni correction, divide the critical P value ($\alpha$) by the number of comparisons being made. For example, if 10 hypotheses are being tested, the new critical P value would be $\alpha$/10. The statistical power of the study is then calculated based on this modified P value. The Bonferroni correction is used to reduce the chances of obtaining false-positive results (type I errors) when multiple pair wise tests are performed on a single set of data. Put simply, the probability of identifying at least one significant result due to chance increases as more hypotheses are tested. For example, a researcher is testing 20 hypotheses simultaneously, with a critical P value of 0.05. In this case, the following would be true: P (at least one significant result) = 1 – P (no significant results) P (at least one significant result) = 1 – (1-0.05) 20 P (at least one significant result) = 0.64 Thus, performing 20 tests on a data set yields a 64 percent chance of identifying at least one significant result, even if all of the tests are actually not significant. Therefore, while a given $\alpha$ may be appropriate for each individual comparison, it may not be appropriate for the set of all comparisons. This fact is potentially problematic because in contemporary orthopaedic research studies, numerous simultaneous tests are routinely performed. Thus, to avoid a large number of spurious positives, $\alpha$ must be lowered to account for the number of comparisons being performed. The Bonferroni correction is based on the idea that if an experimenter is testing n dependent or independent hypotheses on a set of data, the probability of type I error is offset by testing each hypothesis at a statistical significance level 1/ n times what it would be if only one hypothesis were tested.},
author = {{Napierala, M}, A.},
booktitle = {AAOS Now},
title = {{What Is the Bonferroni correction?}},
url = {http://www.aaos.org/news/aaosnow/apr12/research7.asp},
year = {2012}
}
@inproceedings{Augenstein2016,
abstract = {Stance detection is the task of classifying the attitude expressed in a text towards a target such as Hillary Clinton to be "positive", negative" or "neutral". Previous work has assumed that either the target is mentioned in the text or that training data for every target is given. This paper considers the more challenging version of this task, where targets are not always mentioned and no training data is available for the test targets. We experiment with conditional LSTM encoding, which builds a representation of the tweet that is dependent on the target, and demonstrate that it outperforms encoding the tweet and the target independently. Performance is improved further when the conditional model is augmented with bidirectional encoding. We evaluate our approach on the SemEval 2016 Task 6 Twitter Stance Detection corpus achieving performance second best only to a system trained on semi-automatically labelled tweets for the test target. When such weak supervision is added, our approach achieves state-of-the-art results.},
archivePrefix = {arXiv},
arxivId = {arXiv:1606.05464v2},
author = {Augenstein, Isabelle and Rockt{\"{a}}schel, Tim and Vlachos, Andreas and Bontcheva, Kalina},
booktitle = {Proc. Conf. Empir. Methods Nat. Lang. Process.},
doi = {10.18653/v1/d16-1084},
eprint = {arXiv:1606.05464v2},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Augenstein et al. - 2016 - Stance Detection with Bidirectional Conditional Encoding.pdf:pdf},
pages = {876--885},
title = {{Stance Detection with Bidirectional Conditional Encoding}},
year = {2016}
}
@article{Kulshrestha2017,
abstract = {Search systems in online social media sites are frequently used to find information about ongoing events and people. For topics with multiple competing perspectives, such as political events or political candidates, bias in the top ranked results significantly shapes public opinion. However, bias does not emerge from an algorithm alone. It is important to distinguish between the bias that arises from the data that serves as the input to the ranking system and the bias that arises from the ranking system itself. In this paper, we propose a framework to quantify these distinct biases and apply this framework to politics-related queries on Twitter. We found that both the input data and the ranking system contribute significantly to produce varying amounts of bias in the search results and in different ways. We discuss the consequences of these biases and possible mechanisms to signal this bias in social media search systems' interfaces.},
archivePrefix = {arXiv},
arxivId = {1704.01347},
author = {Kulshrestha, Juhi and Eslami, Motahhare and Messias, Johnnatan and Zafar, Muhammad Bilal and Ghosh, Saptarshi and Gummadi, Krishna P. and Karahalios, Karrie},
doi = {10.1145/2998181.2998321},
eprint = {1704.01347},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Kulshrestha et al. - 2017 - Quantifying search bias Investigating sources of bias for political searches in social media.pdf:pdf},
isbn = {9781450343350},
journal = {Proc. ACM Conf. Comput. Support. Coop. Work. CSCW},
keywords = {Political bias inference,Search bias,Search bias quantification,Social media search,Sources of search bias,Twitter},
pages = {417--432},
title = {{Quantifying search bias: Investigating sources of bias for political searches in social media}},
year = {2017}
}
@article{Newman2010,
author = {Newman, David and Noh, Youn and Talley, Edmund and Karimi, Sarvnaz and Baldwin, Timothy},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Newman et al. - 2010 - Evaluating Topic Models for Digital Libraries Categories and Subject Descriptors.pdf:pdf},
isbn = {9781450300858},
journal = {Jcdl},
keywords = {acm acknowl-,computing machinery,copyright 2010 association for,corresponding author,topic models,user evaluation},
pages = {215--224},
title = {{Evaluating Topic Models for Digital Libraries Categories and Subject Descriptors}},
year = {2010}
}
@article{GPowerFaul2007,
abstract = {G*Power (Erdfelder, Faul, {\&} Buchner, 1996) was designed as a general stand-alone power analysis program for statistical tests commonly used in social and behavioral research. G*Power 3 is a major extension of, and improvement over, the previous versions. It runs on widely used computer platforms (i.e., Windows XP, Windows Vista, and Mac OS X 10.4) and covers many different statistical tests of the t, F, and $\chi$2 test families. In addition, it includes power analyses for z tests and some exact tests. G*Power 3 provides improved effect size calculators and graphic options, supports both distribution-based and design-based input modes, and offers all types of power analyses in which users might be interested. Like its predecessors, G*Power 3 is free. Copyright 2007 Psychonomic Society, Inc.},
author = {Faul, Franz and Erdfelder, Edgar and Lang, Albert Georg and Buchner, Axel},
doi = {10.3758/BF03193146},
issn = {1554351X},
journal = {Behav. Res. Methods},
number = {2},
pages = {175----191},
pmid = {17695343},
title = {{G*Power 3: A flexible statistical power analysis program for the social, behavioral, and biomedical sciences}},
volume = {39},
year = {2007}
}
@article{Balog2020,
abstract = {Explanations have a large effect on how people respond to recommendations. However, there are many possible intentions a system may have in generating explanations for a given recommendation-from increasing transparency, to enabling a faster decision, to persuading the recipient. As a good explanation for one goal may not be good for others, we address the questions of (1) how to robustly measure if an explanation meets a given goal and (2) how the different goals interact with each other. Specifically, this paper presents a first proposal of how to measure the quality of explanations along seven common goal dimensions catalogued in the literature. We find that the seven goals are not independent, but rather exhibit strong structure. Proposing two novel explanation evaluation designs, we identify challenges in evaluation, and provide more efficient measurement approaches of explanation quality. CCS CONCEPTS • Information systems → Recommender systems; Presentation of retrieval results; • Human-centered computing → Natural language interfaces; HCI design and evaluation methods.},
annote = {the authors aim to measure recommendation explanation quality; explanations have certain defined goals -- but how can we measure whether the explanations fulfill these goals?

they let crowdworkers come up with explanations and then let participants evaluate those},
author = {Balog, Krisztian and Radlinski, Filip},
doi = {10.1145/3397271.3401032},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Balog, Radlinski - 2020 - Measuring Recommendation Explanation Quality.pdf:pdf},
isbn = {9781450380164},
keywords = {2020,Recommendations,acm reference format,evaluation,explanations,krisztian balog and filip,measuring recommendation ex-,radlinski,recommendations},
pages = {329--338},
title = {{Measuring Recommendation Explanation Quality}},
year = {2020}
}
@article{Kahan2016,
abstract = {This research note presents evidence that political polarization over the reality of human-caused climate change increases in tandem with individuals' scores on a standard measure of actively open-minded thinking. This finding is at odds with the position that attributes political conflict over facts to a personality trait of closed-mindedness associated with political conservatism.},
author = {Kahan, Dan M. and Corbin, Jonathan C.},
doi = {10.1177/2053168016676705},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Kahan, Corbin - 2016 - A note on the perverse effects of actively open-minded thinking on climate-change polarization.pdf:pdf},
issn = {20531680},
journal = {Res. Polit.},
keywords = {Actively open-minded thinking,Climate change,Decision science,Motivated reasoning,Political polarization},
number = {4},
title = {{A note on the perverse effects of actively open-minded thinking on climate-change polarization}},
volume = {3},
year = {2016}
}
@article{Celis2018,
abstract = {Ranking algorithms are deployed widely to order a set of items in applications such as search engines, news feeds, and recommendation systems. Recent studies, however, have shown that, left unchecked, the output of ranking algorithms can result in decreased diversity in the type of content presented, promote stereotypes, and polarize opinions. In order to address such issues, we study the following variant of the traditional ranking problem when, in addition, there are fairness or diversity constraints. Given a collection of items along with 1) the value of placing an item in a particular position in the ranking, 2) the collection of sensitive attributes (such as gender, race, political opinion) of each item and 3) a collection of constraints that, for each k, bound the number of items with each attribute that are allowed to appear in the top k positions of the ranking, the goal is to output a ranking that maximizes the value with respect to the original rank quality metric while respecting the constraints. This problem encapsulates various well-studied problems related to bipartite and hypergraph matching as special cases and turns out to be hard to approximate even with simple constraints. Our main technical contributions are fast exact and approximation algorithms along with complementary hardness results that, together, come close to settling the approximability of this constrained ranking maximization problem. Unlike prior work on the constrained matching problems, our algorithm runs in linear time, even when the number of constraints is large, its approximation ratio does not depend on the number of constraints, and it produces solutions with small constraint violations. Our results rely on insights about the constrained matching problem when the objective satisfies properties that appear in common ranking metrics such as Discounted Cumulative Gain, Spearman's rho or Bradley-Terry.},
annote = {this well-cited paper presents an algorithm for ranking according to utility under fairness constraints

quite technical, but can be used to implement a fair ranking algorithm if that is needed at some point

similar to Zehlike et al. (2017) and Singh {\&} Joachims (2018)},
archivePrefix = {arXiv},
arxivId = {arXiv:1704.06840v4},
author = {Celis, L. Elisa and Straszak, Damian and Vishnoi, Nisheeth K.},
doi = {10.4230/LIPIcs.ICALP.2018.28},
eprint = {arXiv:1704.06840v4},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Celis, Straszak, Vishnoi - 2018 - Ranking with fairness constraints.pdf:pdf},
isbn = {9783959770767},
issn = {18688969},
journal = {Leibniz Int. Proc. Informatics, LIPIcs},
keywords = {Approximation Algorithms,Fairness,Matching,Optimization,Ranking},
pages = {1--32},
title = {{Ranking with fairness constraints}},
volume = {107},
year = {2018}
}
@article{White2014,
abstract = {People frequently answer consequential questions, such as those with a medical focus, using Internet search engines. Their primary goal is to revise or establish beliefs in one or more outcomes. Search engines are not designed to furnish answers, and instead provide results that may contain answers. Information retrieval research has targeted aspects of information access such as query formulation, relevance, and search success. However, there are important unanswered questions on how beliefs-and potential biases in those beliefs-affect search behaviors and how beliefs are shaped by searching. To understand belief dynamics, we focus on yes-no medical questions (e.g., "Is congestive heart failure a heart attack?"), with consensus answers from physicians. We show that (a) presearch beliefs are affected only slightly by searching and changes are likely to skew positive (yes); (b) presearch beliefs affect search behavior; (c) search engines can shift some beliefs by manipulating result rank and availability, but strongly-held beliefs are difficult to move using uncongenial information and can be counterproductive, and (d) search engines exhibit near-random answer accuracy. Our findings suggest that search engines should provide correct answers to searchers' questions and develop methods to persuade searchers to shift strongly held but factually incorrect beliefs.},
annote = {nice paper to read when it comes to influence of the content of SERPs on people's beliefs and behavior;

evidence for confirmation bias 

how do beliefs change during the search process?

they also studied some interventions and the influence of presearch beliefs -- lots of good stuff in here

this was again about medical context; similar to other studies by White},
author = {White, Ryen W.},
doi = {10.1002/asi.23128},
file = {:Users/tim/Surfdrive/Research/Library/Literature/White - 2014 - Belief dynamics in web search.pdf:pdf},
issn = {23301643},
journal = {J. Assoc. Inf. Sci. Technol.},
keywords = {information seeking,user studies},
number = {11},
pages = {2165--2178},
title = {{Belief dynamics in web search}},
volume = {65},
year = {2014}
}
@article{Park2019,
abstract = {Drawing upon Bandura's self-efficacy theory, this study conceptualizes “social media news efficacy” and examines how news efficacy connects perceived news overload on social media to news avoidance and social filtering. Findings from a two-wave panel survey of South Korean adults show that news overload is significantly related to a decrease of news efficacy, which in turn increases news avoidance on social media. The analysis also finds that news efficacy mediates the positive link between perceived news overload and social filtering over time.},
annote = {this examines the relationship between news overload on social media (recommender systems) to news avoidance and social filtering in the context of Bandura's self-efficacy theory

people who experience news overload read the news less (avoidance) and have increased social filtering},
author = {Park, Chang Sup},
doi = {10.1177/2056305119872956},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Park - 2019 - Does Too Much News on Social Media Discourage News Seeking Mediating Role of News Efficacy Between Perceived News Overload.pdf:pdf},
isbn = {2056305119},
issn = {20563051},
journal = {Soc. Media Soc.},
keywords = {news avoidance,news efficacy,news overload,social filtering,social media},
number = {3},
title = {{Does Too Much News on Social Media Discourage News Seeking? Mediating Role of News Efficacy Between Perceived News Overload and News Avoidance on Social Media}},
volume = {5},
year = {2019}
}
@article{Santos2015,
author = {Santos, Rodrygo L.T. and MacDonald, Craig and Ounis, Iadh},
doi = {10.1561/1500000040},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Santos, MacDonald, Ounis - 2015 - Search result diversification.pdf:pdf},
issn = {15540677},
journal = {Found. Trends Inf. Retr.},
number = {1},
pages = {1--90},
title = {{Search result diversification}},
volume = {9},
year = {2015}
}
@article{Yeh,
abstract = {We present a new Dutch news dataset with labeled partisanship. The dataset contains more than 100K articles that are labeled on the publisher level and 776 articles that were crowd-sourced using an internal survey platform and labeled on the article level. In this paper, we document our original motivation, the collection and annotation process, limitations, and applications.},
archivePrefix = {arXiv},
arxivId = {1908.02322v1},
author = {Yeh, Chia-Lun and Loni, Babak and Hendriks, Mari{\"{e}}lle and Reinhardt, Henrike and Schuth, Anne},
eprint = {1908.02322v1},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Yeh et al. - Unknown - DpgMedia2019 A Dutch News Dataset for Partisanship Detection.pdf:pdf},
title = {{DpgMedia2019: A Dutch News Dataset for Partisanship Detection}},
url = {https://github.com/}
}
@article{Olteanu2019,
abstract = {Social data in digital form, which includes user-generated content, expressed or implicit relationships between people, and behavioral traces, are at the core of many popular applications and platforms, driving the research agenda of many researchers.  The promises of social data are many, including understanding "what the world thinks" about a social issue, brand, product, celebrity, or other entity, as well as enabling better decision-making in a variety of fields including public policy, healthcare, and economics.  Many academics and practitioners have warned against the na{\"{i}}ve usage of social data.  There are biases and inaccuracies occurring at the source of the data, but also introduced during processing.  There are methodological limitations and pitfalls, as well as ethical boundaries and unexpected consequences that are often overlooked.  This survey recognizes the rigor with which these issues are addressed by different researchers varies across a wide range.  We present a framework for identifying a broad variety of menaces in the research and practices around social data use. },
annote = {similar to the idea I had about misrepresentativeness of twitter data for public opinion inference},
author = {Olteanu, Alexandra and Castillo, Carlos and Diaz, Fernando and Kıcıman, Emre},
doi = {10.3389/fdata.2019.00013},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Olteanu et al. - 2019 - Social Data Biases, Methodological Pitfalls, and Ethical Boundaries.pdf:pdf},
journal = {Front. Big Data},
keywords = {biases,ethics,evaluation,social media,social media, user data, biases, evaluation, ethic,user data},
number = {July},
title = {{Social Data: Biases, Methodological Pitfalls, and Ethical Boundaries}},
volume = {2},
year = {2019}
}
@article{Pitoura2018,
abstract = {Bias in online information has recently become a pressing issue, with search engines, social networks and recommendation services being accused of exhibiting some form of bias. In this vision paper, we make the case for a systematic approach towards measuring bias. To this end, we discuss formal measures for quantifying the various types of bias, we outline the system components necessary for realizing them, and we highlight the related research challenges and open problems.},
author = {Pitoura, Evaggelia and Tsaparas, Panayiotis and Flouris, Giorgos and Fundulaki, Irini and Papadakos, Panagiotis and Abiteboul, Serge and Weikum, Gerhard},
doi = {10.1145/3186549.3186553},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Pitoura et al. - 2018 - On Measuring Bias in Online Information.pdf:pdf},
issn = {01635808},
journal = {ACM SIGMOD Rec.},
number = {4},
pages = {16--21},
title = {{On Measuring Bias in Online Information}},
url = {http://dl.acm.org/citation.cfm?doid=3186549.3186553},
volume = {46},
year = {2018}
}
@article{He2011,
abstract = {In this paper, we present a novel weakly-supervised method for crosslingual sentiment analysis. In specific, we propose a latent sentiment model (LSM) based on latent Dirichlet allocation where sentiment labels are considered as topics. Prior information extracted from English sentiment lexicons through machine translation are incorporated into LSM model learning, where preferences on expectations of sentiment labels of those lexicon words are expressed using generalized expectation criteria. An efficient parameter estimation procedure using variational Bayes is presented. Experimental results on the Chinese product reviews show that the weakly-supervised LSM model performs comparably to supervised classifiers such as Support vector Machines with an average of 81{\%} accuracy achieved over a total of 5484 review documents. Moreover, starting with a generic sentiment lexicon, the LSM model is able to extract highly domainspecific polarity words from text.},
author = {He, Yulan},
file = {:Users/tim/Surfdrive/Research/Library/Literature/He - 2011 - Latent sentiment model for weakly-supervised cross-lingual sentiment classification.pdf:pdf},
isbn = {9783642201608},
issn = {16113349},
journal = {Lect. Notes Comput. Sci. (including Subser. Lect. Notes Artif. Intell. Lect. Notes Bioinformatics)},
keywords = {Cross-lingual sentiment analysis,Generalized expectation,Latent Dirichlet allocation,Latent sentiment model (LSM)},
pages = {214--225},
title = {{Latent sentiment model for weakly-supervised cross-lingual sentiment classification}},
volume = {6611 LNCS},
year = {2011}
}
@article{Timmermans2017,
author = {Timmermans, B and Aroyo, L and Kuhn, T and Beelen, K and Kanoulas, E and van de Velde, B and van Eerten, G},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Timmermans et al. - 2017 - ControCurator Understanding Controversy Using Collective Intelligence.pdf:pdf},
journal = {Collect. Intell.},
pages = {2015--2018},
title = {{ControCurator: Understanding Controversy Using Collective Intelligence}},
year = {2017}
}
@article{angwin2019machine,
author = {Angwin, Julia and Larson, Jeff and Mattu, Surya and Kirchner, Lauren},
journal = {ProPublica},
title = {{Machine bias: There's software used across the country to predict future criminals and it's biased against blacks}},
url = {https://www.propublica.org/article/machine-bias-risk-assessments-in-criminal-sentencing},
year = {2019}
}
@article{Vargas2011,
abstract = {The Recommender Systems community is paying increasing attention to novelty and diversity as key qualities beyond accuracy in real recommendation scenarios. Despite the raise of interest and work on the topic in recent years, we find that a clear common methodological and conceptual ground for the evaluation of these dimensions is still to be consolidated. Different evaluation metrics have been reported in the literature but the precise relation, distinc- tion or equivalence between them has not been explicitly studied. Furthermore, the metrics reported so far miss important properties such as taking into consideration the ranking of recommended items, or whether items are relevant or not, when assessing the novelty and diversity of recommendations. We present a formal framework for the definition of novelty and diversity metrics that unifies and generalizes several state of the art metrics. We identify three essential ground concepts at the roots of novelty and diversity: choice, discovery and relevance, upon which the framework is built. Item rank and relevance are introduced through a probabilistic recommendation browsing model, building upon the same three basic concepts. Based on the combination of ground elements, and the assumptions of the browsing model, differ- ent metrics and variants unfold. We report experimental observations which validate and illustrate the properties of the proposed metrics.},
annote = {this is more about novelty than diversity; and it's about recommender systems

they do talk about diversity but present more of a general framework given some sort of distance function d(i{\_}k, i{\_}l)},
author = {Vargas, Sa{\'{u}}l and Castells, Pablo},
doi = {10.1145/2043932.2043955},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Vargas, Castells - 2011 - Rank and relevance in novelty and diversity metrics for recommender systems.pdf:pdf},
isbn = {9781450306836},
journal = {Proc. fifth ACM Conf. Recomm. Syst. - RecSys '11},
keywords = {diversity,evaluation,metrics,novelty,recommender systems},
pages = {109},
title = {{Rank and relevance in novelty and diversity metrics for recommender systems}},
url = {http://dl.acm.org/citation.cfm?doid=2043932.2043955},
year = {2011}
}
@article{Trabelsi2015,
abstract = {This work suggests a fine-grained mining of contentious documents, specifically online debates, towards a summarization of contention issues. We propose a Joint Topic Viewpoint model (JTV) for the un-supervised identification and the clustering of arguing expressions according to the latent topics they discuss and the implicit viewpoints they voice. A set of experiments is conducted on online debates documents. Qualitative and quantitative evaluations of the model's output are performed in context of different contention issues. Analysis of experimental results shows the effectiveness of the proposed model to automatically and accurately detect recurrent patterns of arguing expressions in online debate texts.},
author = {Trabelsi, Amine and Zaiane, Osmar R.},
doi = {10.3115/v1/w14-1305},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Trabelsi, Zaiane - 2015 - Finding Arguing Expressions of Divergent Viewpoints in Online Debates.pdf:pdf},
pages = {35--43},
title = {{Finding Arguing Expressions of Divergent Viewpoints in Online Debates}},
year = {2015}
}
@article{Baudin2007,
abstract = {Software algorithms are changing how people work in an ever-growing number of fields, managing distributed human workers at a large scale. In these work settings, human jobs are assigned, optimized, and evaluated through algorithms and tracked data. We explored the impact of this algorithmic, data-driven management on human workers and work practices in the context of Uber and Lyft, new ridesharing services. Our findings from a qualitative study describe how drivers responded when algorithms assigned work, provided informational support, and evaluated their performance, and how drivers used online forums to socially make sense of the algorithm features. Implications and future work are discussed.},
author = {Baudin, Michel},
doi = {10.4324/9780429272806},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Baudin - 2007 - Working with Machines.pdf:pdf},
isbn = {9781450331456},
journal = {Work. with Mach.},
pages = {1603--1612},
title = {{Working with Machines}},
year = {2007}
}
@article{Woodruff2018,
abstract = {Algorithmic systems increasingly shape information people are exposed to as well as influence decisions about employment, finances, and other opportunities. In some cases, algorithmic systems may be more or less favorable to certain groups or individuals, sparking substantial discussion of algorithmic fairness in public policy circles, academia, and the press. We broaden this discussion by exploring how members of potentially affected communities feel about algorithmic fairness. We conducted workshops and interviews with 44 participants from several populations traditionally marginalized by categories of race or class in the United States. While the concept of algorithmic fairness was largely unfamiliar, learning about algorithmic (un)fairness elicited negative feelings that connect to current national discussions about racial injustice and economic inequality. In addition to their concerns about potential harms to themselves and society, participants also indicated that algorithmic fairness (or lack thereof) could substantially affect their trust in a company or product.},
annote = {this is a survey exploring the attitudes and perceptions of people towards algorithmic fairness

main finding: once learning what algorithmic unfairness entails, people got concerned about it and also said that this COULD affect their trust in a company or product},
author = {Woodruff, Allison and Fox, Sarah E. and Rousso-Schindler, Steven and Warshaw, Jeff},
doi = {10.1145/3173574.3174230},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Woodruff et al. - 2018 - A qualitative exploration of perceptions of algorithmic fairness.pdf:pdf},
isbn = {9781450356206},
journal = {Conf. Hum. Factors Comput. Syst. - Proc.},
keywords = {Algorithmic discrimination,Algorithmic fairness},
pages = {1--14},
title = {{A qualitative exploration of perceptions of algorithmic fairness}},
volume = {2018-April},
year = {2018}
}
@inproceedings{Cham2019,
abstract = {The concept of goals is prominent in information systems and also artificial intelligence literature such as goal-oriented requirements engineering and self-adaptive systems. Digital motivation systems, e.g. gamification and persuasive technology, utilise the concept of behavioural goals which require a different mind-set on how to elicit and set them up, how to monitor deviation from such goals and how to ensure their completion. Behavioural goals are characterised by a range of factors which are not the main focus in classic information systems and AI literature such as self-efficacy, perceived usefulness. To engineer software supporting goal setting, a concretised taxonomy of goals would help a better-managed analysis and design process. In this paper, we provide a detailed classification of behavioural goals and their associated properties and elements (types, sources, monitoring, feedback, deviation and countermeasures). As a method, we review the literature on goal setting theory and its application in different disciplines. We subsequently develop five reference checklists which would act as a reference point for researchers and practitioners in persuasive and motivational systems.},
address = {Cham},
author = {Cham, Sainabou and Algashami, Abdullah and McAlaney, John and Stefanidis, Angelos and Phalp, Keith and Ali, Raian},
booktitle = {Persuas. Technol. Dev. Persuas. Behav. Chang. Support Syst.},
editor = {{Oinas-Kukkonen H., Win K., Karapanos E., Karppinen P.}, Kyza E.},
issn = {16113349},
pages = {237----253},
publisher = {Springer International Publishing},
title = {{Goal setting for persuasive information systems: Five reference checklists}},
year = {2019}
}
@article{Calder2015,
abstract = {Durch die am 29.11.2007 vom Europ{\"{a}}ischen Parlament verabschiedete Fernsehrichtlinie wird es den Staaten der EU erm{\"{o}}glicht, Product Placement unter bestimmten Auflagen als Werbeform im Fernsehen zuzulassen. 1 Eine Legalisierung von Produktplatzierungen w{\"{a}}re f{\"{u}}r die werbetreibende Wirtschaft insofern interessant, als mit der zunehmenden Konkurrenz von Werbebotschaften auch die Gefahr w{\"{a}}chst, dass Rezipienten mit Reaktanz auf klassische Werbung reagieren. In dieser Situation erscheint die Integration von Marken und Produkten in Medieninhalte als attraktive Alternative. Allerdings stellt sich die Frage, ob Produktplatzierungen tats{\"{a}}chlich halten, was sie versprechen, und ob der oft propagierte Vorteil dieser Werbeform — ihre geringere Aufdringlichkeit — nicht zugleich ihr gr{\"{o}}{\ss}ter Nachteil ist, d.h. Placements von den Rezipienten kaum bemerkt und nur in geringem Ma{\ss}e erinnert werden. Der vorliegende Forschungs{\"{u}}berblick soll aufzeigen, was wissenschaftliche Studien bislang an Erkenntnissen zur Wirkung von Placements in Film und Fernsehen sowie in Computerspielen erbracht haben, inwieweit diese Befunde einer methodenkritischen Betrachtung standhalten und welche Folgerungen f{\"{u}}r die Praxis sich daraus ableiten lassen. 2},
author = {Calder, Bobby J. and Malthouse, Edward C.},
doi = {10.1002/9781119198154.ch1},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Calder, Malthouse - 2015 - Media Engagement and Advertising Effectiveness.pdf:pdf},
journal = {Kellogg Advert. Media},
pages = {1--36},
title = {{Media Engagement and Advertising Effectiveness}},
year = {2015}
}
@article{Metaxa2019,
abstract = {Concern about algorithmically-curated content and its impact on democracy is reaching a fever pitch worldwide. But relative to the role of social media in electoral processes, the role of search results has received less public attention. We develop a theoretical conceptualization of search results as a form of media—search media—and analyze search media in the context of political partisanship in the six months leading up to the 2018 U.S. midterm elections. Our empirical analyses use a total of over 4 million URLs, scraped daily from Google search queries for all candidates running for federal office in the United States in 2018. In our first set of analyses we characterize the nature of search media from the data collected in terms of the types of URLs present and the stability of search results over time. In our second, we annotate URLs' top-level domains with existing measures of political partisanship, examining trends by incumbency, election outcome, and other election characteristics. Among other findings, we note that partisanship trends in search media are largely similar for content about candidates from the two major political parties, whereas there are substantial differences in search media for incumbent versus challenger candidates. This work suggests that longitudinal, systematic audits of search media can reflect real-world political trends. We conclude with implications for web search designers and consumers of political content online.},
author = {Metaxa, Dana{\"{e}} and Park, Joon Sung and Landay, James A. and Hancock, Jeff},
doi = {10.1145/3359231},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Metaxa et al. - 2019 - Search media and elections A longitudinal investigation of political search results in the 2018 U.S. Elections.pdf:pdf},
issn = {25730142},
journal = {Proc. ACM Human-Computer Interact.},
keywords = {Political partisanship,Search engine results,Search media},
number = {CSCW},
title = {{Search media and elections: A longitudinal investigation of political search results in the 2018 U.S. Elections}},
volume = {3},
year = {2019}
}
@article{Mimno2011,
abstract = {Latent variable models have the potential to add value to large document collections by discovering interpretable, low-dimensional subspaces. In order for people to use such models, however, they must trust them. Unfortunately, typical dimensionality reduction methods for text, such as latent Dirichlet allocation, often produce low-dimensional subspaces (topics) that are obviously flawed to human domain experts. The contributions of this paper are threefold: (1) An analysis of the ways in which topics can be flawed; (2) an automated evaluation metric for identifying such topics that does not rely on human annotators or reference collections outside the training data; (3) a novel statistical topic model based on this metric that significantly improves topic quality in a large-scale document collection from the National Institutes of Health (NIH). {\textcopyright} 2011 Association for Computational Linguistics.},
author = {Mimno, David and Wallach, Hanna M. and Talley, Edmund and Leenders, Miriam and McCallum, Andrew},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Mimno et al. - 2011 - Optimizing semantic coherence in topic models.pdf:pdf},
isbn = {1937284115},
journal = {EMNLP 2011 - Conf. Empir. Methods Nat. Lang. Process. Proc. Conf.},
number = {2},
pages = {262--272},
title = {{Optimizing semantic coherence in topic models}},
year = {2011}
}
@article{Diab2011,
abstract = {Understanding why decision makers resist using standardized approaches to employee selection requires understanding basic feelings and beliefs about different approaches for collecting and combining assessment information. This study examines lay perceptions of selection decision aids, using a sample of 418 working adults. Holding constant the attributes measured, participants from the United States perceive holistic integration to be superior to mechanical integration for combining interview scores, as well as for combining test scores. Participants from outside of the United States prefer holistic integration of interview scores, but slightly prefer mechanical integration of test scores. {\textcopyright} 2011 Blackwell Publishing Ltd.},
author = {Diab, Dalia L. and Pui, Shuang Yueh and Yankelevich, Maya and Highhouse, Scott},
doi = {10.1111/j.1468-2389.2011.00548.x},
issn = {0965075X},
journal = {Int. J. Sel. Assess.},
month = {jun},
number = {2},
pages = {209--216},
title = {{Lay perceptions of selection decision aids in US and non-US samples}},
volume = {19},
year = {2011}
}
@article{Thonet2016,
abstract = {The surge of opinionated on-line texts provides a wealth of information that can be exploited to analyze users' viewpoints and opinions on various topics. This article presents VODUM, an unsupervised Topic Model designed to jointly discover viewpoints, topics, and opinions in text. We hypothesize that partitioning topical words and viewpoint-specific opinion words using part-of-speech helps to discriminate and identify viewpoints. Quantitative and qualitative experiments on the Bitterlemons collection show the performance of our model. It outperforms state-of-the-art baselines in generalizing data and identifying viewpoints. This result stresses how important topical and opinion words separation is, and how it impacts the accuracy of viewpoint identification.},
author = {Thonet, Thibaut and Cabanac, Guillaume and Boughanem, Mohand and Pinel-Sauvagnat, Karen},
doi = {10.1007/978-3-319-30671-1_39},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Thonet et al. - 2016 - VODUM A topic model unifying viewpoint, topic and opinion discovery.pdf:pdf},
isbn = {9783319306704},
issn = {16113349},
journal = {Lect. Notes Comput. Sci. (including Subser. Lect. Notes Artif. Intell. Lect. Notes Bioinformatics)},
pages = {533--545},
title = {{VODUM: A topic model unifying viewpoint, topic and opinion discovery}},
volume = {9626},
year = {2016}
}
@article{Amigo2018,
abstract = {Many evaluation metrics have been defined to evaluate the effectiveness ad-hoc retrieval and search result diversification systems. However, it is often unclear which evaluation metric should be used to analyze the performance of retrieval systems given a specific task. Axiomatic analysis is an informative mechanism to understand the fundamentals of metrics and their suitability for particular scenarios. In this paper, we define a constraint-based axiomatic framework to study the suitability of existing metrics in search result diversification scenarios. The analysis informed the definition of Rank-Biased Utility (RBU) -- an adaptation of the well-known Rank-Biased Precision metric -- that takes into account redundancy and the user effort associated to the inspection of documents in the ranking. Our experiments over standard diversity evaluation campaigns show that the proposed metric captures quality criteria reflected by different metrics, being suitable in the absence of knowledge about particular features of the scenario under study.},
annote = {they compare diversity metrics and introduce a new one (Rank-Biased Utulity)},
author = {Amig{\'{o}}, Enrique and Spina, Damiano and Carrillo-De-Albornoz, Jorge},
doi = {10.1145/3209978.3210024},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Amig{\'{o}}, Spina, Carrillo-De-Albornoz - 2018 - An axiomatic analysis of diversity evaluation metrics Introducing the rank-biased utility m.pdf:pdf},
isbn = {9781450356572},
journal = {41st Int. ACM SIGIR Conf. Res. Dev. Inf. Retrieval, SIGIR 2018},
keywords = {Axiomatic analysis,Evaluation,Search result diversification},
pages = {625--634},
title = {{An axiomatic analysis of diversity evaluation metrics: Introducing the rank-biased utility metric}},
year = {2018}
}
@article{Zafar2017,
abstract = {Automated data-driven decision making systems are increasingly being used to assist, or even replace humans in many settings. These systems function by learning from historical decisions, often taken by humans. In order to maximize the utility of these systems (or, classifiers), their training involves minimizing the errors (or, misclassifications) over the given historical data. However, it is quite possible that the optimally trained classifier makes decisions for people belonging to different social groups with different misclassification rates (e.g., misclassification rates for females are higher than for males), thereby placing these groups at an unfair disadvantage. To account for and avoid such unfairness, in this paper, we introduce a new notion of unfairness, disparate mistreatment, which is defined in terms of misclassification rates. We then propose intuitive measures of disparate mistreatment for decision boundary-based classifiers, which can be easily incorporated into their formulation as convex-concave constraints. Experiments on synthetic as well as real world datasets show that our methodology is effective at avoiding disparate mistreatment, often at a small cost in terms of accuracy.},
archivePrefix = {arXiv},
arxivId = {1610.08452},
author = {Zafar, Muhammad Bilal and Valera, Isabel and Rodriguez, Manuel Gomez and Gummadi, Krishna P.},
doi = {10.1145/3038912.3052660},
eprint = {1610.08452},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Zafar et al. - 2017 - Fairness beyond disparate treatment {\&} disparate impact Learning classification without disparate mistreatment.pdf:pdf},
isbn = {9781450349130},
journal = {26th Int. World Wide Web Conf. WWW 2017},
pages = {1171--1180},
title = {{Fairness beyond disparate treatment {\&} disparate impact: Learning classification without disparate mistreatment}},
year = {2017}
}
@article{Lin2006,
abstract = {In this paper we investigate a new problem of identifying the perspective from which a document is written. By perspective we mean a point of view, for example, from the perspective of Democrats or Repub- licans. Can computers learn to identify the perspective of a document? Not every sentence is written strongly from a per- spective. Can computers learn to identify which sentences strongly convey a partic- ular perspective? We develop statistical models to capture how perspectives are expressed at the document and sentence levels, and evaluate the proposed mod- els on articles about the Israeli-Palestinian conflict. The results show that the pro- posed models successfully learn how per- spectives are reflected in word usage and can identify the perspective of a document with high accuracy.},
author = {Lin, Wei Hao and Wilson, Theresa and Wiebe, Janyce and Hauptmann, Alexander},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Lin et al. - 2006 - Which side are you on Identifying perspectives at the document and sentence levels.pdf:pdf},
journal = {Proc. Tenth Conf. Comput. Nat. Lang. Learn. CoNLL-X},
pages = {109--116},
title = {{Which side are you on? Identifying perspectives at the document and sentence levels}},
year = {2006}
}
@inproceedings{Yang2017,
abstract = {Ranking and scoring are ubiquitous. We consider the setting in which an institution, called a ranker, evaluates a set of individuals based on demographic, behavioral or other characteristics. The final output is a ranking that represents the relative quality of the individuals. While automatic and therefore seemingly objective, rankers can, and often do, discriminate against individuals and systematically disadvantage members of protected groups. This warrants a careful study of the fairness of a ranking scheme, to enable data science for social good applications, among others. In this paper we propose fairness measures for ranked outputs. We develop a data generation procedure that allows us to systematically control the degree of unfairness in the output, and study the behavior of our measures on these datasets. We then apply our proposed measures to several real datasets, and detect cases of bias. Finally, we show preliminary results of incorporating our ranked fairness measures into an optimization framework, and show potential for improving fairness of ranked outputs while maintaining accuracy.},
address = {New York, NY, USA},
author = {Yang, Ke and Stoyanovich, Julia},
booktitle = {Proc. 29th Int. Conf. Sci. Stat. Database Manag.},
doi = {10.1145/3085504.3085526},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Yang, Stoyanovich - 2017 - Measuring fairness in ranked outputs.pdf:pdf},
isbn = {9781450352826},
keywords = {Accountability,Data,Data ethics,Data science for social good,Fairness,Responsibly,Transparency},
pages = {1--6},
publisher = {Association for Computing Machinery},
series = {SSDBM '17},
title = {{Measuring fairness in ranked outputs}},
year = {2017}
}
@article{Vargas2015,
abstract = {Recommender Systems have become a pervasive technology in a wide spectrum of everyday applications, and can be said to be familiar to the general public. In situations where there is an information overload, such as e-commerce, streaming platforms or social networks, providing personalized recommendations has proven to be a major source of enhanced functionality, user satisfaction, and revenue improvements. The development of recommendation algorithms and technologies has typically focused on maximizing the prediction accuracy of the user's interests. However, there is an increasing awareness in the field that there are other properties that have an impact on user satisfaction and business performance. In particular, there are many cases where applying some degree of novelty or diversity may be beneficial for both the users that receive the recommendations and the business that provides them. In this thesis we develop a principled approach to the evaluation and enhancement of novelty and diversity in Recommender Systems. We consider that the improvement of such fundamental dimensions of the usefulness of recommendations has to take into account how users explore and perceive recommendations, what are the problems that novelty and diversity solve and the causes of such problems. We propose in our first contribution a unified framework for the evaluation and enhancement of novelty and diversity in recommendations that generalizes and enhances many of the proposals previously studied in the state of the art under a common basis. Special emphasis is done in the study of the diversity within recommendations lists, for which two different contributions are presented. On the one hand, an adaptation of search result diversification metrics and techniques from Information Retrieval is explored to cope with the ambiguity of user interests and tastes. On the other hand, a domain-specific solution for assessing and optimizing the diversity of recommendations is proposed to address the need of users for varied recommendations when genre information about the recommendation domain is available. Finally, we address diversity as an overall quality from the system point of view, and we propose solutions for the problem in this perspective by turning the recommendation task around and recommending users to items. Our proposals are tested on a common experimental design that considers three different datasets for movie and music recommendation and four well-known baseline recommendation algorithms. The results of our experiments support the validity of our contributions and allow the analysis and further insights on their behavior when applied to different settings.},
author = {Vargas, Sa{\'{u}}l},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Vargas - 2015 - Novelty and Diversity Evaluation and Enhancement in Recommender Systems.pdf:pdf},
isbn = {978-1-4899-7637-6},
number = {February},
title = {{Novelty and Diversity Evaluation and Enhancement in Recommender Systems}},
year = {2015}
}
@inproceedings{Paul2010twodimensional,
annote = {see other paper by same authors where they describe the model shortly and apply it},
author = {Paul, Michael J and Girju, Roxana},
booktitle = {Proc. Twenty-Fourth AAAI Conf. Artif. Intell.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Paul, Girju - 2010 - A Two-Dimensional Topic-Aspect Model for Discovering Multi-Faceted Topics.pdf:pdf},
keywords = {Technical Papers -- Machine Learning},
pages = {545--550},
title = {{A Two-Dimensional Topic-Aspect Model for Discovering Multi-Faceted Topics}},
year = {2010}
}
@article{Zhu2019,
abstract = {When users express their stances towards a topic in social media, they might elaborate their viewpoints or reasoning. Oftentimes, viewpoints expressed by different users exhibit a hierarchical structure. Therefore, detecting this kind of hierarchical viewpoints offers a better insight to understand the public opinion. In this paper, we propose a novel Bayesian model for hierarchical viewpoint discovery from tweets. Driven by the motivation that a viewpoint expressed in a tweet can be regarded as a path from the root to a leaf of a hierarchical viewpoint tree, the assignment of the relevant viewpoint topics is assumed to follow two nested Chinese restaurant processes. Moreover, opinions in text are often expressed in un-semantically decomposable multi-terms or phrases, such as ‘economic recession'. Hence, a hierarchical Pitman–Yor process is employed as a prior for modelling the generation of phrases with arbitrary length. Experimental results on two Twitter corpora demonstrate the effectiveness of the proposed Bayesian model for hierarchical viewpoint discovery.},
author = {Zhu, Lixing and He, Yulan and Zhou, Deyu},
doi = {10.1016/j.eswa.2018.09.028},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Zhu, He, Zhou - 2019 - Hierarchical viewpoint discovery from tweets using Bayesian modelling.pdf:pdf},
issn = {09574174},
journal = {Expert Syst. Appl.},
keywords = {Bayesian modelling,Natural language processing,Opinion mining},
pages = {430--438},
publisher = {Elsevier Ltd},
title = {{Hierarchical viewpoint discovery from tweets using Bayesian modelling}},
volume = {116},
year = {2019}
}
@article{Pan2007,
abstract = {An eye tracking experiment revealed that college student users have substantial trust in Google's ability to rank results by their true relevance to the query. When the participants selected a link to follow from Google's result pages, their decisions were strongly biased towards links higher in position even if the abstracts themselves were less relevant. While the participants reacted to artificially reduced retrieval quality by greater scrutiny, they failed to achieve the same success rate. This demonstrated trust in Google has implications for the search engine's tremendous potential influence on culture, society, and user traffic on the Web.},
author = {Pan, Bing and Hembrooke, Helene and Joachims, Thorsten and Lorigo, Lori and Gay, Geri and Granka, Laura},
doi = {10.1111/j.1083-6101.2007.00351.x},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Pan et al. - 2007 - In Google we trust Users' decisions on rank, position, and relevance.pdf:pdf},
issn = {10836101},
journal = {J. Comput. Commun.},
number = {3},
pages = {801--823},
title = {{In Google we trust: Users' decisions on rank, position, and relevance}},
volume = {12},
year = {2007}
}
@article{Flores2016,
abstract = {The authors respond to a recent ProPublica article claiming that the widely used risk assessment tool COMPAS is biased against black defendants. They conclude that ProPublica's report was based on faulty statistics and data analysis and failed to show that the COMPAS itself is racially biased, let alone that other risk instruments are biased.},
author = {Flores, Anthony W. and Bechtel, Kristin and Lowenkamp, Christopher T.},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Flores, Bechtel, Lowenkamp - 2016 - False positives, false negatives, and false analyses A rejoinder to machine bias There's software us.pdf:pdf},
issn = {00149128},
journal = {Fed. Probat.},
number = {2},
pages = {38--46},
title = {{False positives, false negatives, and false analyses: A rejoinder to "machine bias: There's software used across the country to predict future criminals. And it's biased against blacks"}},
volume = {80},
year = {2016}
}
@article{Mironczuk2018,
abstract = {The aim of this study is to provide an overview the state-of-the-art elements of text classification. For this purpose, we first select and investigate the primary and recent studies and objectives in this field. Next, we examine the state-of-the-art elements of text classification. In the following steps, we qualitatively and quantitatively analyse the related works. Herein, we describe six baseline elements of text classification including data collection, data analysis for labelling, feature construction and weighing, feature selection and projection, training of a classification model, and solution evaluation. This study will help readers acquire the necessary information about these elements and their associated techniques. Thus, we believe that this study will assist other researchers and professionals to propose new studies in the field of text classification.},
author = {Miro{\'{n}}czuk, Marcin Micha{\l} and Protasiewicz, Jaros{\l}aw},
doi = {10.1016/j.eswa.2018.03.058},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Miro{\'{n}}czuk, Protasiewicz - 2018 - A recent overview of the state-of-the-art elements of text classification.pdf:pdf},
issn = {09574174},
journal = {Expert Syst. Appl.},
keywords = {Document classification,Document classification overview,Text classification,Text classification overview},
pages = {36--54},
title = {{A recent overview of the state-of-the-art elements of text classification}},
volume = {106},
year = {2018}
}
@article{Ghenai2020,
abstract = {The majority of US Internet users have searched the internet for health-related information. When people conduct these health searches, searching for information about medical treatments is among the more common reasons. While being a convenient and fast method to collect information, when used by people for health search, search engines can be biased toward results saying treatments are helpful, regardless of the truth. The presence of incorrect information in search results may potentially cause harm, especially if people believe what they read without further research or professional medical advice. In this paper, we aim to better understand the decision making process of determining the efficacy of medical treatments using search result pages. We conducted a think-aloud study in order to gain insights on strategies people use during online search for health related topics. We found that, even when participants are careful and focused on the task, biased search engine results can significantly influence people to make decisions consistent with the bias. The chief reason biased search engines results were able to influence participants is that participants often considered what the majority of the search results stated as part of their decision-making. We also found that participants looked for indications of authoritativeness and quality when evaluating online content. While rank bias and a bias towards wanting treatments to be helpful has been found in prior studies, our participants did not reveal these biases as part of their spoken thoughts. Our results imply that more attention should be paid to search engines' biases given people's bias towards accepting the most common answer in the results as the correct answer. When search results are biased toward incorrect results for health-related searches, dire consequences may be the result.},
annote = {this paper directly builds upon pogacar et.al (2017) where the same authors showed that people are influenced by search result rankings when judging the efficacy of medical treatment

they present a think-aloud study that confirms the results of the previous study; namely that people are biased towards the answer that is preferred in the search result ranking, no matter whether it is helpful or not -- although the results are a bit shaky, because of a multilevel structure (8 treatments, 4 helpful and 4 unhelpful; 16 participants; each participant analysed multiple SERPs... a bit unclear but maybe this becomes clearer when reading the previous paper as they did the same there)

the main findings of this paper are that (1) this effect occurs despite a lab setting in which people have to consciously explain their behavior and choices, (2) majority view in the results, authoritativeness of the source, and quality of source are among the most important factors for decision making here, and (3) people did not experience bias directly despite falling prey to it -- especially findings (2) and (3) are useful for my research

I would like to see some more nuance in this though; biased SERPs had 8/10 results from one side, but what happens when it's 5/10 or 6/10?},
author = {Ghenai, Amira and Smucker, Mark D. and Clarke, Charles L.A.},
doi = {10.1145/3343413.3377961},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Ghenai, Smucker, Clarke - 2020 - A think-aloud study to understand factors affecting online health search.pdf:pdf},
isbn = {9781450368926},
journal = {CHIIR 2020 - Proc. 2020 Conf. Hum. Inf. Interact. Retr.},
keywords = {Decision-making,Health search,Misinformation,User study},
pages = {273--282},
title = {{A think-aloud study to understand factors affecting online health search}},
year = {2020}
}
@inproceedings{Grgic-Hlaca2018,
abstract = {As algorithms are increasingly used to make important decisions that affect human lives, ranging from social benefit assignment to predicting risk of criminal recidivism, concerns have been raised about the fairness of algorithmic decision making. Most prior works on algorithmic fairness normatively prescribe how fair decisions ought to be made. In contrast, here, we descriptively survey users for how they perceive and reason about fairness in algorithmic decision making. A key contribution of this work is the framework we propose to understand why people perceive certain features as fair or unfair to be used in algorithms. Our framework identifies eight properties of features, such as relevance, volitionality and reliability, as latent considerations that inform people's moral judgments about the fairness of feature use in decision-making algorithms. We validate our framework through a series of scenario-based surveys with 576 people. We find that, based on a person's assessment of the eight latent properties of a feature in our exemplar scenario, we can accurately ({\textgreater} 85{\%}) predict if the person will judge the use of the feature as fair. Our findings have important implications. At a high-level, we show that people's unfairness concerns are multi-dimensional and argue that future studies need to address unfairness concerns beyond discrimination. At a low-level, we find considerable disagreements in people's fairness judgments. We identify root causes of the disagreements, and note possible pathways to resolve them.},
author = {Grgic-Hlaca, Nina and Redmiles, Elissa M. and Gummadi, Krishna P. and Weller, Adrian},
booktitle = {Proc. 2018 World Wide Web Conf.},
doi = {10.1145/3178876.3186138},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Grgic-Hlaca et al. - 2018 - Human Perceptions of Fairness in Algorithmic Decision Making.pdf:pdf},
isbn = {9781450356398},
keywords = {Algorithmic Discrimination,Algorithmic Fairness,Fair Feature Selection,Fairness in Machine Learning,Procedural Fairness,algorithmic discrimination,algorithmic fairness,chine learning,elissa redmiles acknowledges support,fair feature selection,fairness in ma-,foundation graduate,from the national science,procedural fairness},
pages = {903--912},
title = {{Human Perceptions of Fairness in Algorithmic Decision Making}},
year = {2018}
}
@article{Muir1996,
author = {{Muir, Bonnie M and Moray}, Neville},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Muir, Bonnie M and Moray - 1996 - Trust in automation. Part II. Experimental studies of trust and human intervention in a process contro.pdf:pdf},
journal = {Ergonomics},
number = {3},
pages = {429--460},
title = {{Trust in automation. Part II. Experimental studies of trust and human intervention in a process control simulation}},
volume = {39},
year = {1996}
}
@article{Posch2018,
abstract = {Micro-task crowdsourcing is an international phenomenon that has emerged during the past decade. This paper sets out to explore the characteristics of the international crowd workforce and provides a cross-national comparison of the crowd workforce in ten countries. We provide an analysis and comparison of demographic characteristics and shed light on the significance of micro-task income for workers in different countries. This study is the first large-scale country-level analysis of the characteristics of workers on the platform Figure Eight (formerly CrowdFlower), one of the two platforms dominating the micro-task market. We find large differences between the characteristics of the crowd workforces of different countries, both regarding demography and regarding the importance of micro-task income for workers. Furthermore, we find that the composition of the workforce in the ten countries was largely stable across samples taken at different points in time.},
archivePrefix = {arXiv},
arxivId = {1812.05948},
author = {Posch, Lisa and Bleier, Arnim and Fl{\"{o}}ck, Fabian and Strohmaier, Markus},
eprint = {1812.05948},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Posch et al. - 2018 - Characterizing the Global Crowd Workforce A Cross-Country Comparison of Crowdworker Demographics.pdf:pdf},
pages = {1--28},
title = {{Characterizing the Global Crowd Workforce: A Cross-Country Comparison of Crowdworker Demographics}},
url = {http://arxiv.org/abs/1812.05948},
year = {2018}
}
@inproceedings{Smith2020,
abstract = {Algorithmic fairness for artificial intelligence has become increasingly relevant as these systems become more pervasive in society. One realm of AI, recommender systems, presents unique challenges for fairness due to trade offs between optimizing accuracy for users and fairness to providers. But what is fair in the context of recommendation--particularly when there are multiple stakeholders? In an initial exploration of this problem, we ask users what their ideas of fair treatment in recommendation might be, and why. We analyze what might cause discrepancies or changes between user's opinions towards fairness to eventually help inform the design of fairer and more transparent recommendation algorithms.},
archivePrefix = {arXiv},
arxivId = {2003.06461},
author = {Smith, Jessie and Sonboli, Nasim and Fiesler, Casey and Burke, Robin},
booktitle = {CHI'20 Work. Human-Centered Approaches to Fair Responsible AI},
eprint = {2003.06461},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Smith et al. - 2020 - Exploring User Opinions of Fairness in Recommender Systems.pdf:pdf},
title = {{Exploring User Opinions of Fairness in Recommender Systems}},
url = {http://arxiv.org/abs/2003.06461},
year = {2020}
}
@inproceedings{Ahmad2013,
abstract = {Attitudinal theory from the social psychology has been widely used in developing persuasive information technology and services in conjunction to shape or change user's attitude or behavior. Persuasion is the essence in building trust. The nature of this article is conceptual-theoretical where it discusses how emotion approach can be used to make people trust persuasive application. This article describes the three components; persuasive technology, trust, and emotion individually and the relation between them. Moreover, a conceptual model with related elements is proposed to show the relationship between those components. {\textcopyright} 2013 Springer International Publishing.},
author = {Ahmad, Wan Nooraishya Wan and Ali, Nazlena Mohamad},
booktitle = {Int. Vis. Informatics Conf.},
doi = {10.1007/978-3-319-02958-0_64},
issn = {03029743},
pages = {707----717},
publisher = {Springer},
title = {{Engendering trust through emotion in designing persuasive application}},
year = {2013}
}
@article{Hollebeek2016,
abstract = {{\textcopyright} 2016, {\textcopyright} Emerald Group Publishing Limited. Purpose: Although “engagement” is receiving increasing attention in the marketing literature, the characteristics and dynamics characterizing this concept in specific contextual conditions, including consumers' selection of particular music and ensuing music-related behaviors, remain nebulous to date. This study aims to develop the concept of consumers' musical engagement (ME) and explore it within a broader nomological network of conceptual relationships. Design/methodology/approach: To investigate the research gap, the authors deploy a survey sampling 2,498 US-based adults to develop and confirm a 25-item ME scale. The authors also test their scale in a broader nomological network of specific theoretical relationships using regression and mediation modeling. Findings: The authors identify three ME factors, namely, social identity, transportive and affect-inducing engagements. The authors find ME to exhibit a nonlinear effect on music consumption with increasing returns. Although both social identity and transportive experiences represent significant predictors of music consumption, the effect of affect-inducing experience is non-significant. Further, the social identity experience has a significantly greater association with music consumption than the transportive experience. Research limitations/implications: This paper provides a conceptualization and an associated diagnostic tool for ME, in addition to initial insight into the role of ME in a broader nomological network of conceptual relationships. Based on the identified research limitations, the authors also provide key future research directions for ME. Practical implications: The insight attained into ME may be used to underpin the design, implementation and evaluation of managerial ME-based tactics and strategies in the music industry. In particular, the authors find that successful appeals to consumers' social identity engagement are a significant driver of increased future music consumption. The authors provide a number of managerial recommendations to develop this particular ME dimension. Originality/value: This paper provides an ME conceptualization and an associated scale and explores ME within a broader nomological network of theoretical relationships. The authors also draw key implications from these analyses.},
author = {Hollebeek, Linda D. and Malthouse, Edward C. and Block, Martin P.},
doi = {10.1108/JCM-02-2016-1730},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Hollebeek, Malthouse, Block - 2016 - Sounds of music exploring consumers' musical engagement.pdf:pdf},
issn = {07363761},
journal = {J. Consum. Mark.},
keywords = {Consumer behavior,Musical engagement (ME),Structural equation model},
number = {6},
pages = {417--427},
title = {{Sounds of music: exploring consumers' musical engagement}},
volume = {33},
year = {2016}
}
@article{Wang2020,
abstract = {Algorithmic decision-making systems are increasingly used throughout the public and private sectors to make important decisions or assist humans in making these decisions with real social consequences. While there has been substantial research in recent years to build fair decision-making algorithms, there has been less research seeking to understand the factors that affect people's perceptions of fairness in these systems, which we argue is also important for their broader acceptance. In this research, we conduct an online experiment to better understand perceptions of fairness, focusing on three sets of factors: algorithm outcomes, algorithm development and deployment procedures, and individual differences. We find that people rate the algorithm as more fair when the algorithm predicts in their favor, even surpassing the negative effects of describing algorithms that are very biased against particular demographic groups. We find that this effect is moderated by several variables, including participants' education level, gender, and several aspects of the development procedure. Our findings suggest that systems that evaluate algorithmic fairness through users' feedback must consider the possibility of outcome favorability bias.},
archivePrefix = {arXiv},
arxivId = {2001.09604},
author = {Wang, Ruotong and Harper, F. Maxwell and Zhu, Haiyi},
eprint = {2001.09604},
file = {:Users/tim/Surfdrive/Research/Library/Literature/Wang, Harper, Zhu - 2020 - Factors Influencing Perceived Fairness in Algorithmic Decision-Making Algorithm Outcomes, Development Procedu.pdf:pdf},
isbn = {9781450367080},
pages = {1--14},
title = {{Factors Influencing Perceived Fairness in Algorithmic Decision-Making: Algorithm Outcomes, Development Procedures, and Individual Differences}},
url = {http://arxiv.org/abs/2001.09604},
year = {2020}
}
@inproceedings{White2013,
abstract = {People's beliefs, and unconscious biases that arise from those beliefs, influence their judgment, decision making, and actions, as is commonly accepted among psychologists. Biases can be observed in information retrieval in situations where searchers seek or are presented with information that significantly deviates from the truth. There is little understanding of the impact of such biases in search. In this paper we study search-related biases via multiple probes: an exploratory retrospective survey, human labeling of the captions and results returned by a Web search engine, and a large-scale log analysis of search behavior on that engine. Targeting yes-no questions in the critical domain of health search, we show that Web searchers exhibit their own biases and are also subject to bias from the search engine. We clearly observe searchers favoring positive information over negative and more than expected given base rates based on consensus answers from physicians. We also show that search engines strongly favor a particular, usually positive, perspective, irrespective of the truth. Importantly, we show that these biases can be counterproductive and affect search outcomes; in our study, around half of the answers that searchers settled on were actually incorrect. Our findings have implications for search engine design, including the development of ranking algorithms that con-sider the desire to satisfy searchers (by validating their beliefs) and providing accurate answers and properly considering base rates. Incorporating likelihood information into search is particularly important for consequential tasks, such as those with a medical focus.},
address = {New York, NY, USA},
annote = {this is a very good paper and quite close to what I want to do in the "bias in search" project;

they focused on medical questions that have a clear "yes / no" answer (as judged by expert consensus)

the study setup is sketched pretty clearly, so I could literally do the same thing with slight adjustments},
author = {White, Ryen W.},
booktitle = {Proc. 36th Int. ACM SIGIR Conf. Res. Dev. Inf. Retr.},
doi = {10.1145/2484028.2484053},
file = {:Users/tim/Surfdrive/Research/Library/Literature/White - 2013 - Beliefs and biases in web search.pdf:pdf},
isbn = {9781450320344},
keywords = {Beliefs,Biases,Health search,Search interaction},
pages = {3--12},
publisher = {Association for Computing Machinery},
series = {SIGIR '13},
title = {{Beliefs and biases in web search}},
url = {https://doi.org/10.1145/2484028.2484053},
year = {2013}
}
@book{jeffreys1939,
address = {Oxford},
author = {Jeffreys, Harold},
publisher = {Oxford University Press},
title = {{Theory of Probability}},
year = {1939}
}

@article{Varshney2019,
  title="Trustworthy Machine Learning and Artificial Intelligence",
  author="Varshney, Kush R.",
  journal="ACM XRDS Magazine",
  volume={25},
  number={3},
  pages={26--29},
  year={2019}
}

@inproceedings{Varshney2020,
  title="On Mismatched Detection and Safe, Trustworthy Machine Learning",
  author="Varshney, Kush R.",
  booktitle="Proceedings of the Conference on Information Sciences and Systems",
  month=mar,
  year={2020}
}
